Finding Adversarial Inputs for Heuristics using Multi-level Optimization

Production systems use heuristics because they are faster or scale better than their optimal counterparts. Yet, practitioners are often unaware of the performance gap between a heuristic and the optimum or between two heuristics in realistic scenarios. We present MetaOpt, a system that helps analyze heuristics. Users specify the heuristic and the optimal (or another heuristic) as input, and MetaOpt automatically encodes these efficiently for a solver to find performance gaps and their corresponding adversarial inputs. Its suite of built-in optimizations helps it scale its analysis to practical problem sizes. To show it is versatile, we used MetaOpt to analyze heuristics from three domains (traffic engineering, vector bin packing, and packet scheduling). We found a production traffic engineering heuristic can require 30% more capacity than the optimal to satisfy realistic demands. Based on the patterns in the adversarial inputs MetaOpt produced, we modified the heuristic to reduce its performance gap by 12.5$\times$. We examined adversarial inputs to a vector bin packing heuristic and proved a new lower bound on its performance.

==> texfiles/abstract.tex <==
%\begin{abstract}
%	\pooria{Lock file: \href{https://docs.google.com/document/d/1rllne4cNdt808XzSEKp8h79GSjC_Efa_2WWLxE56_Sk/edit?usp=sharing}{Link}}
%	Operators use heuristics because they are faster or scale better than their optimal counterparts: we need ``heuristic analyzers'' that find the worst-case gap of these heuristics {\em at scale} and help improve our understanding of their short-comings to avoid unexpected problems in production. 
	
%	 \metaopt advances our understanding of how these heuristics behave at larger scales and enables rich queries. \metaopt can analyze a broad set of heuristics such as popular heuristics in traffic engineering and vector bin packing. It shows some heuristics in traffic engineering~\cite{blastshield, pop} have higher optimality gaps than what the authors of those heuristics thought possible. Our most notable finding using \metaopt is a tighter optimality gap bound for a well-known vector bin packing heuristic compared to what the community has been able to prove to date.
	 
%	 In production systems, heuristics are frequently used instead of optimal solutions because they are faster and scale better. However, the actual worst-case performance of these heuristics in real-world scenarios is often unclear. We introduce {\metaopt}, a tool that helps us better understand the performance of the heuristics at {\em scale}. With {\metaopt}, we can find inputs that lead to the largest gap between a heuristic and an optimal solution and answer a range of performance-related questions. We apply {\metaopt} to a broad set of heuristics from traffic engineering and vector bin packing. Our results uncover new performance gaps for traffic engineering heuristics and prove a tighter optimality bound for a well-known vector bin packing heuristic.
	
	% Instead of optimal solutions, production systems frequently use heuristics because they are faster and scale better. However, the actual worst-case performance of these heuristics in real-world scenarios is often unclear. We introduce MetaOpt, a tool that helps us better understand the performance of the heuristics at scale. With MetaOpt, we can find inputs that lead to the largest gap between a heuristic and an optimal solution and answer a range of performance-related questions about heuristics. We apply MetaOpt to a broad set of heuristics from traffic engineering and vector bin packing. Our results uncover new performance gaps for traffic engineering heuristics and prove a tighter optimality bound for a well-known vector bin packing heuristic.
	
	%Production systems use heuristics because they are faster or scale better than their optimal counterparts. Prior work showed the optimality gap of deployed heuristics is as high as $50\%$~\cite{metaopt}. We show how to {\em scalably} compute bounds on the optimality-gap of practical heuristics, find inputs that result in these gaps, and interpret and use the solution to improve the heuristics themselves. We demonstrate the breadth of use-cases for this system by showing how to apply it to problems in vastly different domains: traffic engineering and vector bin packing --- we find optimality gaps as high as XXX and XXX in each of these domains respectively.
	
	%\pooria{suggestion: Production systems favor heuristics over optimal algorithms for their speed and scalability. Nevertheless, the worst-case performance of these heuristics in real-world scenarios is often unclear to practitioners. In fact, prior work has shown that the difference between heuristics and optimal solutions can be substantial~\cite{metaopt}. We present a {\em scalable} method to measure this performance gap, identify (realistic) inputs that cause it, and help operators improve their heuristics. We demonstrate the versatility of our approach by applying it to two diverse domains: traffic engineering and vector bin packing. Our results reveal optimality gaps of XXX and XXX in each domain, respectively.}
%	\pooria{I prefer to not mention the 50\% gap from hotnets. Our evaluation is different here and more realistic compared to our hotnet submission (more paths, lower upper bound, \etc). So, the gap we find may be lower.}
%	\pooria{From SIGCOMM's website:}
%	\pooria{Work that extends an author's previous workshop paper is welcome, but in their submitted SIGCOMM paper the author(s) should (a) acknowledge their own previous workshop publication with an anonymous citation (e.g., "[7] Anonymized workshop paper") and (b) explain the differences between the SIGCOMM submission and the prior workshop paper. In addition, the online submission form will require authors to submit the deanonymized citation and a short explanation of the differences from the prior workshop paper. }
%	\pooria{Also, should we change the title of the paper?}
%\end{abstract}

==> texfiles/background.tex <==

\section{Heuristic analysis at a glance}
\label{s:background}

Operators use heuristics to solve problems when they are either NP-hard (in which case they have no other alternatives) or the optimum has other limitations (\eg it is too costly). We describe four such heuristics and preview how \metaopt helped us analyze and understand their optimality gap. % We will discuss how we encode these heuristic in \metaopt in~\S\ref{s:d:heur_form} and evaluate \metaopt more completely in~\S\ref{s:eval}. We focus on heuristics from vastly different domains to show \metaopt applies to many heuristics across systems and networking. We look at heuristics in Traffic Engineering (TE), queuing, and Vector Bin-Packing (VBP). Operators use these heuristics in deployed systems and networks~\cite{blastshield, yarn_vbp}.

% \behnaz{do we have citations for \ffd deployments?}
% \behnaz{Can we say anything about how much revenue is lost when these heuristics underperform? do we have any numbers?}
\vspace{-0.7mm}
\subsection{The heuristics and why they matter}

\parab{Traffic engineering (TE).} The demand pinning and \pop heuristics in TE use very different techniques to improve scalability:


%\vspace{0.05in}
\noindent \textit{Demand Pinning (\dempin)}~\cite{blastshield}, which we described in~\S\ref{s:intro} and is in production use at Microsoft, 
pre-allocates flows along the shortest path for any node pair with demand smaller than a threshold $T_d$:

\begin{footnotesize}
\vspace{-3mm}
	\begin{alignat}{5}
		\multispan{4}\mbox{$\displaystyle \label{eq:demand_pinning} {\sf DemandPinning}(\mathcal{D}, \mathcal{P}) \triangleq \big\{\mathbf{f} \mid$} & \\
		& f_k^p & = & \begin{cases} d_k & \mbox{if }\ p\  \mbox{is shortest path in } P_k \\ 0 & \mbox{otherwise} \end{cases}, \,\, \forall k \in \mathcal{D}: d_k \leq T_d \big\}, \nonumber		
\end{alignat}
\vspace{-2mm}
\end{footnotesize}

and uses the SWAN~\cite{swan} optimization to route the remaining demands.


\noindent\textit{Partitioned Optimization Problems (\pop)~\cite{pop}.} \pop divides node pairs (and their demands) uniformly at random into partitions; assigns each partition an even share of edge capacities; and solves the original problem (e.g. the SWAN optimization~\cite{swan}) in parallel, once per partition. \pop results in a substantial speedup because it solves sub-problems that are smaller than the original (LP solver times are super-linear in problem sizes~\cite{boyd_co}) and it solves them in parallel.
 

\vspace{0.05in}
\dempin and \pop are qualitatively different; the former takes conditional actions while the latter uses randomness. 

\parab{Vector bin packing (VBP).} Production deployments use vector bin packing ({\vbp}) in multiple domains to efficiently allocate resources~\cite{protean,tetris,synergy,yarn_vbp,jobpacking}. We consider a simple offline version: given a set of balls and bins with specific sizes and multiple dimensions~(\eg memory, CPU, GPU~\cite{drf,borg,pond}), it tries to pack balls into the fewest number of bins. The optimal VBP problem is APX-hard~\cite{vbp-nphard}. 

A heuristics that practitioners commonly use is first fit decreasing~(\ffd). \ffd is gready and iterative: in each step it picks the unassigned ball with the {\em largest weight} and places it on the {\em first} bin that it {\em fits} in (that has enough capacity).
Prior work propose different ways to weight the balls~\cite{VBP-Heuristics,ffdprod-sandpiper,ffdsum-example,ffddiv-ibm,tetris,protean,synergy}. A particular variant is {\sf FFDSum} which, when balls have multiple dimensions, uses the sum of the dimensions across the items as the weights.  

\parab{Queue scheduling algorithms~\cite{sp-pifo}}. SP-PIFO is an algorithm that approximates Push-In-First-Out (PIFO) queuing. It models a PIFO through $n$ (large) priority first in first out queues where an item can only enter a queue if the priority of the queue (which is {\em usually} equal to the priority of the last item in it) is higher than the item's priority. The algorithm scans queues from lowest to highest priority and places the item in the first queue that accepts it. SP-PIFO updates all the queues' priorities if no queue can admit an item. 



%For either heuristic, given a topology, we use \metaopt to search for an input demand that maximizes the performance gap for that topology. Besides such \textit{worst-case input} demand, we also use \metaopt to quickly find inputs with a large gap (not necessarily the worst) or to search for inputs that also satisfy other realistic constraints~(e.g., within a certain distance from an actual demand). 

We highlight these example heuristics (\dempin, \pop, \ffd, and SP-PIFO) because they cover the broad range of heuristics \metaopt supports: (1) \dempin represents heuristics that involve conditional actions (which introduce non-convexity); (2) \pop represents probabilistic algorithm; (3) \ffd represents algorithmic heuristics that don't solve optimizations at all; and (4) SP-PIFO represents algorithms that involve decisions based on weights or priorities and those that involve updates to such weights/priorities. 


 
\subsection{{\metaopt}'s analysis (a preview)}

A heuristic analyzer can help operators understand the limitations of their heuristics before they deploy them and to create backup plans (\eg through caches that store the optimal solution or changes to the heuristic~\S\ref{s:eval}). We show examples of the analysis \metaopt enables (evaluation continues in~\S\ref{s:eval}).


\begin{table}[t!]
\centering
{\footnotesize
	\begin{tabular}{ c c c c c }
		
		\multirow{2}*{${\sf OPT}(\mathcal{I})$ }& \multicolumn{2}{c}{\metaopt} & \multicolumn{2}{c}{theoretical bound~\cite{VBP-Heuristics}} \\ \cline{2-5}
		& \#balls & approx ratio & \#balls & approx ratio \\ \hline
		2 & 6 & 2.0 & 4 & 1.0 \\
		3 & 9 & 2.0 & 12 & 1.33 \\
		4 & 12 & 2.0 & 24 & 1.5 \\
		5 & 15 & 2.0 & 40 & 1.6 \\
		\hline
	\end{tabular}
}
\caption{The approximation ratios adversarial inputs to 2d-FFD achieve for those inputs that \metaopt generates and those from the best known theoretical bound~\cite{VBP-Heuristics}.\label{tab:2d-ffd}}
%Approximation ratios for 2d-FFD achieved by the adversarial inputs generated by \metaopt and the inputs crafted by the best known theoretical bound~\cite{VBP-Heuristics}. \label{tab:2d-ffd}}
\end{table}


\noindent \textbf{\metaopt helps identify {\em why} \dempin underperforms (Figure~\autoref{f:dp_thresh}).} Intuitively, if we increase the \dempin threshold we increase its optimality gap: the heuristic will pin even more demands on their shortest path. But the gap grows much faster on some topologies~---~even those that have roughly the same number of nodes, edges, and even diameter!

We find the gap grows with the {\em average} (this is different from the diameter of the graph) length of the shortest paths.

As the shortest path length between the different node-pairs increases it causes \dempin to use the capacity on more edges when it pins their demand (if their demand falls bellow the threshold). This, in turn, reduces the available capacity to route other demands and increases the optimality gap.

\begin{figure}[t!]
	\centering
	\subfigure[Gap vs. the threshold value for {\dempin}.]{
		\centering
		\includegraphics[width=0.91\linewidth]{figs/sweep_threshold_dp/demandpinning_sweep_threshold.pdf}
		\label{f:dp_thresh}
	}
	\\
	\subfigure[Gap vs. connectivity.]{
		\centering
		\includegraphics[width=0.91\linewidth]{figs/sweep_topo_dp/demand_pinning_sweep_topo.pdf}
		\label{f:dp_path_length}
	}
	\caption{DP's optimality gap when we vary: (a) the \dempin threshold; and (b) connectivity. We normalize the gap by the total capacity.
		%for different values of threshold and on synthetic graphs with different path lengths.
		\label{f:maxgap_vs_params_dp}}
\end{figure}

\vspace{1mm}

\parab{We can use \metaopt to analyze combinations of heuristics.}
Imagine a new heuristic that runs \pop and \dempin in parallel and selects the best solution for each input. At first it seems the two heuristics have distinct adversarial inputs: \dempin underperforms when distant pairs have small demands and \pop when large demands that go through the same link end up in the same partition~---~we expect we can significantly reduce the optimality gap compared to each individual heuristic if we combine them. \metaopt found the new heuristic only improves the optimality gap by $6\%$! It finds adversaries where small demands are between distant pairs and large demands are between nearby nodes that end up in the same partition (which matches our intuition) but the combination of the two heuristics is not enough to fully mitigate the impact of the adversarial pattern. %Small demands are adversarial to \dempin and large ones to \pop. 


\parab{\metaopt can also find {\em realistic} adversarial inputs (\figref{f:real-constr:locality}).}  
Demands have strong locality in production~\cite{ncflow} and the demand matrices are very sparse (only a small fraction of pairs have non-zero demands). We can add these requirements as additional constraints in \metaopt and it indeed finds dense adversarial demands where the majority of demands are between nearby nodes. We find the gap only reduces by less than one percent when we do this! %This shows even in realistic settings \dempin and \pop have substantial optimality gaps.  


%\figref{f:real-constr:locality} shows features of the adversarial inputs \metaopt finds for \dempin and \pop in the absence of additional constraints: $50\%$ of large demands are over $7$ hops apart in both cases and more than half the demands in the \dempin case ($\ge 54\%$) are non-zero. 
%These findings suggest \metaopt's result is likely an over-estimate and not representative of how these heuristics perform in empirically relevant inputs.

%To find more realistic adversarial inputs, we restrict the demand space: we only allow large demands between nodes that are less than $4$ hops apart. 
%This constraint improves the locality and density of the adversarial demands and they become closer to real-world demand matrices. 
%But the gap is only minimally reduced by this change ($<1\%$).
%This shows {\pop} and {\dempin} can still have large gaps even when subjected to realistic demand matrices.



\begin{figure}[t]
	\subfigure[Impact of adding locality constraint on gap and density]{
		\centering
		{\footnotesize
			\begin{tabular}{c l c c }
				
				Heu & Constraint & Density & Gap \\ \hline
				\multirow{2}{*}{{\dempin}} & ~--~ & 54.06\% & 33.9\% \\ 
				& locality (distance of large demands $\leq 4$) & 12.03\% & 33.4\% \\\hline
				\multirow{2}{*}{{\pop}} & ~--~ & 16.14\% & 20.76\% \\ 
				& locality (distance of large demands $\leq 4$)& 4.74\% & 20.70\% \\ \hline
			\end{tabular}
		}
	}  
	\\
	\subfigure[Impact of adding locality constraint on {\dempin}]{
		\centering
		\includegraphics[width=0.91\linewidth]{figs/realistic_constraints/locality_demands_dp_0.05.pdf}
	}
	\\
	\subfigure[Impact of adding locality constraint on {\pop}]{
		\centering
		\includegraphics[width=0.91\linewidth]{figs/realistic_constraints/locality_demands_Avg-POP_0.05.pdf}
	}
	\caption{We use \metaopt to find practical adversarial inputs on Cogentco where we ensured large demands can only happen between nearby nodes. In both cases, the constraint on the input space led to more local and sparser adversarial inputs. \label{f:real-constr:locality}}
\end{figure}







\parab{\metaopt helps prove a tighter bound for the optimality gap of 2d-\ffd.} Multiple systems use two dimensional \ffd (2d-\ffd)~\cite{protean,tetris,synergy}. Theoretical guarantees for \ffd~\cite{VBP-Heuristics,multi-bp-survery} substantially lag behind its production use. Recently, \cite{VBP-Heuristics} crafts an example to show 
${\sf FFDSum}(\mathcal{I}) \geq \alpha_{{\sf OPT}(\mathcal{I})} {{\sf OPT}(\mathcal{I})}$ where $\alpha_{{\sf OPT}(\mathcal{I})} \in [1,2)$ and $\alpha_{{\sf OPT}(\mathcal{I})} \to 2$ as ${{\sf OPT}(\mathcal{I})} \to \infty$ which means
the approximation ratio $\frac{{\sf FFDSum}(\mathcal{I})}{{\sf OPT}(\mathcal{I})}$ converges to $2$ for large enough problems. But this bound is strictly smaller than $2$ for any problem of finite size. \metaopt finds adversarial inputs that cause an approximation ratio of $2$ \emph{for every problem size we considered} (Table~\ref{tab:2d-ffd})! These empirical findings suggest the approximation ratio of ${\sf FFDSum}$ is at least $2$ for a wide variety of problems. This means the heuristic is $2\times$ worse than the optimal!

We next show how we can derive constructive proofs for combinatorial problems with {\metaopt}'s help~---~
we extrapolated from the adversarial inputs it generated and proved:


%\metaopt in this setting finds adversarial inputs that achieve approximation ratios of $2$ \emph{for every problem size we considered} (Table~\ref{tab:2d-ffd}).
%For example, when $\opt(\mathcal{I}) = 4$ bins, \metaopt finds an adversarial input $\mathcal{I}$ with $12$ balls such that ${\sf FFDSum}(\mathcal{I}) = 8$ (=approx. ratio of $2$)  while \cite{VBP-Heuristics} uses $24$ balls and only achieves ${\sf FFDSum}(\mathcal{I}) = 6$ (approx. ratio = $1.5$).





%The empirical findings in~\autoref{tab:2d-ffd} suggest the approximation ratio of ${\sf FFDSum}$ is at least $2$ for a wide variety of problems.
%We show this formally:

% Thus, the approximation ratio of FFDSum for 2-dimensional \vbp is at least 2. 
\begin{theorem}
	\label{th:ffdsum:approx-ratio}
	In 2-dimensional \vbp, for any $k > 1$, there exists an input $\mathcal{I}$ with $OPT(\mathcal{I}) = k$ and $FFDSum(\mathcal{I}) \geq 2k$. 
\end{theorem}
\begin{proof}[Proof Sketch]
	\secref{apendix:proof:ffdsum} contains the detailed proof. For any non-negative integer $p$ and $m$ (at least one positive), we can construct an input with $6m + 9p$ balls such that \opt needs $k = 2m + 3p$ bins while ${\sf FFDSum}$ needs $4m + 6p$ bins.
\end{proof}

Our constructive proof in~\secref{apendix:proof:ffdsum} directly follows from the adversarial inputs \metaopt found: Theorem~\ref{th:ffdsum:approx-ratio} shows yet another use of {\metaopt}, where users can interpret common features across the adversarial inputs \metaopt finds and incorporate them in theoretical proofs. We derive a similar constructive proof for SP-PIFO through the adversarial inputs \metaopt found (see~\S\ref{}).
\behnaz{add SP-PIFO theorem to appendix and then reference here.}

\begin{figure}[t]
	\includegraphics[width=0.91\linewidth]{figs/SP-PIFO/sp_pifo_packet_delay.pdf}
	\caption{We compared the average delay of packets with the same priority. We use a stream of $10^6$ packets where the priority of packets is between $0-100$. As in SP-PIFO we use infinite queues. We normalize the numbers by the average delay of the highest priority packets (rank = 0). For the case where all the $10^6$ packets arrive at the same time and the queues drains at $40$ Gbps the average delay for the highest priority packets in PIFO is $0.074$ seconds (the sequence of packets results in similar relative performance between the heuristic and the optimal for any arrival/departure pattern).}
\end{figure}
\parab{\metaopt shows SP-PIFO delays the highest priority packets by $3\times$ compared to PIFO.} \metaopt finds a packet trace where SP-PIFO cannot approximate priorities correctly (the highest priority packets experience $3\times$ higher delay on average compared to the second lowest priority packets).



%We find the optimality gap of both heuristics is higher than what previous studies reported~\cite{blastshield,pop}.

\vspace{1mm}



These results show how \metaopt can help operators understand the limitations of different heuristics and compare heuristics against each other. An interesting future direction is to add support to \metaopt to identify what topologies trigger the worst case outcome for the heuristic.

%We next describe how \metaopt works in more detail. For more evaluations of how \metaopt performs please see~\S\ref{s:eval}.




==> texfiles/design.tex <==
\section{Finding adversaries quickly}
%\section{Quickly finding High-Quality Adversarial Inputs}
\label{s:design}


Our goal is to build a {\em widely applicable} tool that produces inputs {\em that trigger large optimality gaps} (i.e., large gaps between the optimal and the heuristic) {\em quickly and at scale}.


%\parab{Produces good quality adversaries:} 
%
%
%
%We want to find inputs that produce large optimality gaps (i.e., large gaps between the optimal and the heuristic) and recover the worst-case inputs, when possible.
%
%\parab{Scales to realistic instances:} We want a tool that can operate at scale~---~one that can directly analyze large instances.
%
%
%\parab{Is cost-effective and quick:} Performance analysis is more useful if it is quick and computationally inexpensive so that developers can use it to iterate over heuristics. 
%
%
%\parab{Is widely applicable:} We want a technique that we can apply to a broad set of heuristics.

\begin{figure}[t!]
%\includegraphics*[width=3in]{figs/metaopt_workflow.png}
\includegraphics[width=\linewidth]{figs/metaopt_workflows.pdf}
\caption{{\metaopt}'s workflow involves four steps; (1) User encodes the heuristic as a convex or a feasibility problem~\secref{s:d:heur_form}, (2) {\metaopt} automatically detects alignment and applies necessary rewrites to transform the optimization to one-shot~\secref{s:d:rewrites}, (3) {\metaopt} automatically partitions the problem into smaller subproblems to achieve scalability~\secref{s:d:part}, (4) {\metaopt} runs one or more instances of the one-shot optimization on existing solvers~\cite{gurobi,Z3}.\label{f:metaopt_workflow}}
\end{figure}


\begin{table}[t!]
	\begin{footnotesize}
		\begin{tabular}{cc|cc}
			 {\bf Optimal} & {\bf Heur.} & {\bf Formulation} & {\bf Rewrite} \\\hline
			 \multirow{2}{*}{\sf OptMaxFlow} & {\pop} & Convex (Random)~\secref{ss:convexify:vbp_1} & KKT/P-D~\secref{s:d:rewrites} \\
			 & {\dempin} & Convex (Conditional)~\secref{ss:convexify:te_1} & KKT/P-D~\secref{s:d:rewrites}  \\
			 {VBP MILP} & {\ffd} & Non-convex MILP~\secref{ss:convexify:vbp_1} &  Feasibility \\\hline
		\end{tabular}
	\end{footnotesize}
	\caption{Overview of our three use-cases. We cover how to formulate the heuristics as optimizations in \secref{ss:convexify:vbp_1} and discuss their rewrites as constraints in~\secref{s:d:rewrites}. We write \ffd as a feasibility problem which does not need a rewrite. \label{t:metaopt_usecases}}
\end{table}


%\begin{table*}[t!]
%\begin{footnotesize}
%\begin{tabular}{cc|ccc|c}
%{\bf Heuristic} & {\bf Optimal} & {\bf Formulation} & {\bf Rewrite} & {\bf Partitioning} & {\bf Properties}\\\hline
%{\pop} or {{\sf POPMaxFlow}} & \multirow{2}{*}{\sf OptMaxFlow} & Random~\secref{ss:convexify:vbp_1} & Convex~\secref{s:d:rewrites} & \secref{s:d:part} & \\
%{\dempin} or {{\sf DemPinMaxFlow}} & & Conditional~\secref{ss:convexify:te_1} & Convex~\secref{s:d:rewrites} & \secref{s:d:part} & \\
%{\ffd} & {Vector bin packing MILP} & Sequential non-convex~\secref{ss:convexify:vbp_1} &  feasibility & - & \\\hline
%\end{tabular}
%\end{footnotesize}
%\caption{\label{t:metaopt_usecases}}
%\end{table*}
%
%\vspace{1mm}
%Existing solutions do not meet these goals. 
%Search techniques such as simulated annealing and hill climbing~\cite{hill_climbing,simulated_annealing} have the broadest applicability because they are {\em black boxes}. 
%These algorithms repeatedly select a new input, evaluate both the optimal and the heuristic on that input, and use the result to determine the next input to evaluate. 
%We have implemented several search techniques (see~\xref{appendix:black-box} for pseudocode and details). We find that these methods are slow in practice~(\secref{s:eval}): they ignore the inner workings of the heuristic and the problem (\eg the network topology), can converge to local optima, and lack optimality guarantees.
%
%


%If we could solve the problem in Eqn.~\ref{eqn:adversarial_outer} directly, we could produce optimal adversaries. 
%Our idea is to model the problem a Stackleberg equilibrium~\cite{sGames}.
%The outer (leader) problem in our model seeks inputs which maximize the difference between the optimal and the heuristic followers. 
%The inner (follower) problems are also optimizations that take variables of the outer problem (inputs $\mathcal{I}$) as constants and optimize internal variables~(e.g., flow %allocations in TE, ~\xref{s:background}). 

We model this problem as a two-level or meta optimization (hence \metaopt):
%A two-level optimization, as its name suggests, has an outer (leader) problem and inner (follower) sub-problems: the leader optimizes its objective subject to the followers' solutions and the followers solve their problems subject to the followers' variables,

{\small
	\vspace{-3mm}
	\begin{alignat}{3}
&		\arg\max_{\mathcal{I}}{\sf OPT}(\mathcal{I}) - {\sf Heuristic}(\mathcal{I}) && \quad\text{(leader problem)}\label{eq:metaopt_full_1} \nonumber\\
&		\mbox{s.t.} \quad {\mathcal{I} \in {\sf ConstrainedSet}} && \quad\text{(input constraints)}\nonumber\\
&		{\sf OPT}(\mathcal{I}) = \max_{\mathbf{f} \in \mathcal{F}}{\sf Opt\_Objective}(\mathbf{f},\mathcal{I})  && \quad\text{(optimal)} \nonumber\\
&		{\sf Heuristic}(\mathcal{I}) = \max_{\mathbf{f}' \in \mathcal{F}'} {\sf Heuristic\_Objective}(\mathbf{f}', \mathcal{I})&& \quad\text{(heuristic)} 
	\end{alignat}} 
	\vspace{-2mm}
	
where the {\em leader} or {\em outer} optimization maximizes the difference between the optimal and the heuristic problem and controls the input variable $\mathcal{I}$. This leader problem is subject to the {\sf OPT} and {\sf Heuristic} {\em follower} or {\em inner} problems which can only control the $\mathbf{f}$ and $\mathbf{f}'$ variables respectively (we use $\mathcal{F}$ and $\mathcal{F}'$ to model the set of values $\mathbf{f}$ and $\mathbf{f}'$ can take).

In this model the leader's objective conflicts with at least one of the followers. The leader wants to maximize {\sf OPT} and minimize {\sf Heuristic} to maximize the difference between them but this conflicts with the {\sf Heuristic} if {\sf OPT} and {\sf Heuristic} are maximization problems and with {\sf OPT} when they are minimizations~---~their {\em objectives are misaligned} with the leader. SMT~(\eg Z3~\cite{Z3}) or optimization~(\eg Gurobi~\cite{gurobi}) solvers cannot solve two-level optimizations with objective misalignment directly and its hard to find a work-around because the problem's semantics require we ensure the leader's objective takes priority (\ie the conflict in the two objectives does not cause the leader to get a lower objective).
 
%We cannot use
% SMT~(\eg Z3~\cite{Z3}) or optimization~(\eg Gurobi~\cite{gurobi}) solvers directly to solve this two-level optimization~\cite{bilevel_survey}. This is because the objective of the leader conflicts with the objective of one or more of the followers.
% We refer to this as {\em objective misalignment}: it happens when one or more of the followers (in our case the optimal and/or heuristic) are optimizations and maximize (or minimize) a function with variables that influence the outcome of an objective which the leader wants to minimize (or maximize)~---~the two objectives clash because one tries to maximize and the other minimize their objective and they share variables that influence each-other's outcome. The problem's semantics require we ensure the leader's objective takes priority (\ie the conflict in the two objectives does not cause the leader to get a lower objective) which makes the problem tricky.
 
% A somewhat secondary issue happens when the heuristic is itself an optimization. In these cases
% the {\em the objectives are not aligned} between the heuristic follower and the leader: the heuristic aims to maximize its own objective but the leader wants the heuristic to under perform so that it can maximize the gap~---~it wants to minimize the heuristic objective\footnote{The ${\sf OPT}$ follower's objective aligns with the outer leader's objective. If the outer problem was $\arg\max {\sf OPT} + {\sf Heuristic}$, i.e., a sum instead of a difference, the objectives would align.}. For some heuristics we can avoid this issue and write them as feasibility constraints.
 
  %Intuitively, there is a circular relationship between the leader and the follower. The leader needs to find inputs that maximize the gap between the optimal and the heuristic but has to wait for the outputs of those two problems to do so. On the flip side, the followers need the leader's output to compute their own solutions.
 
The second issue is that the inputs, which for the individual followers were constants, now become variables in the two-level optimization. 
This can cause non-linearities because what used to be a constant multiplying a variable in the follower now becomes a variable (for the outer problem) that multiplies another variable (for the follower).

\vspace{0.05in}
{\metaopt} is a {\em white-box} approach that solves these problems. 
It uses rewrites that convert the two-level optimization in Eqn.~\ref{eq:metaopt_full_1} into a one-shot optimization. 
We convert the misaligned followers into feasibility problems: we convert them into a set of constraints where any input that satisfies these constraints matches the solution of the original problem. 
This approach preserves the structure of the problem (it optimizes the follower's objectives in a way that prioritizes the leader's objective). The optimization chooses the shared variables that maximize the leader's objective and the constraints (which we derive from the rewrites) ensure we also optimize the follower's objective subject to those choices. 

\begin{figure}[t!]
	\begin{center}
		\begin{tikzpicture}[->,>=stealth]
		\node[state,
		text width=3.3cm] (A) 
		{\begin{tabular}{l}
			\textbf{min}$_{w, \ell}$ $\big( w^2 + \ell^2 \big)$\\[.5em]
			$2 \cdot (w + \ell) \geq P$ \\
			$P \geq 0$ \\
			\end{tabular}};
		
		\node[state,
		text width=3.2cm,
		right of=A,
		yshift = -1.1cm,
		node distance=4.8cm,
		anchor=center] (B)
		{%
			{\begin{tabular}{l}
				\textbf{solve} for $w, \ell, \lambda$\\[.5em]
				$2 (w + \ell) \geq P$ \\
				$P \geq 0$ \\
				$\lambda \geq 0$ \\
				$2w - 2\lambda = 0$ \\
				$2\ell - 2\lambda = 0$ \\
				%		$\big( \lambda = 0 \big)$ or \\
				%		$~~~~\big( w + \ell - \frac{P}{2} = 0 \big)$ \\
				\fcolorbox{myp}{myp}{$\lambda\big( w + \ell - \frac{P}{2} \big) = 0$}\\
				\end{tabular}}
		};
		
		\node[state,
		below of=A,
		yshift=-1.4cm,
		fill={rgb,255:red,222;green,226;blue,255},
		%		fill=cyan!20,
		anchor=center,
		text width=3.6cm] (C) 
		{%
			{\renewcommand{\arraystretch}{1.3}
				%	\begin{tabular}{p{2.6cm}}
				%		$w = \frac{P}{4}$, $\ell = \frac{P}{4}$  \\ \hdashline
				%		$\lambda = \frac{P}{4}$ \\
				%	\end{tabular}
				\begin{tabular}{p{1.8cm} p{1.2cm}}
				$w = \ell = \frac{P}{4}$  & $\lambda = \frac{P}{4}$ \\
				\end{tabular}}
		};
		
		\path (A) 	edge[bend left=20]  node[anchor=south,above]{KKT}
		node[anchor=north,below]{encode} (B)
		(A)     	edge[bend right=20] node[anchor=south,right]{optimize}   (C)
		(B)       	edge[bend left=20]  node[anchor=south,above]{solve}      (C);
		
		\end{tikzpicture}
	\end{center}
	\caption{{\label{f:eg_conversion_1} Example rewrite using KKT. The inner variables are the width $w$ and length $\ell$ of a rectangle. The right shows the feasibility problem using the KKT theorem. Equations with $\lambda$ variables correspond to first order derivatives of inequality constraints in the original problem. The perimeter $P$ is a variable to the outer optimization but is treated as a constant in the inner problem.}}
\end{figure}

%; some lead to consequent challenges which we solve and have different scopes of applicability.

Users have to formulate the follower problems (the optimal and the heuristic in our case) as a convex optimization or a feasibility problem (feasibility problems do not have an objective and search for any input that satisfies all the constraints). Followers that are feasibility problems need not be convex
(we still need commodity solvers to support them; Gurobi~\cite{gurobi} solves non-convex quadratic constraints and objectives, including bilinear and quadratic equality constraints, linear, non-linear, or mixed-integer problems).

We build a system to make it easier to encode heuristics in this way. We provide various helper-functions in \metaopt which allow users to automatically convert the patterns (e.g. if conditions; weight updates; and others) that commonly appear in networking and systems heuristics into their convex form. Due to space constraints we show the full list of these helper-functions and how they help encode the heuristics we analyzed in the appendix (see~\S\ref{}). We show examples of how to write many diverse heuristics as convex optimization problems in~\S\ref{} and show how to do so through {\metaopt}'s helper functions in~\S\ref{}.
\behnaz{fill blank.}

%We show examples of how to do this and
%translate the conditional and random steps in heuristics such as {\dempin} and {\pop} into optimizations.
%We show a novel rewrite of a non-convex heuristic (\ffd) for vector bin packing (VBP) as a feasibility problem. 
%We also show how to model and update weights and priorities.

Users also need to pick which rewrite they want to use. 
\metaopt automatically handles everything else~---~it re-writes the follower if it needs to. %Feasibility problems allow \metaopt to convert the two-level optimization into a single-shot one without a rewrite (we no longer have a mismatch with the leader's objective because the heuristic no longer has an objective).


%We formulate the {\ffd} heuristic~\cite{VBP-Heuristics} to the vector bin packing problem~\cite{vbp-nphard}, as a feasiblity problem over a set of constraints where we do not have an objective term (feasibility problems search for any input that satisfies all constraints).
%To our knowledge, this formulation of FFD is novel.
%We discuss heuristic formulations in~\xref{s:d:heur_form}.

To allow \metaopt to scale to large instances we introduce a new partitioning technique~(\xref{s:d:part}). This technique allows us to convert the larger \metaopt problem into smaller sub-problems, which we can solve in parallel. We discuss how to extend {\metaopt} in~\xref{s:d:ext}~(\eg to find adversarial inputs for a combination of heuristics). 




\vspace{0.05in}
%\parab{Summary.} We design and build \metaopt, a system to analyze hueristics.
%{\metaopt} converts the two-level optimization problem in Eqn.~\ref{eqn:adversarial_outer} to one-level optimizations that commodity solvers can solve.
 \autoref{f:metaopt_workflow} shows how to run \metaopt.
%We describe how \metaopt rewrites heuristics in \secref{s:d:rewrites} and 
%preview how we can formulate the heuristics into \metaopt in \secref{ss:convexify:vbp_1}.
% We use partitioning on \pop and \dempin (\secref{s:d:part}). We may not need to partition small problems but it is
% crucial when we analyze TE heuristics on large topologies. 
\metaopt is optimal when we can write the heuristic as a convex optimization or a feasibility problem: it provably finds the adversarial inputs that produce the worst-case gap. 
{\metaopt}'s ability to scale depends on the optimal problem, how we formulate the heuristic, and what re-write we use: how many integer variables we add when we formulate the heuristic or when we rewrite it determine {\metaopt}'s speed. \metaopt can scale to large problem instances through our novel partitioning solution. We may not need to partition small problems but it is
crucial when we analyze TE heuristics on large topologies. 

%Overall it is not fully clear to us yet when \metaopt does not apply~---that is, when it is not optimal or fast---~because it depends on how we formulate the heuristic and the optimal problem. We show results on three substantial use-cases and believe that the techniques herein have broader value.

%\input{../SIGCOMM-MetaOpt/texfiles/design_rewrite}
%\input{../SIGCOMM-MetaOpt/texfiles/design_heuristic_formulations}
%\input{../SIGCOMM-MetaOpt/texfiles/design_partitioning}
%\input{../SIGCOMM-MetaOpt/texfiles/design_ext}


==> texfiles/design_ext.tex <==
\subsection{Extensions}
\label{s:d:ext}


\parab{Scaling using solver-specific knobs:} We can speedup \metaopt further because commodity solvers: (1) find a near-optimal solution quickly but take a long time to prove optimality or improve on this initial solution; (2) periodically estimate the optimality gap and report progress. We track this progress over fixed timesteps and when the incremental progress dips below a threshold (say $0.5\%$), we stop the solver early and use the best solution. Gurobi reports this progress through the primal-dual gap~\cite{boyd_co}. For solvers, such as Z3~\cite{Z3}, which do not report incremental progress, we progressively ask for inputs with a higher gap.  

\parab{Find inputs with bounded distance from a goalpost.} Users can search for adversaries within a certain {\em distance} from a {\em goalpost} (using ${\sf ConstrainedSet}$ in~\eqnref{eq:metaopt_full_1}). This helps understand how far inputs can deviate from the norm before the heuristic breaks; to find an appropriate threshold for switching heuristics; or to apply other remedies. Users can leave some inputs unconstrained.

\parab{Compare input sets.} \metaopt can analyze the {\em types} of input a heuristic is sensitive to. For example, it can output the adversarial gap when the inputs are sparse. To compare input sets, users must specify each set as a ${\sf ConstrainedSet}$ in~\eqnref{eq:metaopt_full_1}. Each constraint is in terms of $g(\mathcal{I}) \geq f(\mathcal{I})$ or $g(\mathcal{I}) = f(\mathcal{I})$ where $f$ and $g$ are functions of the input $\mathcal{I}$.

\parab{Analyze a combination of heuristics.} Users can combine different heuristics~---~which have non-overlapping sets of adversaries~---~so each covers the weakness of the other and to reduce the optimality gap. To use \metaopt to analyze this heuristic we replace ${\sf Heuristic}(\mathcal{I})$ in the objective of~\eqnref{eq:metaopt_full_1} with $\max_{h}({\sf Heuristic}_{h}(\mathcal{I}))$ so that the follower returns the solution of the best heuristic for each input. To transform the optimization into a single-level optimization, \metaopt needs to rewrite each of the heuristics.


%
%Different heuristics that solve the same problem have different adversarial patterns: we can potentially reduce the optimality gap of these heuristics by combining them. Operators can use \metaopt to analyze such combinations and understand the resulting heuristic. We can replace ${\sf Heuristic}(\mathcal{I})$ in the objective of~\eqnref{eq:metaopt_full} with $\max_{h}({\sf Heuristic}_{h}(\mathcal{I}))$ so that the follower returns the solution of the best heuristic for each input:
%
%\vspace*{-2ex}
%{\small
%	\begin{alignat}{3}
%%		\label{eq:metaopt_multiple_heuristics} 
%		\mbox{\sf AdversarialInput}() \triangleq & \arg\max_{\mathcal{I}}\,\,{\sf OPT}(\mathcal{I}) - \max_{h}({\sf Heuristic}_{h}(\mathcal{I}))& \nonumber
%	\end{alignat}
%}
%%

\parab{Improve heuristics through strategic changes.} Insights from \metaopt can help improve the heuristic (see~\secref{s:eval:te}).

%Users can study the adversarial inputs from \metaopt to understand why a heuristic underperforms. Understanding these weaknesses can help them apply fixes to reduce the optimality gap. We show how to do this for \dempin in~\secref{s:eval:te}.
%\pooria{fill this after finishing evaluation.}


\parab{Compare Heuristics.} \metaopt can compare heuristics directly (instead of comparing with \opt): 

\vspace*{-2ex}
{\small
	\begin{equation}
		\mbox{\sf AdversarialInput}() \triangleq \arg\max_{\mathcal{I}}\,\,{\sf Heuristic}_{1}(\mathcal{I}) - {\sf Heuristic}_{2}(\mathcal{I}) \nonumber
\end{equation}}

\parab{Identify Suitable Inputs.} \metaopt can identify inputs for which the heuristic performs well. To do this we need to change the leader objective:

%\metaopt can also identify ideal inputs for a given heuristic. Users can achieve this by altering the objective of the leader in~\eqnref{eq:metaopt_full_1}, so it minimizes the gap between \opt and \heur instead of maximizing it. 

\vspace*{-2ex}
{\small
	\begin{equation}
		\mbox{\sf SuitableInput}() \triangleq \arg\min_{\mathcal{I}}\,\,{\sf OPT}(\mathcal{I}) - {\sf Heuristic}(\mathcal{I}) \nonumber
\end{equation}}
%
Users should restrict inputs using ${\sf ConstrainedSet}()$ to ensure the answers are meaningful and relevant otherwise the optimization may lead to trivial answers~---~any TE heuristic is optimal when all demands are zero.




==> texfiles/design_heuristic_formulations.tex <==

\subsection{How we model heuristics in \metaopt}
\label{s:d:heur_form}
%We next provide examples on how to formulate heuristics.
We describe a few examples to show how users can model a diverse set of heuristics in \metaopt. We focus our discussion in this section on how to model these heuristics as convex or feasibility problems. Users can use the helper-functions in \metaopt(see~\S\ref{}) to avoid manually writing the constraints we describe here (we present them for technical completeness). We only discuss a few heuristics here because of space constraints but refer the user to~\S\ref{} for other examples.
\behnaz{add ref.}



\label{ss:convexify:te_1}
\parab{Traffic Engineering Heuristics} TE optimizations and heuristics take a set of nodes, capacitated edges, demands, and 
a set of (pre-determined) paths per demand as input. The output is a set of feasible flows that meet demand and capacity constraints: ${\sf FeasibleFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P})$ (see \secref{sec::appendix-flow}). \autoref{t:notation} describes our notation. The optimal algorithm solves a multi-commodity flow problem. Typical objectives maximize the total flow~\cite{ncflow}, utility~\cite{bwe} or consider max-min fairness~\cite{swan,b4}. Those that maximize total flow:
%${\sf OptMaxFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P})$ in~\S\ref{sec::appendix-flow}.

\vspace{-3mm}
{\footnotesize
	\begin{align}
	\label{eq:max_flow}
	\mbox{\sf OptMaxFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) \triangleq & \arg\max_{\mathbf{f}}\sum_{k \in \mathcal{D}} f_k\\
	\mbox{s.t.} \quad & \mathbf{f} \in {\sf FeasibleFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}).\nonumber
	\end{align}} 
%The number of variables and constraints in this problem grows as $|\mathcal{D}| + |\mathcal{E}|$ where $|\mathcal{D}|$ is quadratic in $|\mathcal{V}|$. Prior work shows that the optimal algorithm can takes tens of minutes for large network sizes and is impractical to use on networks with dynamic demands~\cite{ncflow}. 

\begin{table}[t!]
	\centering
	{\footnotesize
		\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{l p{2.3in}}
			{\bf Term} & {\bf Meaning}\\
			\hline
			\hline
			$\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}$ & Sets of nodes, edges, demands, and paths \\
			\hline
			$c_e, p$ & {$c_e$: capacity of edge $e \in \mathcal{E}$,  path $p$: set of edges}\\\hline
			$(s_k, t_k, d_k)$ & {The $k$th element in $\mathcal{D}$ has source and target nodes~($s_k, t_k \in \mathcal{V}$) and a volume~($d_k \geq 0$)}\\\hline
			$\mathbf{f}, f_k^p$ & {$\mathbf{f}$: flow assignment vector with elements $f_k$ \newline $f_k^p$: flow for demand $k$ on path $p$} \\
			
		\end{tabular}
	}
	\caption{Notation for multi-commodity flow problems.\label{t:notation}} 
	%	\vspace{-3mm}
\end{table}


We show how to rewrite two heuristics from TE~---~conditional and randomized.



\parae{Demand Pinning.} We can pose {\dempin} as an optimization with constraints that route demands below the threshold on the shortest paths:
%\vspace{-4mm}

\begin{footnotesize}
	\vspace{-3mm}
	\begin{alignat}{3}
	\label{eq:dp_max_flow}
	\mbox{\sf DemPinMaxFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) \triangleq & \arg\max_{\mathbf{f}}\sum_{k \in \mathcal{D}} f_k & \\
	\mbox{s.t.} \quad & \mathbf{f} \in {\sf FeasibleFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) &\nonumber \\
	& \mathbf{f} \in {\sf DemandPinning}(\mathcal{D}, \mathcal{P}) &\nonumber
	\end{alignat}
	\vspace{-2mm}
\end{footnotesize}

\dempin has a conditional or {\em if} clause: if a demand is smaller than the threshold $T_d$, then route it over its shortest path; otherwise, use the optimal algorithm to route it. We discuss a simple method to encode this heuristic directly in~\secref{sec:dempin_bigM}. We use this method in our helper-function that encodes conditional constraints (see~\S\ref{}). We also have a method that uses the quantization points in the primal-dual rewrite to encode the constraints in demand pinning:
%
{\small
	\begin{eqnarray}
		f_k^{\widehat{p}_k} \geq \sum_{q=1}^{Q} \mathbb{1}[L_{q} \leq T_d] L_{q}x^{k}_{q}, \,\,\, \forall k \in \mathcal{D}. \label{eqn:dempin_pdq}
	\end{eqnarray}
}
%
The $\{0, L_1, \dots,L_Q\}$ are the quantas and $x^k_q$'s are binary variables that pick which quanta is active for demand $k$ (for which $\widehat{p}_k$ is the shortest path).  The term $\mathbb{1}[L_{q} \leq T_d]$ is a no-op at runtime: it shows which terms exist in the sum. 

We defined quantization such that $d_k = \sum_q L_q x^k_q$. Thus, if the demand $d_k$ is no larger than the threshold $T_d$,~\eqnref{eqn:dempin_pdq} ensures its allocation on the shortest path equals the value of its demand.\footnote{When $d_k \leq T_d$,~\eqnref{eqn:dempin_pdq} effectively becomes $f_k^{\widehat{p_k}} \geq d_k$. In the converse case, \ie $d_k > T_d$, Eqn.~\ref{eqn:dempin_pdq} becomes $f_k^{\widehat{p}_k} \geq 0$, a no-op.} \metaopt analyzes \dempin faster when we model it this way compared to the simpler model (see~\secref{sec:dempin_bigM}) because it introduces fewer new variables.
Users can model {\em if cluases} in their heuristics with the same technique.
%When the value of demand $d_k$ is below the threshold $T_d$, one of the quantization levels below $T_d$ is in effect (\ie $x^k_j = 1$). 
%To ensure such demands follow their default shortest path $\widehat{p}_k$, we use these constraints to lower bound the related flow variables.
%We linearize the $L_j x_j^k$ terms in Eqn.~\ref{eqn:dempin_pdq} using big-M as we did in the quantized p-d rewrite.
%\pooria{I removed We linearize because the term is linear. $L_j$s are constant.



% We show in a more direct encoding of the conditional which 
% These constraints effectively mimic the big-$M$ model from standard optimization theory~\cite{boyd_co} but result in better solver performance in practice (we show the big-$M$ formulation of {\dempin} in appendix~\S\ref{sec:dempin_bigM}~---~ we use it for our KKT encoding where the demands are not quantized).

\parab{Partitioned Optimization Problems.} {\pop} is the union of solutions to disjoint linear optimizations and is convex. \pop divides the problem into $c$ partitions so that each sub-problem is  $\sim 1/c$ the size of the original.


%If $|\mathcal{D}|$ is much larger than $|\mathcal{E}|$ and \pop uses $c$ partitions, each sub-problem is $\sim 1/c$ the size of the original and \pop will offer a substantial speedup~---~LP solver times are super-linear in problem sizes~\cite{boyd_co}. 


%
%\vspace{-1mm}

%\begin{footnotesize}
%	%\vspace{-5mm}
%	\begin{equation}
%	\label{eq:pop_max_flow}
%	\mbox{\sf POPMaxFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) \triangleq  \bigcup_{\mbox{part. c}} \mbox{\sf OptMaxFlow}(\mathcal{V}, \mathcal{E}_c, \mathcal{D}_c, \mathcal{P}),
%	\end{equation}
%	%\vspace{-2mm}
%\end{footnotesize}
%
%\cut{
%	\begin{footnotesize}
%		\vspace{-5mm}
%		\begin{alignat}{2}
%		\label{eq:pop_max_flow}
%		\mbox{\sf POPMaxFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) &\triangleq  \\
%		& \bigcup_{\mbox{part. c}} \mbox{\sf OptMaxFlow}(\mathcal{V}, \mathcal{E}_c, \mathcal{D}_c, \mathcal{P}), \nonumber
%		\end{alignat}
%		\vspace{-2mm}
%	\end{footnotesize}
%}
%
%\noindent where $\cup$ is the vector union, the per-partition demands $\mathcal{D}_c$ are disjoint subsets of the actual demands drawn uniformly at random, and the per-partition edge list $\mathcal{E}_c$ matches the original edges but with proportionally smaller capacity.



{\pop} is hard to model.
{\metaopt} needs a deterministic representation of the heuristic as its input but {\pop} uses random partitions which makes ${\sf POP}(\mathcal{I})$ a random variable in the leader problem.
Na\"ively, if we only consider a specific instance of each random variable (\eg for one instance of randomly assigning demands to partitions), it will overfit to that instance and not reflect {\pop}'s true behavior. 

We use the {\em expected value} or {\em tail percentile} of the gap from multiple random trials. To compute the average, we replace \heur in \eqnref{eq:metaopt_full_1} with its expected value and approximate the expectation through empirical averages over a few randomly generated partitions (see \secref{s:eval:te}). To find the tail, we use a sorting network~\cite{sorting_net_1,pretium} to compute the desired percentile across multiple random trials. 

% Finally, we discuss in~\xref{s:appendix:pop}, how to encode an advanced version of {\pop} which splits large demands across multiple partitions instead of assigning each demand to one partition.
In addition, we encode an advanced version of \pop in~\xref{s:appendix:pop} that splits large demands across multiple partitions instead of assigning each demand to one partition. 

\label{ss:convexify:vbp_1}
\parab{Vector Bin Packing Heuristics} %Production deployments use vector bin packing ({\vbp}) in multiple domains to efficiently allocate resources~\cite{protean,tetris,synergy,yarn_vbp,jobpacking}. We consider a simple offline version: given a set of balls and bins with specific sizes and multiple dimensions~(\eg memory, CPU, GPU~\cite{drf,borg,pond}), it tries to pack balls into the fewest number of bins.
We can pose the optimal form of VBP as a MILP which is non-convex and known to be APX-hard~\cite{vbp-nphard}. 

It is easy to see that \ffd is not convex and so the rewrites in~\xref{s:d:rewrites} do not apply. \ffd is also hard because it is iterative and chooses the first fitting bin in each iteration.


We introduce a novel and exact formulation for \ffd as a feasibility problem. The solution to the feasibility problem matches exactly how \ffd assigns balls to bins. To save space we defer the details to~\xref{a:s:vbp_new}. 

We do not need rewrites for our model of \ffd: we directly encode it as a feasibility problem. But the overall optimization \metaopt has to solve is an MILP since both the optimal and the \ffd are MILP.

%\metaopt analyzes large instances of \ffd within hours.


This use-case shows \metaopt applies to even complex non-convex scenarios. In fact, the worst-case adversarial inputs that we discover when we apply \metaopt on \ffd match or supercede the decades of work on theoretical analysis of \ffd-style heuristics~\cite{VBP-Heuristics,ffd-1d-1973,ffd-1d-1985,ffd-1d-1991,ffd-1d-tight,multi-bp-survery}.

%\behnaz{@Pooria, cite missing here}
These heuristics show how users can analyze heuristics that involve conditional constraints; randomness; and non-convexity in \metaopt. We also model SP-PIFO~\cite{sp-pifo} in~\S\ref{} to describe how users can model priority updates and priority-based decisions. We show how they can model these heuristics through the \metaopt helper functions in~\S\ref{}.



==> texfiles/design_rewrite.tex <==


\begin{figure}[t!]
\begin{center}
	\begin{tikzpicture}[->,>=stealth]
		\node[state, text width=2.9cm, label=Primal-dual] (A)
		{
			{
				\small
				\begin{tabular}{l}
					\textbf{solve} for $w, \ell, \lambda$\\[.5em]
					{$2 (w + \ell) \geq P$} \\
					{$\lambda \geq 0$} \\
					$P \geq 0$ \\
					\fcolorbox{myp}{myp}{$P \lambda -2 \lambda^2 = w^2 + \ell^2$}
				\end{tabular}
			}
		};
		
		\node[state,
		text width=3.6cm,
		right of=A,
		% yshift = -0.3cm,
%		align=left,
		node distance=5.05cm,
		anchor=center, label=Quantized Primal-dual] (B)
		{%
			{
				\small
				\begin{tabular}{l}
					\textbf{solve} for $w, \ell, \lambda$\\[.5em]
					{$2 (w + \ell) \geq P$} \\
					{$\lambda \geq 0$} \\
					\fcolorbox{myp}{myp}{$x_j \in \{0,1\} \sum_{j=1}^{Q} x_j \leq 1$}\\
					\fcolorbox{myp}{myp}{$\sum\limits_{j=1}^{Q}{L_j z_j} -2 \lambda^2 = w^2 + \ell^2$}\\
					\fcolorbox{myp}{myp}{$z_j = \lambda x_j \,\, \forall j \in \{1,\dots,Q\}$}
				\end{tabular}
			}
		};
		% \draw [-stealth](2.1,-1) -- (3.7,-1);
		
		% \path (A) 	edge[yshift=-0.5em]  node[anchor=south,above]{$P = L_1x_1$} node[anchor=north,below]{} (B);
		% (A)     	edge[bend right=20] node[anchor=south,right]{optimize}   (C)
		% (B)       	edge[bend left=20]  node[anchor=south,above]{solve}      (C);
		\begin{scope}[transform canvas={yshift=-3em}]
			\draw [->] (A) -- node[anchor=north,above] {{\footnotesize $P = \sum\limits_{j=1}^{Q}{L_j x_j}$}} (B);
		\end{scope}
	\end{tikzpicture}
\end{center}
\caption{Left shows rewrite through primal-dual theorem. The p-d rewrite has fewer constraints and different multiplicative terms~($\lambda P$ in the bottom equation versus $\lambda (w + \ell - \frac{P}{2})$ in the KKT rewrite) and a quadratic constraint (in red) due to the quadratic objective of the original problem. On the right, we show how we quantize the parameters in the outer problem~($P$ in this case) so the p-d-q rewrite no longer has any multiplicative terms. The values $L$ are constants and $x_j$ are indicator variables.\label{f:pd_conversion_1}}
\end{figure}



\subsection{How we rewrite convex heuristics}%Rewriting convex heuristics as feasibility problems}
\label{s:d:rewrites}


We need to rewrite the misaligned followers in Eqn.~\ref{eq:metaopt_full_1} into a feasibility problem to convert the two-level optimization into a single-shot one~---~for aligned followers, we can just port their constraints directly into the outer problem.

\behnaz{@Pooria, can you add cites please?}
Prior work in domains such as XXX solve multi-level optimizations based on the Karush–Kuhn–Tucker (KKT) and Primal-Dual theorems~\cite{}. {\metaopt}'s rewrites are also based on these theorems. We use a running example (one which maximizes the diagonal length of a rectangle such that its perimeter is greater than $P$) to describe them. This example (\autoref{f:eg_conversion_1}-\ref{f:pd_conversion_1}) is not related to distributed systems or even heuristics but it is simple and helps us explain the theory without having to introduce a lot of extra notation.
%\autoref{f:eg_conversion_1} describes the Karush–Kuhn–Tucker (KKT) theorem and~\autoref{f:pd_conversion_1} describes strong duality.~\autoref{f:pd_conversion_1} also describes a novel quantized variant of strong duality which we introduce to scale {\metaopt}.

\parab{KKT rewrite.} The KKT theorem allows us to convert convex optimizations that have at least one strictly feasible point~\cite{boyd_co} into feasibility problems. The theorem states any point that solves the new problem matches the solution of the original. 






% Based on the $KKT$ theorem~\cite{boyd_co}, this rewrite can convert any convex optimization with at least one strictly feasible point, into a set of feasibility constraints. \figref{f:eg_conversion} illustrates this rewrite. In this example, the original optimization finds the rectangle with the longest diameter ($w^2 + l^2$) where the perimeter is greater than some positive {\em constant} value $P$. The KKT rewrite produces a set of feasibility constraints (\figref{f:eg_conversion}). When a convex optimization has at least one strictly feasible point (Slater's condition~\cite{boyd_co}), this rewrite is \textit{exact}~---~a feasible solution to the rewrite is an optimal solution to the original problem.

\parab{Primal-dual rewrite.} We can also use the strong duality theorem~---~any feasible point of a convex problem is optimal iff the primal objective at that point is the same as the dual~---~to construct an equivalent form of the problem. 

The primal dual introduces more complex constraints compared to KKT and although solvers such as Gurobi~\cite{gurobi} support it, we find it takes much longer to solve. Both of these approaches in their current form do not scale to the types of heuristics we use in sytems and networking. This is primarily because they introduce multiplicative terms (\autoref{f:eg_conversion_1} and~\autoref{f:pd_conversion_1}). Commodity solvers support such constraints~---~\eg special ordered sets (SOS) in Gurobi~\cite{gurobi} or disjunctions in Z3~\cite{Z3} (this is why prior work which solve two-level optimizations has not had to address this issue). However, these constraints slow down the solvers~---~the number of constraints with multiplications (and not the overall size of the problem) dictates the latency of the solver. We introduce a novel, quantized, version of the Primal-Dual re-write that also leverages the KKT theorem to address this issue.

 

%This rewrite has fewer constraints compared to KKT one; has different multiplicative terms; and has a quadratic constraint that comes from the quadratic objective in the primal (\autoref{f:pd_conversion_1}). 

%This rewrite has more complex constraints compared to KKT.% The KKT constraints encode complimentary slackness conditions and multiply two linear terms but reduce to SOS constraints (at least one of the linear terms must be zero). 
%Even though Gurobi~\cite{gurobi} supports the primal-dual rewrite, we do not have a similar reduction for its constraints and in practice we find it takes much longer to solve.


% Every (primal) optimization has a corresponding dual. This rewrite technique relies on a well-known relationship between the two: the strong duality theorem~\cite{boyd_co} which states that any feasible point of a convex problem is optimal if and only if the primal objective at that point is the same as the dual objectives. The primal-dual rewrite converts a convex optimization into a set of feasibility constraints that include: the feasibility constraints of the primal (green background in \figref{f:pd_conversion}), the feasibility constraints of the dual (blue background), and a constraint that encodes the strong duality theorem~---~the primal objective has to match the dual objective (light red background). The primal-dual rewrite is also exact.

\parab{Quantized primal-dual rewrite.} We convert the primal-dual rewrite into an easier problem to scale it. We quantize and replace some input variables with the sum of constants and integer variables. These new terms convert the original multiplicative terms into {\em different} multiplicative terms which multiply binary variables with a linear term. This conversion allows us to linearize the multiplicative terms easily through the well-known big-$M$ approach from optimization literature~\cite{boyd_co}, which commodity solvers (\eg~\cite{gurobi}) support and solve more quickly.

We show this approach end-to-end through our earlier example. We replace the input $P$ with $\sum_{j=1}^{Q} L_j x_j$ where $L_j$ are constants we choose a priori and $x_j$ are binary variables. We require $\sum_j x_j \leq 1$. This means the outer problem has to pick one of the $Q+1$ values $0, L_1, \ldots L_Q$ for $P$. We only need to quantize the leader's variables that appear in the multiplicative terms in the primal-dual rewrite. These variables only appear in the (misaligned) follower's constraints.

%The multiplicative terms in the primal-dual rewrite only result from the leader's variables that appear in the (misaligned) follower's constraints. These are the only variables we have to quantize.
%Notice quantization also causes multiplicative terms~---~ones that multiply binary variables with a %linear term. We can linearize these terms using the well-known big-$M$ approach from optimization literature~\cite{boyd_co}, which commodity solvers (\eg~\cite{gurobi}) support. 

%The optimization problem we write as a result of this quantized primal-dual rewrite is solved much more quickly.

Two challenges remain: (a) how to pick the number of quanta; and (b) which quanta to pick (\eg which values for $L_j$). 
More quanta leads to more integer variables which slow down the solver. But fewer quanta leads to poor-quality adversaries because we now constrain the input variables to only a few pre-selected values.

Because the quantized primal-dual rewrite is much faster to solve than the other rewrites, we can sweep multiple quanta choices and pick the best. 
We recommend using the exact KKT rewrite on smaller problem instances to find good candidates and also present an empirical observation:
adversarial inputs occur at so-called extreme points. 
For example, the worst-case demands have values of either $0$ or the maximum possible in the \pop heuristic\footnote{For {\dempin}, the worst-case demands take values of $0$, the demand pinning threshold $T_d$, or the maximum possible demand.}. We do not fully know the reason; we conjecture the intuition is similar to the intuition behind the simplex theorem~\cite{bertsimasLinOptBook}. 
  
We will evaluate how these rewrites impact the problem size and investigate the approximation gap the quantized primal-dual rewrite introduces in section \xref{s:eval}. We find the quantized primal-dual rewrite is much faster than the others and leads to higher quality adversarial inputs on the use-cases we examined. But it is approximate and it is not guaranteed to find the worst-case inputs. We use it as {\metaopt}'s default rewrite unless we state otherwise.


==> texfiles/eval.tex <==
%\vspace{-0.7mm}
\section{Evaluation}
\label{s:eval}

%We described different ways \metaopt can help users analyze performance of their heuristics in~\S\ref{s:background}. 
%We next evaluate \metaopt further (to save space we do not repeat the results in~\S\ref{s:background}).
We demonstrate the generality of \metaopt by applying it to vector bin packing, traffic engineering and packet scheduling heuristics. We show how \metaopt helped us quantify and understand the performance gaps of heuristics, prove theoretical properties, and improve the performance gap if possible.

\parab{Implementation.} Our prototype is in C\# and uses Gurobi v9.5.2~\cite{gurobi}; we also have a port that uses Z3~\cite{Z3}.
To partition the graph, we adapt previous code~\cite{ncflow,communities_code} for spectral clustering~\cite{njw} and FM partitioning~\cite{louvain_method,communities}
and report results for different cluster numbers and clustering techniques.


\subsection{Heuristics for Vector Bin Packing}
\label{s:eval:vbp}

%We use \metaopt and analyze the \ffd heuristic in VBP in both the single and two dimensional case (1d-\ffd and 2d-\ffd respectively). Our results reproduce the existing optimality gap for 1d-\ffd and discover a new one for 2d-\ffd. The adversarial inputs \metaopt generated helped us arrive at a new theorem that proves this bound for 2d-\ffd.


We use \metaopt in vector bin packing (\vbp) to: (1)~recover an existing theoretical suboptimality bound for \ffd in one dimension (1d-\ffd), (2)~unveil unknown optimality bounds under realistic settings, and (3)~show a novel theoretical bound for \ffd in two dimensions (2d-\ffd).

\parab{Reproducing the existing bound for 1d-\ffd.} 
After decades of theoretical studies on 1d-\ffd~\cite{ffd-1d-tight,ffd-1d-1973,ffd-1d-1985,ffd-1d-1991},
the work in~\cite{ffd-1d-tight} established the tight bound $\ffd(\mathcal{I}) \leq \frac{11}{9} \opt(\mathcal{I}) + \frac{6}{9}$ for any $\mathcal{I}$. 
To prove the tightness, the authors craft a careful example where $\opt(\mathcal{I}) = 6$ bins and $\ffd(\mathcal{I})=8$. 
\metaopt found the same example when we constrainted its inputs $\opt(\mathcal{I}) = 6$ and proved \ffd needs $8$ bins in the worst-case.
%\behnaz{what if you dont add the constraint?}
%We ran \metaopt to find the worst-case input $\mathcal{I}$ for 1d-{\ffd} among all inputs where $\opt(\mathcal{I}) = 6$ bins.
%\metaopt proved \ffd needs at most $8$ bins and, interestingly, returned the same $\mathcal{I}$ crafted by the authors of~\cite{ffd-1d-tight}.

\parab{Finding optimality gaps for realistic settings.} 
The proof in~\cite{ffd-1d-tight} assumes: (1) $\mathcal{I}$ can have an unlimited number of balls; and (2) the balls in $\mathcal{I}$ can have any size (even 0.00001$cm^3$!). This is not always the case in practice: \eg when packing jobs (balls) in machines (bins)~\cite{jobpacking}, we often know \textit{apriori} an upper bound on the number of jobs or the quantization levels for resource requirements. We can incorporate such constraints and ensure \metaopt finds practical adversarial inputs. For example, we constrain the number of balls and the ball sizes \metaopt finds (\autoref{tab:1d-ffd}): not only does it find adversarial inputs that meet these constraints but it also finds adversarial inputs that produce a slightly tighter bound compared to~\cite{ffd-1d-tight}. 

%This may often be unrealistic: \eg when we schedule jobs (balls) to machines (bins)~\cite{jobpacking} we might know \textit{a priori} an upper bound on the number of jobs or even quantization levels on the resources that these jobs will require. We expect the theoretical bound in~\cite{ffd-1d-tight} is loose under this constrained scenario but this is not amenable to theoretical analysis.
%Under this constrained scenario, we expect the theoretical bound in~\cite{ffd-1d-tight} to be loose, but this setting is not amenable to a theoretical analysis.
%\metaopt seamlessly incorporate such constraints and can find worst-case inputs given constraints. The theoretical bound in~\cite{ffd-1d-tight} predicts $\ffd(\mathcal{I}) \leq 8$ bins for all cases in~\autoref{tab:1d-ffd}. As the table shows, \metaopt shows that the worst possible outcome for \ffd is better in some cases.

% We see we can still achieve this worst case when we constrain the maximum number of balls to $20$ and set the granularity of ball sizes to $0.01$ (the bins have unit capacity). But if we constrain the granularity to $0.05$ or if we reduce the number of balls to $14$ \metaopt reveals the worst possible outcome is actually $\ffd(\mathcal{I}) = 7$.

\begin{table}[t!]
	\centering
	{\footnotesize
		\begin{tabular}{c c c}
			max \#balls & ball size granularity & {\sf{FFD}}($\mathcal{I}_{{\metaopt}}$)\\ \hline
			20 & 0.01x &  8 \\
			20 & 0.05x &  7\\
			14 & 0.01x &  7\\
			\hline
		\end{tabular}
	}
	\caption{\metaopt finds slightly tighter bounds when constraining the number and size of balls. For \sf{OPT}($\mathcal{I}$)=\textbf{6}, the tightest known theoretical bound for \ffd~\cite{ffd-1d-tight} is \textbf{8}. This assumes the input can have an unlimited number of balls and that ball can have any size.\label{tab:1d-ffd}}
	\vspace{1mm}
	{\footnotesize
		\begin{tabular}{ c c c c c }
			
			\multirow{2}*{${\sf OPT}(\mathcal{I})$ }& \multicolumn{2}{c}{\metaopt} & \multicolumn{2}{c}{theoretical bound~\cite{VBP-Heuristics}} \\ \cline{2-5}
			& \#balls & approx ratio & \#balls & approx ratio \\ \hline
			2 & 6 & 2.0 & 4 & 1.0 \\
			3 & 9 & 2.0 & 12 & 1.33 \\
			4 & 12 & 2.0 & 24 & 1.5 \\
			5 & 15 & 2.0 & 40 & 1.6 \\
			\hline
		\end{tabular}
	}
	\caption{\metaopt finds adversarial examples with tighter approx. ratio for 2d-\ffd than the best known theoretical bound~\cite{VBP-Heuristics}.\label{tab:2d-ffd}}
		
%		The approximation ratio of of 2d-\ffd for adversarial inputs from \metaopt and those from the best known theoretical bound~\cite{VBP-Heuristics}.\label{tab:2d-ffd}}
\end{table}

%\begin{table}[t!]
%	\centering
%	{\footnotesize
%		\begin{tabular}{ c c c c c }
%			
%			\multirow{2}*{${\sf OPT}(\mathcal{I})$ }& \multicolumn{2}{c}{\metaopt} & \multicolumn{2}{c}{theoretical bound~\cite{VBP-Heuristics}} \\ \cline{2-5}
%			& \#balls & approx ratio & \#balls & approx ratio \\ \hline
%			2 & 6 & 2.0 & 4 & 1.0 \\
%			3 & 9 & 2.0 & 12 & 1.33 \\
%			4 & 12 & 2.0 & 24 & 1.5 \\
%			5 & 15 & 2.0 & 40 & 1.6 \\
%			\hline
%		\end{tabular}
%	}
%	\caption{The approximation ratios of adversarial inputs for 2d-\ffd achieve for those inputs that \metaopt generates and those from the best known theoretical bound~\cite{VBP-Heuristics}.\label{tab:2d-ffd}}
%\end{table}

\parab{Improving the bound on the optimality gap of 2d-\ffd.} While multi-dimensional \ffd is widely used in practice~\cite{protean,tetris,synergy}, its theoretical guarantees substantially lag behind. Recently, \cite{VBP-Heuristics} crafts an example where
${\sf FFDSum}(\mathcal{I}) \geq \alpha_{{\sf OPT}(\mathcal{I})} {{\sf OPT}(\mathcal{I})}$ with $\alpha_{{\sf OPT}(\mathcal{I})} \in [1,2)$ and $\alpha_{{\sf OPT}(\mathcal{I})} \to 2$ as ${{\sf OPT}(\mathcal{I})} \to \infty$. This implies that the approximation ratio $\frac{{\sf FFDSum}(\mathcal{I})}{{\sf OPT}(\mathcal{I})}$ converges to $2$ for large enough problems, but it is strictly smaller than $2$ for any finite size problem. 

In this setting, \metaopt finds adversarial inputs with approximation ratio of $2$ \emph{for every problem size we considered} (Table~\ref{tab:2d-ffd}). For example, when ${\sf OPT}(\mathcal{I}) = 4$ bins, \metaopt finds an adversarial input $\mathcal{I}$ with $12$ balls such that ${\sf FFDSum}(\mathcal{I}) = 8$ (= approx. ratio of $2$)  while \cite{VBP-Heuristics} uses $24$ balls and only achieves approximation ratio of $1.5$.

These empirical findings suggest that the approximation ratio of ${\sf FFDSum}$ is at least $2$. We prove this formally:

%We next show how we can derive constructive proofs for combinatorial problems with {\metaopt}'s help~---~
%we extrapolated from the adversarial inputs it generated and proved:


%\metaopt in this setting finds adversarial inputs that achieve approximation ratios of $2$ \emph{for every problem size we considered} (Table~\ref{tab:2d-ffd}).
%For example, when $\opt(\mathcal{I}) = 4$ bins, \metaopt finds an adversarial input $\mathcal{I}$ with $12$ balls such that ${\sf FFDSum}(\mathcal{I}) = 8$ (=approx. ratio of $2$)  while \cite{VBP-Heuristics} uses $24$ balls and only achieves ${\sf FFDSum}(\mathcal{I}) = 6$ (approx. ratio = $1.5$).





%The empirical findings in~\autoref{tab:2d-ffd} suggest the approximation ratio of ${\sf FFDSum}$ is at least $2$ for a wide variety of problems.
%We show this formally:


% Thus, the approximation ratio of FFDSum for 2-dimensional \vbp is at least 2. 
\begin{theorem}
	\label{th:ffdsum:approx-ratio}
	In 2-dimensional \vbp, for any $k > 1$, there exists an input $\mathcal{I}$ with $OPT(\mathcal{I}) = k$ and $FFDSum(\mathcal{I}) \geq 2k$. 
\end{theorem}
\begin{proof}[Proof Sketch]
	\secref{apendix:proof:ffdsum} contains the detailed proof. For any non-negative integer $p$ and $m$ (at least one positive), we can construct an input with $6m + 9p$ balls such that \opt needs $k = 2m + 3p$ bins while ${\sf FFDSum}$ needs $4m + 6p$ bins.
\end{proof}

Our proof directly follows from the adversarial inputs by \metaopt, and shows another application of {\metaopt}, where users can interpret common features across the adversarial inputs and incorporate them in theoretical proofs. 

%We derive a similar constructive proof for SP-PIFO through the adversarial inputs \metaopt found (see~\S\ref{}).

%The significance of this theorem goes beyond just improving the approximation ratio, but also in using substantially fewer balls compared to~\cite{VBP-Heuristics}. For instance, when ${\sf OPT}(\mathcal{I}) = 10$,~\cite{VBP-Heuristics} needs 180 balls to get an approximation ratio of 1.8 whereas \theoremref{th:ffdsum:approx-ratio} requires 30 (6x less) balls to achieve an approximation ratio of 2. For ${\sf OPT}(\mathcal{I}) = 100$, these numbers are 19800 balls and approx ratio of 1.98 for~\cite{VBP-Heuristics} and 300 (66x less) balls and approx ratio of 2 for~\theoremref{th:ffdsum:approx-ratio}.


\subsection{Heuristics for WAN Traffic Engineering}
\label{s:eval:te}

\begin{table}[t]
	\centering
	{\footnotesize
		\begin{tabular}{c l l}
			\textbf{Topology} & \textbf{\# Nodes} & \textbf{\# Edges} \\\hline
%			\textbf{LargeWAN} & $\sim$1000s  & $\sim$1000s\\
			%			\textbf{WANSmall} & $\sim$100s & $\sim$1000s\\
%			\textbf{\href{http://www.topology-zoo.org/maps/Kdl.jpg}{KDL}} & 754     & 1790 \\ 
			\textbf{\href{http://www.topology-zoo.org/maps/Cogentco.jpg}{Cogentco}} & 197 & 486 \\
			%			\textbf{\href{http://www.topology-zoo.org/maps/UsCarrier.jpg}{UsCarrier}} & 158 & 378 \\
			%			\textbf{\href{http://www.topology-zoo.org/maps/GtsCe.jpg}{GtsCe}}  & 149  & 386 \\
			%			\textbf{\href{http://www.topology-zoo.org/maps/TataNld.jpg}{TataNld}}  & 145 & 372
			\textbf{\href{http://www.topology-zoo.org/maps/Uninett2010.jpg}{Uninett2010}} & 74 & 202 \\
			\textbf{Abilene}~\cite{Abilene} & $10$ & $26$ \\
			\textbf{B4}~\cite{b4} & $12$ & $38$ \\
			\textbf{SWAN}~\cite{swan} & $8$ & $24$		
		\end{tabular}
	}
	\caption{\footnotesize Details of the topologies used in~\secref{s:eval:te}. \label{t:topos}}
\end{table}

\begin{figure*}[t!]
	\centering
	\subfigure[Gap vs. latency for B4 + {\dempin} ($T_d=1\%$)]{
		\centering
		\includegraphics[width=0.43\linewidth]{figs/gap-vs-time/dp_B4_DP-0.01.pdf}
		\label{f:dp-0.01-baseline:b4}
	}\hfill
	\subfigure[B4 + {\dempin} ($T_d=5\%$)]{
		\centering
		\includegraphics[width=0.215\linewidth]{figs/gap-vs-time/max_dp_B4_DP-0.05.pdf}
		\label{f:dp-0.05-baseline:b4}
	}\hfill
	\subfigure[B4 + average gap of {\pop}]{
		\centering
		\includegraphics[width=0.215\linewidth]{figs/gap-vs-time/max_expected_pop_B4.pdf}
		\label{f:pop_quality}
	}
	\\
	\subfigure[Gap vs. latency for Cogentco + {\dempin} ($T_d=1\%$)]{
		\centering
		\includegraphics[width=0.43\linewidth]{figs/gap-vs-time/dp_Cogentco_DP-0.01.pdf}
		\label{f:dp-0.01-baseline:Cogentco}	
	} \hfill
	\subfigure[Cogentco + {\dempin} ($T_d=5\%$)]{
		\centering
		\includegraphics[width=0.215\linewidth]{figs/gap-vs-time/max_dp_Cogentco_DP-0.05.pdf}
		\label{f:dp-0.05-baseline:Cogentco}	
	} \hfill
	\subfigure[Cogentco + average gap of {\pop}]{
		\centering
		\includegraphics[width=0.215\linewidth]{figs/gap-vs-time/max_expected_pop_Cogentco.pdf}
		\label{f:pop-baseline:Cogentco}	
	}
	\caption{{\metaopt} is faster and finds larger gaps between {\sf OPT} and \pop or \dempin on the Cogentco and B4. For fair comparison, we report the gap relative to the total capacity and use only one thread to run each methods (SA = Simulated Annealing, HC = Hill Climbing).\label{f:method_gap_vs_latency:dp}}
\end{figure*}

% We next introduce the setup for our experiments and evaluate several aspects of \metaopt (comparing it with baselines, use it to better understand and improve existing heuristics, and evaluates its ability to find realistic adversaries).


\parab{Experiment Setup.} We use $K$-shortest paths~\cite{YenKLoopLess} to find the paths between node pairs~($=4$ if unspecified). We constrain the demands to be below a maximum value (half the average link capacity if unspecified) to ensure they are realistic and a single demand does not create a bottleneck. For \dempin, we vary the demand pinning threshold (=$5$\% of average link capacity if unspecified). For \pop, we vary the number of partitions (=$2$ if unspecified) and report the average gap over $5$ random trials (see~\secref{s:d:heur_form}). We report runtimes on an AMD Operaton 2.4GHz CPU (6234) with 24 cores and 64GB of memory. 
%To be fair to the baselines we ran everything on a single thread. For all other experiments, we use all available threads. When we use our clustering approach, we timeout each optimization after $20$ minutes.


\vspace{1mm} 
\noindent \emph{Topologies.} We use two large topologies from~\cite{itzoo} and three public production topologies~\cite{swan,Abilene,b4}. See~\autoref{t:topos}.

\vspace{1mm}
\noindent \emph{Metrics.} To obtain a metric comparable across different scales, we normalize the performance gap by the sum of the link capacities. 


\vspace{1mm} 
\noindent \emph{Benchmarks.} We compare \metaopt with random search, hill climbing~\cite{hill_climbing}, and simulated annealing~\cite{simulated_annealing}. Random search repeatedly picks new random inputs and returns the one with maximum gap. Hill climbing (HC) and simulated annealing (SA) use information from past observed inputs to guide the search (more details in~\xref{appendix:black-box}).  


\parab{Comparison to baselines (\figref{f:method_gap_vs_latency:dp}).} {\metaopt} is the only method that consistently discovers substantially larger gaps over time, while other techniques get stuck in local optima and improve slightly even after many hours (Fig.~\ref{f:dp-0.01-baseline:b4},~\ref{f:dp-0.01-baseline:Cogentco}). 


%\autoref{f:method_gap_vs_latency:dp} shows the gaps discovered by various methods on two topologies (Cogentco and B4) and three heuristics (\pop and \dempin with $T_d=5$\%, $1$\%).
%The left-most figures show how the gap found increases over execution time. To conserve space, the other figures only show the largest gaps that were found.

%We compare \metaopt with the three benchmarks in \figref{f:method_gap_vs_latency:dp}. 
%This figure illustrates the maximum gap (between \opt and \heur) \metaopt found for 2 topologies at different scales (Cogentco and B4) and 3 different heuristics ({\dempin} with two thresholds and average {\pop}). 
%\figref{f:dp-0.01-baseline:Cogentco} and \figref{f:dp-0.01-baseline:b4} show each method's progress over time. For the remainder of the settings, we only show the final gap due to space constraints. 



Overall, \metaopt finds larger gaps ($1.7$x~-~$17$x compared to the next best).
The baselines fail since they ignore the details of the heuristic and treat it as black-box. However, {\metaopt} uses its knowledge of the heuristic and the topology to guide the search.
This effect is more noticeable for {\dempin} and small topologies perhaps because the inputs with sizable gaps are relatively fewer in these cases.
%is small as is the case .\footnote{Only a small portion of the space of valid demand values is pinned (1\% or 5\%) and the number of demand pairs is limited.}

%This comparison is unfair to \metaopt: we run everything on a single thread. We designed {\metaopt}'s clustering technique to run multiple instances in parallel and if we use multiple threads we can get significant speed-up. But the baselines cannot leverage the additional threads as effectively even if we use methods such as \pop or NCFlow~\cite{pop,ncflow} to speedup their search~---~they find the same gap after a few hours as they had after a few minutes.

\parab{Adversarial patterns for \dempin (\figref{f:maxgap_vs_params_dp}).}
Intuitively, the optimality gap of \dempin increases as we increase its threshold since the heuristic forces more demands on their shortest path. The gap grows faster on some topologies even though they have roughly the same number of nodes and edges.

To explain this, we studied \dempin using synthetic topologies. We create each topology by starting with a ring graph and then connecting each node to a varying number of nearest neighbors. The results (\figref{f:dp_path_length}) indicate that the performance gap grows with the (average) shortest path length (fewer connections = longer shortest paths). Intuitively, if the shortest path lengths are longer on average, \dempin will use the capacity on more edges to route the small demands. This reduces the available capacity to route other larger demands.

\begin{figure}[t!]
	\centering
	\subfigure[Gap vs. the threshold value for {\dempin}.]{
		\centering
		\includegraphics[width=0.89\linewidth]{figs/sweep_threshold_dp/demandpinning_sweep_threshold.pdf}
		\label{f:dp_thresh}
	}
	\\ \vspace{-2mm}
	\subfigure[Gap vs. connectivity.]{
		\centering
		\includegraphics[width=0.89\linewidth]{figs/sweep_topo_dp/demand_pinning_sweep_topo.pdf}
		\label{f:dp_path_length}
	}
	\caption{\dempin's optimality gap increases with the threshold and decreases with the connectivity.
		\label{f:maxgap_vs_params_dp}}
\end{figure}


\parab{Adversarial patterns for \pop (\figref{f:expected_pop}).}
Since \pop is a random heuristic, we search for inputs that maximize the expected gap. We approximate this expectation by an empirical average over $n$ random partition samples. Then, we evaluate the generalization of adversarial inputs from \metaopt by testing them on 100 other random instances. When \metaopt uses a small number of samples to estimate the expected gap, the adversarial inputs overfit. Increasing the number of samples improves the generalization but at the cost of scalability. We find $n=5$ is usually enough for a robust estimation.

As we increase the number of \pop partitions, the optimality gap of \pop increases because each partition (1) gets a smaller fraction of each edge's capacity, and (2) has less information about the global state. We can reduce this gap by increasing the number of paths as it helps each partition better allocate the fragmented capacity.

\begin{figure}[t!]
	\centering
	\subfigure[Gap vs. instances to approximate the expected value.]{\centering\includegraphics[width=0.89\linewidth]{figs/pop_num_samples/b4_expected_pop.pdf}\label{f:expected_pop}}
	\\
	\subfigure[Gap vs. \#paths and \#partitions for avg {\pop}.]{\centering\includegraphics[width=0.89\linewidth]{figs/pop_path_partition/pop_varying_path_partitions.pdf}\label{f:pop_vs_numpartitions}}
	\caption{The optimality gap of \pop on B4 when we vary: (a) \#instances to approximate average; and (b) \#paths and \#partitions.}
\end{figure}

\parab{Finding {\em realistic} adversarial demands (\figref{f:real-constr:locality}).}  
Production demands have strong locality~\cite{ncflow} and are very sparse (a small fraction of pairs have non-zero demands). We add these requirements as additional constraints in \metaopt. The resulting gap is only <1\% lower than the unconstrained case. while the discovered demands are sparser and between nearby nodes. The result shows these two have large gaps even under realistic constraints.
% In this case, \metaopt finds the gap only reduces by less than one percent. %This shows even in realistic settings \dempin and \pop have substantial optimality gaps.  


%\figref{f:real-constr:locality} shows features of the adversarial inputs \metaopt finds for \dempin and \pop in the absence of additional constraints: $50\%$ of large demands are over $7$ hops apart in both cases and more than half the demands in the \dempin case ($\ge 54\%$) are non-zero. 
%These findings suggest \metaopt's result is likely an over-estimate and not representative of how these heuristics perform in empirically relevant inputs.

%To find more realistic adversarial inputs, we restrict the demand space: we only allow large demands between nodes that are less than $4$ hops apart. 
%This constraint improves the locality and density of the adversarial demands and they become closer to real-world demand matrices. 
%But the gap is only minimally reduced by this change ($<1\%$).
%This shows {\pop} and {\dempin} can still have large gaps even when subjected to realistic demand matrices.



\begin{figure}[t]
	\centering
	\subfigure[Impact of adding locality constraint on gap and density]{
		\centering
		{\footnotesize
			\begin{tabular}{c l c c }
				
				Heu & Constraint & Density & Gap \\ \hline
				\multirow{2}{*}{{\dempin}} & ~--~ & 54.06\% & 33.9\% \\ 
				& locality (distance of large demands $\leq 4$) & 12.03\% & 33.4\% \\\hline
				\multirow{2}{*}{{\pop}} & ~--~ & 16.14\% & 20.76\% \\ 
				& locality (distance of large demands $\leq 4$)& 4.74\% & 20.70\% \\ \hline
			\end{tabular}
		}
	}  
	\\
	\subfigure[Impact of adding locality constraint on {\dempin}]{
		\centering
		\includegraphics[width=0.89\linewidth]{figs/realistic_constraints/locality_demands_dp_0.05.pdf}
	}
	\\
	\subfigure[Impact of adding locality constraint on {\pop}]{
		\centering
		\includegraphics[width=0.89\linewidth]{figs/realistic_constraints/locality_demands_Avg-POP_0.05.pdf}
	}
	\caption{We use \metaopt to find practical adversarial inputs on Cogentco. In both cases, the constraint on the input space led to more local and sparser adversarial inputs. \label{f:real-constr:locality}}
\end{figure}


\parab{Improving performance gap of \dempin (\figref{f:modified-dp:thresh-fix}).} \metaopt shows \dempin has higher performance gap when nodes have larger average distance.
We use this insight to modify {\dempin} and design a better heuristic (modified-\dempin): we only pin a demand if it is below the threshold and {\em it is between nodes that are less than $k$ hops apart}. The user specifies $k$. The new heuristic routes small demands between far apart nodes optimally and leaves more capacity for other demands. Its performance gap is $12.5\times$ smaller than \dempin for $T_d=1\%$ and $k = 4$.

As we increase the distance threshold, modified-\dempin can pin more demands (better scalability) but at the cost of higher optimality gap. {\metaopt} can help operators adjust the parameter $k$ based on their needs.

Modified-{\dempin} has another benefit: we can use a higher demand threshold $10$x-$50$x and maintain the same gap as the original {\dempin}. We show this by fixing the gap at $5\%$ and computing the maximum threshold each method can admit using \metaopt (\figref{f:modified-dp:gap-fix}). Operators can leverage this to pin more demands when small demands exhibit strong locality~\cite{ncflow}. 


\begin{figure}[t]
	\centering
	\subfigure[Maximum threshold such that discovered gap $\sim 5\%$.]{
		\centering
		{\footnotesize
			\begin{tabular}{ c c c }
				
				Heuristic & Distance & Threshold wrt avg link cap \\ \hline
				{\dempin} & ~--~ & 0.1\% \\ \hline
				\multirow{2}{*}{modified-{\dempin}} & $\leq 6$ & $1\%$ (10x) \\
				& $\leq 4$ & $5\%$ (50x) \\ \hline
			\end{tabular}
		}
		\label{f:modified-dp:gap-fix}
	} 
	\\
	\subfigure[{\dempin} vs. modified-{\dempin}]{
		\centering
		\includegraphics[width=0.89\linewidth]{figs/modified_dp/max_modified_pop_Cogentco.pdf}
		\label{f:modified-dp:thresh-fix}
	}
	\caption{We propose modified-{\dempin} based on insights from \metaopt. It only pins small demands between near nodes, is more resilient, and pins more demands with the same gap\label{f:modified-dp}.}
%	We propose modified-{\dempin} based on \metaopt~---~we constrained which default shortest paths DP can use: it became more resilient and pinned more demands, with the same gap\label{f:modified-dp}.
\end{figure}


%\noindent \textbf{\metaopt with a large $n$ generalizes across partitions in \pop(~\figref{f:expected_pop}).} Because \pop is a random heuristic we search for inputs that lead to large expected gaps. We use an empirical average over $n$ random partitions to approximate this expectation. We evaluate the quality of this approximation as a function of the number of partitions we use and test the adversarial inputs we found on 100 other random partition samples to see if the result generalizes. 
%
%The worst case gap reduces by $\sim3$x when we only use a single random partition compared to when we use $n = 10$. This indicates the adversarial input can overfit to the set of random partitions we use (if we use few partitions). We can avoid this problem if we increase $n$: our results confirm the gap \metaopt finds generalizes for larger $n$. But larger $n$ makes it harder for \metaopt to scale: we need to find the right balance to both generalize and maintain our ability to scale. We find $n=4$ is enough to find high-quality inputs and not affect \metaopt's ability to scale.
%
%We find the gap between {\sf OPT} and \pop increases as we increase the number of partitions because each partition gets a smaller fraction of each edge's capacity and because the partition does not see the global state. \pop can reduce this gap with more paths because the heuristic can use them to better allocate the fragmented capacity.



%\begin{figure}[t!]
%	\centering
%	\subfigure[Gap vs. instances to approximate the expected value.]{\centering\includegraphics[width=0.89\linewidth]{figs/pop_num_samples/b4_expected_pop.pdf}\label{f:expected_pop}}
%	\\
%	\subfigure[Gap vs. \#paths and \#partitions for avg {\pop}.]{\centering\includegraphics[width=0.89\linewidth]{figs/pop_path_partition/pop_varying_path_partitions.pdf}\label{f:pop_vs_numpartitions}}
%	\caption{The optimality gap of \pop on B4 when we vary: (a) \#instances to approximate average; and (b) \#paths and \#partitions.}
%\end{figure}

\parab{Performance gap of running \pop and \dempin in parallel.}
Imagine a new heuristic that runs \pop and \dempin in parallel and selects the best solution for each input. At first, the two heuristics appear to have distinct adversarial inputs: \dempin underperforms when distant pairs have small demands and \pop when large demands that go through the same link end up in the same partition. We expected combining them would reduce the optimality gap significantly compared to each one. However, \metaopt shows the new heuristic only improves the optimality gap by $6\%$ on Cogentco. It uncovers inputs where small demands are between distant pairs (adversarial to \dempin ) and large demands are between nearby nodes that end up in the same partition (adversarial to \pop).


\subsection{Heuristics for Packet Scheduling}
\label{s:packet-scheduling-eval}
\pooria{will finish this section after adding the results to appendix.}

\begin{figure}[t]
	\includegraphics[width=0.91\linewidth]{figs/SP-PIFO/sp_pifo_packet_delay.pdf}
	\caption{We compared the average delay of packets with the same priority. We use a stream of $10^6$ packets where the priority of packets is between $0-100$. As in SP-PIFO we use infinite queues. We normalize the numbers by the average delay of the highest priority packets (rank = 0). For the case where all the $10^6$ packets arrive at the same time and the queues drains at $40$ Gbps the average delay for the highest priority packets in PIFO is $0.074$ seconds (the sequence of packets results in similar relative performance between the heuristic and the optimal for any arrival/departure pattern).}
\end{figure}
\parab{\metaopt shows SP-PIFO delays the highest priority packets by $3\times$ compared to PIFO.} \metaopt finds a packet trace where SP-PIFO cannot approximate priorities correctly (the highest priority packets experience $3\times$ higher delay on average compared to the second lowest priority packets).

\textit{We also show how we used \metaopt in a similar way to modify SP-PIFO~\S\ref{}.} We omit details here due to space.%They will have to explore the tradeoff between how many demands \dempin can pin and how big the gap can grow.

\behnaz{add SP-PIFO theorem and modified SP-PIFO to appendix and then reference here.}


\subsection{Impact of Design Choices}
\label{s:import-design-choic}

\metaopt uses partitioning, rewrites, and quantization to find adversarial gaps quickly.
%\metaopt's clustering, convex rewriting, and quantization all contribute to its ability to find adversarial gaps quickly. 

%We evaluated how a new heuristic that runs \pop and \dempin in parallel and choose the best solution for each input works. Our results show a small reduction (less than 6\%) compared to the best of individual heuristics. At the first glance, these two (\pop and \dempin) seem to have a non-overlapping set of adversarial inputs and we would expect a substantial gap from combining them; \pop's gap comes from large demands on the same link ending up in the same partition while \dempin's gap is from small demands between distant pairs. However, we can have an adversarial input that combines both effects; a traffic that has small demands between distant pair while near-by nodes exchange large demands and end up in the same partition. These small demands cause gap for \dempin whereas those large demands cause gap for \pop. This result illustrates another importance of \metaopt in finding whether combining multiple heuristics is effective or not.
%\pooria{waiting for the results.}
%\pooria{reporting the numbers. DP: $33.39\%$, Avg \pop: $20.70\%$, Combined: $14.85$.}

%\begin{figure}
%	\includegraphics[width=1\linewidth]{figs/parallel_pop_dp/parallel_pop_dp_Cogentco_DP-0.05.pdf}
%	\caption{Combining \pop and \dempin on Cogentco.}
%\end{figure}

%\begin{table}
%	\centering
%	{\footnotesize
%		\begin{tabular}{|c|c|c|}
%			\hline
%			\dempin & Avg \pop & Combined \\ 
%			$33.39\%$ & $20.70$ & $14.85$
%		\end{tabular}
%	}
%	\label{f:parallel-dp-pop}
%\end{table}

%\pooria{please review the below two.}
\parab{Partitioning.} \metaopt uses partitioning to find larger gaps faster than both (non-partitioned) quantized  primal-dual and KKT, even on medium-sized topologies (\figref{f:cluster-ablation:comparison}). For larger topologies, neither KKT nor primal-dual can find large gaps without partitioning.


As we increase the number of partitions, \metaopt scales better and finds larger gaps until it eventually plateaus ($10$ for Cogentco in~\figref{f:cluster-ablation:num-clusters}). We can slightly improve the gap if we double the timeout.


The inter-cluster step in our partitioning technique is important, especially for heuristics that under-perform when demands are between distant nodes such as \dempin (\figref{f:cluster-ablation:inter-cluster}).
The partitioning algorithm also impacts the gap we find.


\begin{figure}[t!]
	\subfigure[KKT vs Quantized primal-dual vs w partitioning on Uninett2010]{
		\centering
		\includegraphics[width=0.91\linewidth]{figs/clustering-ablation/cluster_w_wo_Uninett2010_DP-0.05.pdf}
		\label{f:cluster-ablation:comparison}
	}
	\subfigure[Number of partitions and solver timeout on Cogentco]{
		\centering
		\includegraphics[width=0.89\linewidth]{figs/clustering-ablation/impact_num_clusters_timeout.pdf}
		\label{f:cluster-ablation:num-clusters}
	}
	\subfigure[Inter-cluster on Cogentco]{
		\centering
		\includegraphics[width=0.43\linewidth]{figs/clustering-ablation/impact_inter_cluster.pdf}
		\label{f:cluster-ablation:inter-cluster}
	} \hfill
	\subfigure[Graph partitioning on Cogentco]{
		\centering
		\includegraphics[width=0.45\linewidth]{figs/clustering-ablation/impact_graph_clustering.pdf}
		\label{f:cluster-ablation:graph}
	}
	\caption{We investigate the impact of partitioning in \metaopt's results. It helps \metaopt find larger gaps faster. \label{f:cluster-ablation}}
\end{figure}

\parab{Convex rewrites (\figref{t:rewriting:quantization_qpd}).} We compare the number of \textit{binary variables} after the quantized primal-dual or KKT rewrites. This measures the complexity and estimates speed (the number of branches in MILP is $2^\text{\#binary}$). KKT has a significantly larger number of binary variables than quantized primal-dual, which explains why it was unable find any gap in~\figref{f:cluster-ablation:comparison} even after many hours.


\begin{figure}[t!]
	\centering
	\subfigure[\#binary in KKT vs in Quantized primal-dual]{
		\centering
		{\footnotesize
			\begin{tabular}{ c c c c }
				
				\#edges & 38 & 202 & 486 \\ \hline
				\#binary Quantized primal-dual & 264 & 10804 & 77224 \\
				\#binary KKT & 1226 & 48622 & 347572 \\ \hline
			\end{tabular}
			\label{t:rewriting:quantization_qpd}
		}
		\label{f:rewriting:branches}
              }

       \subfigure[Quantization error on B4]{
	\centering
			{\footnotesize
		\begin{tabular}{ c c c }
			
			 & Avg POP & DP (5\%) \\ \hline
			Quantization error & 0\% & 4\% \\ \hline
		\end{tabular}
		\label{t:rewriting:quantization_b4}
	}}
	\caption{We measure the complexity and impact of rewrites as the number of binary variables and the quantization error.
		\label{f:rewriting}}
      \end{figure}

\parab{Quantization (\figref{t:rewriting:quantization_b4}).} Quantization has little impact on solution quality. The relative difference between the gap from quantized primal-dual and KKT (which does not use quantization) is $4\%$ for \dempin and 0 for \pop on B4. 

For \pop, the primal-dual rewrites use two quantiles: 0 and the max demand. If a demand $d$ in an uncongested partition falls in between these values, forcing the demand to zero cannot decrease the gap: the rewrite's throughput would drop by $d$, and the optimal throughput by some value between 0 and $d$. A similar argument applies to the congested case. 

For \dempin, we use three quantiles: 0, the threshold, and the max demand. For a high enough threshold, quantized primal-dual may avoid assigning the threshold value to demands between distant nodes to avoid violating capacity constraints, whereas KKT can assign any value, resulting in a relative difference in solution quality.



==> texfiles/intro.tex <==
\vspace{-2mm}
\section{Introduction}
\label{s:intro}

Many solutions to network and systems problems are heuristic approximations to potentially intractable optimal algorithms~\cite{ncflow,swan,b4,pop,arrow,tetris,synergy,teavar}.
While these heuristics are faster or scale better than their optimal counterparts, users and designers alike often do not fully understand how these heuristics behave with previously-untested inputs or how far from the optimal their results may drift in realistic use.
% Many heuristics lack optimality proofs, approximation bounds, or even guidance on when and to what extent they may underperform.

%Heuristic solutions lack worst-case performance guarantees but remain widely deployed.

For example, a heuristic Microsoft uses to distribute traffic among paths on their wide area network~\cite{blastshield} has an optimality gap of {\em at least} 40\%.
It routes small demands (\ie demands $\leq$ a given threshold) through their shortest path and applies a more computationally complex optimization~\cite{swan}, which jointly considers all demands, on the remaining demands. We refer to this heuristic as demand pinning (\dempin).
\figref{f:pinning_issues} shows a case where {\dempin} has a 40\% optimality gap: the demand $1 \rightarrow 3$ is at the threshold $(=50)$, so {\dempin} consumes capacity on its shortest path, which reduces the available capacity for flows $1\rightarrow2$ and $2\rightarrow3$. A $40\%$ gap in this case means Microsoft would have to either over-provision their network by 40\%; delay 40\%; or drop 40\% of their customers' demand! In some cases (e.g., in Google's B4E~\cite{b4AndAfter}) this can reduce quality of service. Notice the maximum gap may be higher!

\vspace {0.05in}
We want to enable practitioners to ask questions such as: What inputs would trigger a heuristic's worst-case outcome? Do these outcomes hold for practical inputs? For which inputs would a heuristic be within (or over) a certain percentage of the optimal? How often and by how much does one heuristic outperform another? Answers to these questions can enable practitioners to choose better heuristics or to devise workarounds that avoid the negative impact.



\begin{figure}  
	\centering  
	\begin{tikzpicture}[  
	scale=0.75, transform shape,  
	node distance=0.75cm,  
	font=\small,  
	every edge/.style={draw, -Stealth},  
	every edge quotes/.style={auto, font=\footnotesize},  
	state/.style={circle, draw}  
	]  
	\begin{scope}  
	\node[state] (1) {1};  
	\node[state, right=of 1] (2) {2};  
	\node[state, right=of 2] (3) {3};  
	\node[state, below=of 1] (4) {4};  
	\node[state, right=of 4] (5) {5};  
	
	\path  
	(1) edge[above, "100"] (2)  
	(2) edge[above, "100"] (3)  
	(4) edge[below, "50"] (5)  
	(1) edge[below, "50"] (4)  
	(5) edge[below, "50"] (3)  
	;  
	\end{scope}  
	
	\node[anchor=west] at ([yshift=-0.5cm]3.east){  
	\begin{tabular}{cc | cc | cc}  
	\multicolumn{2}{c}{Demand} & \multicolumn{2}{c}{DP (thresh = 50)} & \multicolumn{2}{c}{OPT} \\  
	\hline  
	src-dest & value & path & value & path & value \\  
	\hline  
	1-3 & 50 & 1-2-3 & 50 & 1-4-5-3 & 50 \\  
	1-2 & 100 & 1-2 & 50 & 1-2 & 100 \\  
	2-3 & 100 & 2-3 & 50 & 2-3 & 100 \\  
	\hline
	& & Total DP & \textbf{150} & Total Opt & \textbf{250}  \\
	\cline{3-6}
	\end{tabular}  } ; 
	\end{tikzpicture}  
\caption{{Suboptimal performance of \dempin. (left) Topology with unidirectional links. (right) A set of demands and their flow allocations using the \dempin heuristic and the optimal ({\opt}) solution. \dempin first sends the demands at or below the threshold ($50$) over their shortest paths and then optimally routes the remaining demands. \label{f:pinning_issues}}}%\vspace{-0.05in} 
\end{figure}   

%\begin{figure}[t!]
%	\centering
%%	\includegraphics[width=0.95\linewidth]{figs/intro_example_v2.png}
%	\includegraphics[width=0.95\linewidth]{figs/fig1new_crop.pdf}
%	\caption{{Suboptimal performance of \dempin. (left) Topology with unidirectional links. (right) A set of demands and their flow allocations using the \dempin heuristic and the optimal ({\opt}) solution. \dempin first sends the demands at or below the threshold ($50$) over their shortest paths and then optimally routes the remaining demands. \label{f:pinning_issues}}}%\vspace{-0.05in} 
%\end{figure}


\vspace {0.05in}
We design and implement a system, {\metaopt}, that solves this problem through a multi-level optimization: 
\begin{equation}
\arg\hspace{-12mm}\max_{{\text{s.t. input} \,\, \mathcal{I} \in {\sf ConstrainedSet}}}   {\sf OPT}(\mathcal{I}) - {\sf Heuristic}(\mathcal{I}),
\label{eqn:adversarial_outer}
\end{equation}
%
where ${\sf OPT}()$ and ${\sf Heuristic}()$ solve the optimal and heuristic algorithms, the input is $\mathcal{I}$, and ${\sf ConstrainedSet}$ contains constraints on the space of inputs. We can view this problem and its formulation through the lens of game-theory as an instance of a broader set of problems known as Stackelberg games~\cite{games} (see~\S\ref{sec::stackelberg}). We show this solution applies to, and finds a provable worst-case gap quickly for, any heuristic we can pose as a convex optimization or as a feasibility problem. We show how to use it to compare different heuristics (this is also useful in those cases where we do not know {\sf OPT}). 

We used {\metaopt} to test two heuristics {\em operators often use in production} from different domains: vector bin packing~\cite{VBP-Heuristics,tetris} and traffic engineering~\cite{swan,b4,blastshield,pop}. We also analyzed other recently proposed heuristics~\cite{pop, sp-pifo}. We find larger optimality gaps for the heuristics we analyzed than the authors~\cite{blastshield, pop} reported. We build on the insights from the inputs \metaopt found and developed a new heuristic that has a $12.5\times$ lower optimality gap than \dempin. We prove a tighter performance bound than what was known for a vector bin packing heuristic~\cite{VBP-Heuristics} that has received substantial theoretical scrutiny~\cite{ffd-1d-tight,ffd-1d-1973,ffd-1d-1985,ffd-1d-1991,multi-bp-survery}. Through these examples we show the various ways operators can use \metaopt to understand the performance of their heuristics; and how they can apply {\metaopt} to a broad spectrum of optimization-based, algorithmic, and probabilistic heuristics. We show 
{\metaopt} outperforms other search methods~---~it finds up to $17\times$ larger gaps in orders of magnitude less time.  

It is hard to find good adversarial examples, quickly, for a broad class of heuristics and this model allows us to avoid the common pitfall of other search techniques~\cite{hill_climbing,simulated_annealing} which get stuck in local optima (see~\S\ref{s:eval}) and fail to find large gaps quickly.
% Recent work~\cite{venkat} uses bounded model checking to solve similar problems but fail to quantify the {\em true} gap since they do not fully model the heuristic for its entire duration\footnote{These work tackle a different space of heuristics~---~those that we can represent through a sequence of decisions~---~in that sense {\metaopt} is complementary as it opens the space to not only sequential heuristics but also any that we can represent as a set of feasibility or convex constraints.} (when we use \metaopt in its approximate mode~\S\ref{s:d:part}, it applies to more cases and is more precise compared to~\cite{venkat}).
 We discuss related work in~\xref{s:related}. 


It is also hard to solve {multi-level} optimizations and commodity solvers~\cite{Z3,gurobi} do not support them~\cite{bilevel_survey}. {\metaopt} automatically converts the problem into a provably equivalent form that commodity solvers support (\xref{s:design}): it examines the optimal and the heuristic and decides if it needs to change its formulation to convert the bi-level optimization into a single-shot one (see~\autoref{fig::scope}). These changes are in terms of ``re-writes'' based on the KKT and strong duality theorem~\cite{boyd_co}, and a novel quantized variant~---~each of which has different strengths. We also extend this approach to support heuristics that make conditional~(e.g., {\dempin} in~\autoref{f:pinning_issues}) or random actions~(e.g., {\pop}~\cite{pop}); appear as iterative code~(e.g., \ffd~\cite{VBP-Heuristics}); or involve updates to weights and priorities~\cite{sp-pifo,aifo}~---~they do not, at first, look like optimizations.  To scale, we show a novel partitioning technique that applies {\metaopt} in parallel on different sub-problems and composes the results carefully to find good adversarial inputs for the full instance.

%\begin{figure}  
%	\centering  
%	\begin{tikzpicture}[  
%	node distance=1.9cm,  
%	auto,  
%	every node/.style={align=center, font=\footnotesize},  
%	decision/.style={diamond, draw, text width=1.2cm, inner sep=0pt},  
%	block/.style={rectangle, draw, text width=1.3cm, minimum height=1cm},  
%	line/.style={draw, -latex'}  
%	]  
%	
%	\node[decision] (aligned) {Follower aligned?};  
%	\node[decision, below of=aligned] (feasibility) {Feasibility?};  
%	\node[decision, below of=feasibility] (convex) {Convex?};  
%	\node[block, right of=aligned, xshift=1cm] (do_nothing1) {as is};  
%	\node[block, right of=feasibility, xshift=1cm] (do_nothing2) {as is};  
%	\node[block, below of=convex] (kkt) {primal/dual\\or KKT};  
%	\node[block, right of=convex, xshift=1cm] (not_supported) {Error!};  
%	
%	\path[line] (aligned) -- node[above]{Yes} (do_nothing1);  
%	\path[line] (aligned) -- node[right]{No} (feasibility);  
%	\path[line] (feasibility) -- node[above]{Yes} (do_nothing2);  
%	\path[line] (feasibility) -- node[right]{No} (convex);  
%	\path[line] (convex) -- node[left]{Yes} (kkt);  
%	\path[line] (convex) -- node[above]{No} (not_supported);  
%	
%	\end{tikzpicture}  
%	\caption{Top: How MetaOpt converts the bi-level problem to a single optimization automatically. Bottom: How MetaOpt decides whether to use Zen or Gurobi. MetaOpt supports any follower which either (1) is a convex optimization; (2) is a feasibility problem; or (3) has an objective which aligns with the outer problem.}  
%\end{figure}  


%It runs a multi-step workflow, and (when needed) re-writes the inner problems as a set of equivalent 

%{\metaopt} rewrites the two-level optimization as a one-shot optimization that off-the-shelf solvers can solve (\xref{s:design}). 





%To demonstrate {\metaopt} is general, we show how to apply it to heuristics in vastly different domains: vector bin packing~\cite{VBP-Heuristics,tetris} and traffic engineering.
%\metaopt shows the optimality gap of both \dempin and \pop is higher (by {\color{red}XXX}) than what either work reports~\cite{blastshield, pop}; helps identify how to improve \dempin to reduce its optimality gap (by up to $12.5$x); proves a tighter bound for the performance of a vector bin packing heuristic than what, to the best of our knowledge, has been theoretically proven to date (by up to $2$x); and outperforms local search methods~---~it finds larger gaps ($1.7$x~-~$17x$)  while reducing the search time by orders of magnitude.ac

To our knowledge, no prior work {\em provably} finds worst-case gaps for resource allocation heuristics. Some of the techniques we use have deep roots in optimization literature~\cite{boyd_co,bertsimasLinOptBook}. Our main contribution is an end-to-end, scale-able, optimization-based \emph{system} that helps analyze practical heuristics. We further: {\em develop} extensible functions to help users formulate complex heuristics as optimizations; {\em design} automated re-write solutions which allow \metaopt to write heuristics as a set of constraints; and {\em implement} a system that supports multiple commodity solvers (we currently support both Zen~\cite{zen} and Gurobi~\cite{gurobi} and have an interface that easily allows users to add others as well) so that \metaopt applies to a broader set of heuristics. As part of this work we also make an important contribution to the theory on vector bin packing heuristics: we prove a novel, tighter, bound for the \ffd heuristic that operators commonly use in practice.




%we introduce mechanisms in \metaopt that automatically writes heuristics as a set of constraints  


%Yet, our work makes novel contributions in formulating complex heuristics as optimizations, rewriting convex heuristics as sets of constraints, partitioning to improve scalability, implementations on commodity solvers and new tighter bounds for \ffd and a better performing TE heuristic. 
% uses the worst-case gaps it finds to improve existing heuristics, and offers implementations on commodity solvers.
%Some of the techniques that we use (e.g., rewrites using KKT) were previously known~\cite{bilevel_3,bilevel_2,chemKKT}, but 
%combining rewrites with adaptations for randomized and conditional heuristics, using partitioning techniques to enhance scalability, relying on the discovered worst-case gaps to improve existing heuristics, and offering implementations on commodity solvers constitute novel contributions of the current work. 


%Applying {\metaopt} to other heuristics and extending {\metaopt} to the case of sequential optimizations where the results of one optimization feed into the next\footnote{Congestion control and bit-rate selection are instances of such problems.} are some key open issues for future work.  
% alongside possibly unknown environmental changes

% We show that our approach has merit in~\xref{s:eval} where we 
%We are unaware of any prior work that finds provably strong adversarial examples for heuristics. 
%\ryan{we should state some high-level results. don't we have new results for bin packing, and some new ones for demand pining etc. How much better we did than stochastic search. Something punchy here.}

\cut{
we introduce {\metaopt}, a first system that enables practitioners to determine the worst-case optimality gap for optimization heuristics {\em at scale}. \metaopt enables operators to automatically find (realistic) inputs that cause poor performance and to understand the reason so they can efficiently mitigate them.
%
%In the DP example, {\metaopt} shows that when there are many small demands where the shortest path between the source and destination is long, this leads to a high optimality gap: DP routes the small demands on these long default paths and consumes capacity on too many links. The fix is simple. We modify the DP condition so it only routes small flows with short default paths on their default paths. This fix improves the optimality gap by XX.
For instance, similar to the toy example in Figure~\ref{f:pinning_issues}, {\metaopt} found that in realistic settings {\dempin} struggles when there are many small demands between source-destination pairs that are far apart: DP routes these small demands on their long default paths and consumes capacity on too many links. The fix is simple. We modify the DP condition so it pins a small flow only if its default path is short. This fix improves the optimality gap by \textcolor{red}{XX}.


%\santi{I do not understand the `see Figure 2 for an example'. This figure seems to be showing a different thing.}

{\metaopt} helps operators improve their understanding of the heuristics and its limitations by answering questions such as, are there cases where the heuristic is $10\%$ less efficient than the optimal? What is the heuristic's worst-case outcome? Are these examples realistic? What happens if we add constraints on the inputs (e.g., demands following the hose model~\cite{hedera,thr})? Are there conditions that guarantee the heuristic performs well? How does one heuristic compare against another? (see~\secref{ss:extensions})
%Worst-case examples are not always realistic, thus raising the question: given some constraints (e.g., demands following the hose model~\cite{hedera,thr}), are there realistic inputs that trigger poor outcomes? Conversely, are there conditions which guarantee that the heuristic will perform well?
%Answers to these questions can guide practitioners in choosing between heuristics, devising alternatives for hard-to-solve inputs, or in combining heuristics with complementary strengths.


% by deploying multiple heuristics with disjoint sub-optimality regions, combining heuristics with complementary strengths, using a cache to serve the optimal solution for the (potentially limited) set of common bad inputs, or improving the heuristic's design in cases where the tool provides insight about why an input is bad. 


%While this example is illustrative, the largest possible gap for this topology and heuristic is not clear. Similarly, it is unclear what happens if the topology or heuristic changes.

%Also, what about other heuristics and practically relevant topologies?
%\autoref{f:pinning_issues} shows two cases when this heuristic is sub-optimal: in the example on the left, the heuristic loses because the ``small demands'' use up capacity on multiple hops and in the example on the right the heuristic loses because the shortest path of the ``small demands'' is congested and those demands are better served on a different path. Finding demands that result in such sub-optimalities can be tricky: although at first glance one may think increasing the small demands to the threshold should increase the optimality gap (moving more of the demand away from the optimization's control), this is not the case --- in the example in the left of figure~\autoref{f:pinning_issues} increasing the demand between nodes 5 - 4 to the threshold reduces the optimality gap.  While these examples are illustrative, the broader impact of these (or other) concerns on larger and more practically relevant topologies is unclear.

	%\caption{Shows the sub-optimal performance of a deployed heuristic. Values above edges show directional link capacities. The heuristic first sends those demands that fall below a given threshold over their shortest paths and then solves an optimization problem to route the remaining demands over their K-shortest paths. Left hand side example: a scenario where the small demands use-up capacity on multiple hops resulting in sub-optimality. Right hand side example: a scenario where the small demands cause congestion thus resulting in sub-optimality.\label{f:pinning_issues}}%\vspace{-0.05in} 
%	\vspace{-4mm}
%\begin{figure}
%	\includegraphics[width=0.9\linewidth]{figs/MetaOpt-Usecase.pdf}
%	\caption{XXX \pooria{Will fix the colors later.} %\santi{I think that this figure has some issues (see text). In any case, if we keep it, please notice that the blocks on the right should say HEU instead of HUE.}
%		 \ryan{I would vote for cutting this figure. I don't know what it is adding and the text barely refers to it.}}
%	\label{f:metaopt-usecase}
%\end{figure}
 
%\vspace{0.03in}



\vspace{0.03in}
Our main contribution is \emph{a method that can provably find the input that leads to the largest gap between a heuristic and an optimal solution and supports a rich class of additional constraints on the inputs that practitioners can specify to define realistic scenarios}. We further enable operators to pose queries to the method and to compare different heuristics.  

It is hard to find adversarial inputs that lead to a large optimality gap because we have to reason about both the heuristic and optimal algorithm simultaneously. We found naive search techniques based on standard stochastic methods, such as simulated annealing, yield poor results (see~\secref{s:eval}). Instead, in \metaopt we view the adversarial input problem as its own \emph{multi-level} optimization problem -- namely, the problem may be thought of as finding inputs that optimize the gap created from optimizing the two separate problems. We formulate this as
%
%The problem of searching for adversarial inputs with the largest gap can itself be formulated as an optimization problem:
%
\begin{equation}
\arg\hspace{-12mm}\max_{{\text{s.t. input} \,\, \mathcal{I} \in {\sf ConstrainedSet}}}   {\sf OPT}(\mathcal{I}) - {\sf Heuristic}(\mathcal{I}),
\label{eqn:adversarial_outer}
\end{equation}
%
where ${\sf OPT}()$ and ${\sf Heuristic}()$ are solutions to the optimal and heuristic algorithms, the input is $\mathcal{I}$, and ${\sf ConstrainedSet}$ contains constraints on the feasible inputs.
%\srikanth{Just minor rewording here: is it our key insight to write out this two-level opt? I think the following may be better things to call out.}

One can interpret the solution to \eqnref{eqn:adversarial_outer} through the lens of game theory as a Stackelberg equilibrium~\cite{sGames}, where the {\em outer} problem (or leader) picks an input, and the {\em inner} followers maximize ${\sf OPT}$() and ${\sf Heuristic}$() individually in response to the leader's choice. We can model games using two-level optimizations~\cite{bilevel_survey} that existing solvers~\cite{Z3,gurobi} do not support.
We show how to translate the two-level optimization into a single-shot optimization that off-the-shelf solvers can solve (~\secref{s:methods}). 


Solving the adversarial input problem is at least as hard as solving both the optimal and heuristic optimizations together: we scale \metaopt beyond small problem sizes through a clustering technique that decomposes the optimization into several smaller subproblems. \metaopt finds inputs that maximize the gap between the heuristic and the optimal (at the cluster-level) within each cluster in parallel; adds these inputs as {\em constants} to the original, larger, problem; and finds the remaining inter-cluster inputs such that it finds the largest gap in the full problem (subject to the fixed intra-cluster inputs).  We can apply this scaling technique to any graph-based heuristic.


% We discuss support for heuristics that take random decisions~(e.g., {\pop}~\cite{pop}) and those that take conditional actions and may not appear at first blush to be convex~(e.g., {\dempin}~\cite{blastshield}) so they fit within this framework. We show how to use the tool to compare heuristics, to combine them, and to understand why a particular input causes a high optimality-gap.

To demonstrate {\metaopt} is general, we show how to apply it to heuristics in vastly different domains: vector bin packing~\cite{VBP-Heuristics,tetris} and traffic engineering.
\metaopt shows the optimality gap of both \dempin and \pop is higher (by {\color{red}XXX}) than what either work reports~\cite{blastshield, pop}; helps identify how to improve \dempin to reduce its optimality gap (by up to $12.5$x); proves a tighter bound for the performance of a vector bin packing heuristic than what, to the best of our knowledge, has been theoretically proven to date (by up to $2$x); and outperforms local search methods~---~it finds larger gaps ($1.7$x~-~$17x$)  while reducing the search time by orders of magnitude.
% We show that our approach has merit in~\xref{s:eval} where we 
We are unaware of any prior work that finds provably strong adversarial examples for heuristics. 
%\ryan{we should state some high-level results. don't we have new results for bin packing, and some new ones for demand pining etc. How much better we did than stochastic search. Something punchy here.}
\behnaz{@Pooria, fill in the numbers please.}

%\ryan{didn't you also discover a better demand pining heuristic?}
}


==> texfiles/methods.tex <==
\section{Finding Adversarial Inputs}
\label{s:methods}

%MetaOpt is a heuristic analysis tool that not only allows operators to find worst case optimality gaps but also to find realistic inputs that result in bad outcomes and to compare different heuristics. We now explain how MetaOpt achieves this.

%We next describe how we build MetaOpt: a tool that not only allows operators to find worst case optimality gaps but to also find realistic inputs that result in bad outcomes and to compare different heuristics. 

One can search for adversarial inputs using \emph{black-box} methods such as simulated annealing. These algorithms repeatedly select a new input, evaluate both the optimal and heuristic on that input, and use the result to guide the next step. But these methods can be slow in practice~(\secref{s:eval}): they ignore the inner workings of the heuristic and the environment (\eg the network topology), can converge to local optima, and lack optimality guarantees.
We introduce {\metaopt}, a novel {\em white-box} approach that finds the worst-case adversarial inputs and overcomes these limitations.

We observe this problem is similar to a game between a leader and two or more followers. In this game, the leader decides on the inputs for the followers, who then optimize their own objectives based on those inputs. The outcome of the followers determines the leader's reward. In our TE example, the leader (also referred to as outer problem) wants to find the demand that causes the largest difference between the optimal and the heuristic's objective. Meanwhile, each follower (\eg the optimal form and the heuristic) strives to maximize its satisfied demand.

%We can apply this idea to any heuristic but to find the equilibrium the heuristic has to be either convex or written as a set of feasibility constraints~\cite{boyd_co}. Notice the optimal form need not be convex: we can apply this technique to a qualifying heuristic as long as we can write the optimal form as any type of optimization (convex, non-convex, linear, non-linear, or mixed-integer). 

Game theorists refer to this problem as a Stackelberg game~\cite{sGames} and formulate it as a two-level optimization. In this paper, we show how to solve this two-level optimization at scale and find adversarial inputs for a variety of heuristics in WAN TE and vector bin packing. We also illustrate how to use this approach to improve existing heuristics.

 We can  use \metaopt to answer other, more complex, queries about the heuristic: How does it compare to other heuristics? How does it perform under realistic constraints? What sets of inputs does it perform well (or poorly) on? How does a combination of heuristics compare to each individually? as well as others (see~\S\ref{ss:extensions}).
%{\metaopt} is generally faster, finds higher quality gaps (as well as optimal) compared to black box techniques.

%ur method uses the Primal-Dual and the KKT theorems~\cite{boyd_co} to rewrite the two-stage game as a single-shot optimization, can be implemented in existing solvers, is generally faster, and finds higher quality (as well as optimal) gaps compared to black-box approaches. 

%A direct approach to find adversarial inputs is \emph{black-box} search algorithms such as simulated annealing~\cite{simulated_annealing}. They iteratively select a new input, execute optimal and heuristic solvers on that, and then use the gap to guide future iterations. Black-box solutions are, however, slow in practice~\secref{s:eval}. We present a novel \emph{white-box} approach applicable whenever ${\sf OPT}()$ and ${\sf Heuristic}()$ are representable as convex optimizations. Our method uses the KKT theorem~\cite{boyd_co} to rewrite the two-stage game as a single-shot optimization, can be implemented in existing solvers, is generally faster, and finds higher quality (as well as optimal) gaps than black-box approaches. 

% We need to first decide between: blackbox approaches that can support any arbitrarily specified optimal algorithm/heuristic; whitebox approaches that require intimate knowledge of the inner workings of both the heuristic and optimal solutions; or alternatively greybox solutions which are a tradeoff between the earlier two approaches and require only partial knowledge of the heuristic/optimal solutions.

%\noindent {\bf Blackbox approaches:} We can support any arbitrarily specified optimal algorithm and heuristic (e.g., code binary) by blackbox techniques as they do not need to know the specifics of how either the heuristic or optimal form are encoded.  


%\noindent{\bf Whitebox approaches:} These require intimate knowledge of the inner workings of both the heuristic and the optimal solutions and (in certain cases) that they be amenable to the requirements of the search algorithm.

%\noindent{\bf GreyBox approaches:} These are a tradeoff between whitebox and blackbox approaches and require only partial knowledge of the heuristic/optimal solutions.

% While blackbox approaches are general and apply to a more diverse set of problems they tend to be slower (see~\autoref{s:eval}). On the other hand, whitebox approaches tend to be more performant but are far less general and may not apply to all heuristics. Greybox approaches pose a good compromise but are far trickier to get right as they require identifying properties of the heuristic/optimal problem which the search process can then exploit to find a solution more efficiently. 



% We explore the efficacy of both blackbox and whitebox approaches. We show how blackbox solutions can be too slow in practice (see~\autoref{s:eval}). We then describe a white-box approach. We offer a technique using KKT~\cite{boyd_co} rewrites that runs on commodity solvers, is generally faster, and can find higher quality (as well as optimal) gaps compared to blackbox approaches. 

%\subsection{Goals and Scope of applicability}
%\label{ss:scope}

%\vspace{0.07in}
\parab{{\metaopt}'s formulation.} 
\eqnref{eq:metaopt_full} shows the complete \metaopt formulation. 
It is a two-level (bilevel) optimization where the optimal and heuristic algorithms are embedded within an (outer) optimization. The leader (outer problem) seeks realistic inputs that maximize the difference between optimal and heuristic. The first set of constraints, ${\sf ConstrainedSet}$, restrict {\metaopt}'s search space to make sure the inputs it finds are practical. Users specify the \opt and \heur functions (which themselves can be optimization problems with their own set of constraints).
These are followers in the Stackelberg model that map the input, $\mathcal{I}$, to solutions that satisfy the constraints (\eg ${\sf FeasibleFlow}$~\eqref{eq:feasible_flow}) and maximize (or minimize) their objective (\eg ${\sf OptMaxFlow}$~\eqref{eq:max_flow}).

%${\sf OPT}()$ in TE is a multi-commodity flow problem~\eqref{eq:max_flow}. Some example ${\sf HEURISTIC}()$ in TE are \dempin~\eqref{eq:dp_max_flow} and \pop~\eqref{eq:pop_max_flow}.

{\small
	\begin{alignat}{3}
		\label{eq:metaopt_full} 
		\mbox{\sf AdversarialInput}() \triangleq & &\\
		\arg\max_{\mathcal{I}}{\sf OPT}(\mathcal{I}) - {\sf Heuristic}(\mathcal{I}) && \quad\text{(leader or outer problem)} \nonumber \\
		\mbox{s.t.} \quad {\mathcal{I} \in {\sf ConstrainedSet}} && \quad\text{(input constraints)}\nonumber
	%	{\sf OPT}: \mathcal{I} \mapsto \mathbb{R} && \quad\text{(optimal follower)} \nonumber\\
	%	{\sf Heuristic}: \mathcal{I} \mapsto \mathbb{R} && \quad\text{(heuristic follower)} \nonumber
\end{alignat}}
%\srikanth{Do not see value from the last two equations above.}
\pooria{The last two constraints explicitly show what we mean by optimal and heuristic followers (that we repeatedly use in the next few sections).}

In our TE example (\secref{s:background}), ${\sf OPT}()$ finds the optimal solution to a multi-commodity flow problem (\eqnref{eq:max_flow}) and ${\sf HEURISTIC}()$ is one of \dempin (\eqnref{eq:dp_max_flow}) or \pop (\eqnref{eq:pop_max_flow}).
%\santi{It is a bit confusing to have AdversarialInput as a function of I, right? this is not a function of I}
%\santi{In this equation and others you are using very small font. I understand it in some previous equations were you needed the smaller font to make things fit, but you should consider whether you want to use normal font in the case where things would fit.}
%\ramesh{Metaopt formulation. Don’t draw attention to the formulation first. Give an intuitive description of the key idea: using a solver to search for an input that maximizes the difference between OPT and HEURISTIC. With that description, point out that it is general: not specific to TE, but can work for many settings (forward reference to bin packing). Then introduce the formulation (7), but avoid terminology from the optimization literature ("inner problems") if possible. In this, it is also OK to omit the constraints and simply focus on the objective function (i.e., (1)) to make it easier to read.}

\parab{Scope of applicability.} 
%We can apply~\eqnref{eq:metaopt_full} to any heuristic but to solve the two level optimization, the heuristic must be expressed either convex or written as a set of feasibility constraints: MetaOpt applies when we can write (or transform) a heuristic into either a feasibility problem or a convex optimization. We show we can transform a broad class of heuristics (randomized and those which take conditional actions  -- {\pop} and {\dempin}) into convex optimizations\footnote{In~\secref{}, we show how we can represent a greedy heuristic such as First-Fit Decreasing (FFD) used to solve Vector Bin Packing~\cite{VBP-Heuristics} as a feasibility problem. \pooria{todo: fill in the blanks.}}.
We can use~\eqnref{eq:metaopt_full} to analyze any heuristic but, to use existing solvers~\cite{gurobi}, we must express the heuristic either as a convex optimization or as a set of feasibility constraints.

\opt can take any form as long as existing solvers support it. For example, Gurobi~\cite{gurobi}, a popular solver, can solve non-convex quadratic constraints and objectives, including bilinear and quadratic equality constraints, as well as linear, non-linear, or mixed-integer problems.

In~\secref{ss:convexify}, we show how to transform a broad class of heuristics, including randomized ({\pop}), those which take conditional actions ({\dempin}), and sequential heuristics ({\ffd} in vector bin packing~\cite{VBP-Heuristics}) into an appropriate form.


\parab{Scale.} It is harder to solve the two-level optimization in~\eqnref{eq:metaopt_full} compared to either of the optimal or heuristic problems. But we only need to run {\metaopt} offline to analyze a heuristic: we can tolerate higher runtimes compared to real-world applications of the heuristics. Even so, we use optimization techniques (in the general case) and domain knowledge (for graph-based networking heuristics) to improve \metaopt's ability to scale and its run-time performance (see~\secref{ss:cluster}). Some of these techniques introduce approximations (\secref{ss:convex-follower}, \secref{ss:cluster}); in these cases, \metaopt may not produce a worst-case input, but quickly finds adversarial ones.

To identify inputs that have large gaps, we do not have to solve {\metaopt} to completion but rather only must find large gaps quickly.

For a more fuller analysis, such as to bound the worst-case performance, we have to run {\metaopt} to completion. We can do this in small problem instances.

For much larger graphs, we use approximating techniques.

%\metaopt applies whenever the heuristic is transformed into either a feasibility problem or a convex optimization.
%We show that a broad class of heuristics (randomized and those that take conditional actions -- {\pop} and {\dempin}) can be specified as convex optimizations\footnote{In~\secref{}, we show how a greedy heuristic such as First-Fit Decreasing (FFD) used to solve Vector Bin Packing~\cite{VBP-Heuristics} can be represented as a feasibility problem. \pooria{todo: fill in the blanks.}}.
%Finding adversarial gaps as in~\eqref{eq:metaopt_full} is more complex than the underlying optimal algorithms and heuristics; thus, scalability and timeliness are valid concerns. 
%However, in practice, we only invoke gap finding on each new heuristic to better understand its limitations and so timeliness is a less stringent constraint.
%In fact, all the results in this paper finish within an hour.


%Although the overall problem in~\eqref{eq:metaopt_full} is larger (in terms of constraints and variables) than the underlying problems,
%we show that the key computational challenge stems from the non-linear (convex) constraints introduced by the Primal-Dual and the KKT rewrites. To scale to large problem sizes, we leverage our domain knowledge in traffic engineering and exploit the clustered structure of WAN topologies; see~\secref{ss:cluster}.
%Thus, we report results on small albeit practical topologies. Scaling to larger topologies remains an open problem; see~\secref{s:discuss}.

%We also show that the size of the metaoptimization to find adversarial gaps is within one order of magnitude of the underlying problems in terms of numbers of constraints and variables. The key computational challenge, as we will show in~\xref{s:eval}, 

% Although the proposed white-box approach requires knowledge of the optimal solver and the heuristic, our formulation is not specific to a given heuristic but rather encompasses the broad sub-class of heuristics and optimal algorithms that can be stated as convex problems.

%\ramesh{Applicability discussion. The second and third paras in this discussion don’t seem to be about applicability, unless by applicability we mean scalability and timeliness. I also didn’t understand the sentence "However, in practice..": In practical use cases, isn’t timeliness important. The 3rd para about the key computational challenge can be omitted because we are getting there next in 3.1?}



\begin{figure}[t]
\begin{center}
\begin{tikzpicture}[->,>=stealth']
	\node[state,
	      text width=3.3cm] (A) 
	{\begin{tabular}{l}
		\textbf{min}$_{w, \ell}$ $\big( w^2 + \ell^2 \big)$\\[.5em]
		$2 \cdot (w + \ell) \geq P$ \\
		$P \geq 0$ \\
	\end{tabular}};
		
	\node[state,
		text width=3.2cm,
		right of=A,
		yshift = -1.1cm,
		node distance=4.8cm,
		anchor=center] (B)
	{%
	{\begin{tabular}{l}
		\textbf{solve} for $w, \ell, \lambda$\\[.5em]
		$2 (w + \ell) \geq P$ \\
		$P \geq 0$ \\
		$\lambda \geq 0$ \\
		$2w - 2\lambda = 0$ \\
		$2\ell - 2\lambda = 0$ \\
%		$\big( \lambda = 0 \big)$ or \\
%		$~~~~\big( w + \ell - \frac{P}{2} = 0 \big)$ \\
		\fcolorbox{myp}{myp}{$\lambda\big( w + \ell - \frac{P}{2} \big) = 0$}\\
	\end{tabular}}
	};
	
	\node[state,
		below of=A,
		yshift=-1.4cm,
		fill={rgb,255:red,222;green,226;blue,255},
%		fill=cyan!20,
		anchor=center,
		text width=3.6cm] (C) 
	{%
	{\renewcommand{\arraystretch}{1.3}
%	\begin{tabular}{p{2.6cm}}
%		$w = \frac{P}{4}$, $\ell = \frac{P}{4}$  \\ \hdashline
%		$\lambda = \frac{P}{4}$ \\
%	\end{tabular}
	\begin{tabular}{p{1.8cm} p{1.2cm}}
		$w = \ell = \frac{P}{4}$  & $\lambda = \frac{P}{4}$ \\
	\end{tabular}}
	};
	
	\path (A) 	edge[bend left=20]  node[anchor=south,above]{KKT}
									node[anchor=north,below]{encode} (B)
	(A)     	edge[bend right=20] node[anchor=south,right]{optimize}   (C)
	(B)       	edge[bend left=20]  node[anchor=south,above]{solve}      (C);
	
	\end{tikzpicture}
\end{center}
\caption{{\label{f:eg_conversion} Example optimization. Minimize the diagonal length of a rectangle with width $w$ and length $\ell$ whose perimeter $\geq P$. We convert the inner optimization (top left) into a feasibility problem using the KKT theorem. The equations with $\lambda$ variables correspond to first order derivatives of inequality constraints in the original problem. The perimeter $P$ is a variable to an outer optimization but is treated as a constant in the inner problem.}}
\end{figure}

\begin{figure}[t]
\begin{center}
	\begin{tikzpicture}[->,>=stealth']
		\node[state, text width=2.9cm, label=Primal-dual] (A)
		{
			{
				\small
				\begin{tabular}{l}
					\textbf{solve} for $w, \ell, \lambda$\\[.5em]
					\fcolorbox{mygreen}{mygreen}{$2 (w + \ell) \geq P$} \\
					\fcolorbox{myb}{myb}{$\lambda \geq 0$} \\
					$P \geq 0$ \\
					\fcolorbox{myp}{myp}{$P \lambda -2 \lambda^2 = w^2 + \ell^2$}
				\end{tabular}
			}
		};
		
		\node[state,
		text width=3.6cm,
		right of=A,
		% yshift = -0.3cm,
%		align=left,
		node distance=5.05cm,
		anchor=center, label=Quantized Primal-dual] (B)
		{%
			{
				\small
				\begin{tabular}{l}
					\textbf{solve} for $w, \ell, \lambda$\\[.5em]
					\fcolorbox{mygreen}{mygreen}{$2 (w + \ell) \geq P$} \\
					\fcolorbox{myb}{myb}{$\lambda \geq 0$} \\
					$x_j \in \{0,1\} \,\, \forall j \in \{0, \dots, Q\}$\\
					\fcolorbox{myp}{myp}{$\sum\limits_{j=0}^{Q}{L_j z_j} -2 \lambda^2 = w^2 + \ell^2$}\\
					\fcolorbox{myp}{myp}{$z_j = \lambda x_j \,\, \forall j \in \{0,\dots,Q\}$}
				\end{tabular}
			}
		};
		% \draw [-stealth](2.1,-1) -- (3.7,-1);
		
		% \path (A) 	edge[yshift=-0.5em]  node[anchor=south,above]{$P = L_1x_1$} node[anchor=north,below]{} (B);
		% (A)     	edge[bend right=20] node[anchor=south,right]{optimize}   (C)
		% (B)       	edge[bend left=20]  node[anchor=south,above]{solve}      (C);
		\begin{scope}[transform canvas={yshift=-3em}]
			\draw [->] (A) -- node[anchor=north,above] {{\footnotesize $P = \sum\limits_{j=0}^{Q}{L_j x_j}$}} (B);
		\end{scope}
	\end{tikzpicture}
\end{center}
\caption{XXXX.\label{f:pd_conversion}}
\end{figure}

%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.8\linewidth]{figs/KKT_v3.png}\vspace{-0.1in}
%\begin{subfigure}[b]{3in}
%\boxalign{\footnotesize
%\begin{alignat}{1}
%\max_{x,y} \quad y - x \quad \quad \nonumber\\
%\mbox{ s.t. } \quad x + 2y = t \quad\nonumber\quad \\
%\quad 0 \le x \le d \quad \nonumber \quad \\
%\quad 0 \le y \le d \quad \nonumber \quad
%\end{alignat}
%}
%\caption{An example convex optimization problem\label{f:eg_convex_opt}}
%\end{subfigure}
%\hfill%
%\begin{subfigure}[b]{3in}
%\centering
%\boxalign{\footnotesize
%\vspace{0.05in}
%$\ \ \ \ \ \ \ \ \ \ \ \ \exists\  x, y, \lambda_1, \lambda_2, \lambda_3, \lambda_4, \nu \ \  \mbox{ s. t. } $\\[-0.05in]
%\begin{minipage}{.3\linewidth}
%\begin{alignat}{1}
%\quad x + 2y = t \quad\nonumber\quad \\
%\quad 0 \le x \le d \quad \nonumber \quad \\
%\quad 0 \le y \le d \quad \nonumber \quad
%\end{alignat}
%\end{minipage}
%\begin{minipage}{.5\linewidth}
%\begin{alignat}{2}
%\quad x\lambda_1 \quad= 0  \quad \nonumber\\
%\quad (d-x)\lambda_2 \quad = 0\quad \nonumber\\
%\quad y\lambda_3 \quad= 0 \quad \nonumber\\
%\quad (d-y)\lambda_4 \quad= 0\quad \nonumber\\
%\quad -1-\lambda_1 - \lambda_2 +\nu \quad= 0\quad \nonumber\\
%\quad 1 - \lambda_3 - \lambda_4 + 2\nu \quad= 0 \quad \nonumber \\
%\quad \lambda_1, \lambda_2, \lambda_3, \lambda_4 \quad\ge 0\quad \nonumber
%\end{alignat}
%\end{minipage}
%}
%\caption{Conversion to a set of constraints using the KKT theorem.\label{f:eg_convext_opt_kkt}}
%\end{subfigure}
%\caption{\label{f:eg_conversion} Showing KKT conversion; we convert the inner optimizations in Eqn.~\ref{eqn:adversarial_outer} into a feasibility problem using the KKT theorem. The inequalities in the original problem lead to multiplicative constraints. The optimal answer is $(x, y, \lambda_1, \lambda_2, \lambda_3, \lambda_4, \nu) = (0, \frac{t}{2}, \frac{1}{2}, 0, 0, 0, \frac{1}{2})$. The equations with $\lambda$ variables correspond to inequality constraints in the original problem and the equations with the $\nu$ variable are the partial derivatives with respect to the variables of the inner optimization. The values $d$ and $t$ may be variables to the outer optimization but are constants in the inner problem --- we do not need to take partial derivatives corresponding to those variables in order to compute KKT constraints.}
%\vspace{-3mm}
%\end{figure}

\subsection{\metaopt, an overview}
\label{ss:sso}

%To our knowledge, no commodity solver directly solves two-stage optimization problems. This may not be a problem for many heuristics: we can write some followers (heuristics and their optimal form) as a set of feasibility constraints~\cite{boyd_co}; in other cases the followers' objective may align with the leader and so we can directly merge the two problems~---~ this is always true for ${\sf OPT}()$ if it is a maximization.
%But when the followers don't fall in either of these categories we need to reformulate the problem in~\eqref{eq:metaopt_full} as a single-shot optimization:

To find adversarial inputs we need to solve the {\metaopt} two-level optimization at scale . 
To our knowledge, existing solvers~\cite{gurobi,Z3} cannot directly handle multi-level optimization problems like the one in~\eqnref{eq:metaopt_full}.  \metaopt converts the problem into a single-shot optimization to overcome this. We next discuss the overall approach and how \metaopt can do this for followers with different mathematical properties.



We replace the followers (optimal and heuristic) with sets of constraints. This simplifies the problem and makes it a single-level optimization that we can solve with existing solvers. The key challenge is to ensure that these sets of constraints reflect the original behavior of the follower. 

The follower's objective can either align with the \metaopt objective or not. Each follower is also either convex or non-convex. We handle each of these cases as follows:



\parab{Optimization with aligned objective.} If the follower is an optimization whose objective aligns with the leader, we can easily capture its behavior: we can include the constraints from the follower into the leader's optimization. This is possible because the leader's objective ensures the follower remains optimal. For example, in~\eqnref{eq:metaopt_full} both the optimal follower and the leader want to maximize flow. In this case, we can take the constraints from the optimal algorithm and add them to the outer problem without any modification. \metaopt can perform this transformation automatically.


%\santi{I am not entirely sure why we frame the paragraph above under `matching objectives'. Isn't what we are saying there true about \opt in general?}
%\pooria{Thanks for the comment, Santi. Yes, what we are saying is true about \opt based on the objective in~\eqnref{eq:metaopt_full}. But, for example, if we change the objective such that we maximize HUE - OPT to find cases where HUE actually works as well as OPT. Then, we can not apply this to OPT anymore, and should apply it to HUE instead. In another case, if we are comparing two heuristics ($HUE_1 - HUE_2$), we can apply the trick to heuristic 1. I think a general discussion would help when people are using these tricks in the future, and OPT in~\eqref{eq:metaopt_full} can provide an example of how this applies. Please let me know if this makes sense.}
%\ramesh{Santi's point is a good one. The distinction you make Pooria might be too detailed to bring out here. It might, however, be OK to keep the framing as is to contrast with the next para. I tweaked the text below to make this clear.}

\parab{Convex optimization.} Sometimes, a follower's objective is not aligned with the leader's. For example, in~\eqnref{eq:metaopt_full}, the \heur follower attempts to maximize its maximum flow, but the leader does not. If the follower is a convex optimization problem, we can build upon prior work~\cite{boyd_co,bilevel_survey} to \textit{rewrite the follower} as a set of constraints that represent the behavior of the follower. \metaopt can perform these rewrites automatically from, for example, the user-specified \heur. We discuss convex follower rewriting in \secref{ss:convex-follower} and show how rewriting applies to \pop and \dempin in \secref{ss:convexify:te}.


% These constraints represent the behavior of the follower and any solution that satisfies them is guaranteed to be optimal in the original formulation. We use these techniques to translate convex heuristics such as {\dempin} or {\pop} in~\eqnref{eq:metaopt_full}. 

\parab{Non-convex optimizations.} If the follower's objective is not aligned with the leader's and if it is not a convex optimization, \metaopt requires the user to encode the follower directly as a feasibility problem, and add the constraints to the leader's optimization. \secref{ss:convexify:vbp} illustrates this for the non-convex heuristic {\ffd}~\cite{VBP-Heuristics} for vector bin packing.

%\santi{The wording of the paragraph above feels like it says `If the other two does not work, then we can do this and it will work', which is probably not the message we want to send since many things cannot be encoded in any of these ways, right? Maybe we can word it as `Another set of heuristics can be encoded directly as a feasibility problem ...'}
%\ramesh{Made it clearer, please review.} 
\ryan{We almost need a table or something to enumerate the different set of requirements. Hard for a reviewer to keep all of this straight.}


%\parab{Reformulating ${\sf OPT}()$.} Both ${\sf OPT} ()$ and the leader (outer problem in~\eqref{eqn:adversarial_outer}) want to maximize the ${\sf OPT}()$: the leader so it maximizes the gap between ${}\sf OPT()$ and the heuristic and ${\sf OPT}()$ so it maximizes its objective (if ${\sf OPT}()$ is a minimization we can convert it to an equivalent maximization). This means we can just take the constraints in the ${\sf OPT}()$ and add them to the outer problem (without any modification).

%We can add ${\sf OPT}()$'s constraints directly to the outer problem~\eqref{eqn:adversarial_outer} without any other modification since the objective of the inner problem ${\sf OPT}()$ is aligned with the outer problem; Both are trying to maximize the ${\sf OPT}()$'s solution and therefore, optimality of ${\sf OPT}()$ is guaranteed.


%\parab{Reformulating ${\sf HEURISTIC}()$.} To convert the heuristic into a set of constraints we have multiple options: if we can write the heuristic as a feasibility problem, we can directly take the constraints and add them to the outer problem; if not, we can use the KKT theorem~\cite{boyd_co} or the Primal-Dual method~\cite{bilevel_survey} to convert it to a set of constraints~---~ any point that satisfies the new constraints is also optimal in the original formulation as long as the original form is convex~\cite{boyd_co}. 



%\metaopt currently supports heuristics that are written either in a feasibility format or a convex optimization. For the former, we add the feasibility constraints directly to the outerproblem~\eqref{eqn:adversarial_outer}. For the latter, we reformulate and replace them with sets of feasibility constraints that guarantee the optimality of inner problems~\cite{bilevel_survey}. Leveraging the properties of convex optimizations, we derive two such transformations; KKT encoding and Primal-Dual encoding.

\section{The \metaopt solution}
\label{sec::solution_details}
\behnaz{@Pooria make sure the references match this change.}
\behnaz{I don't know what title would work better here.}

\metaopt converts the two-level optimization~\ref{eq:metaopt_full} into a single-shot optimization. When the follower's objective aligns with the \metaopt objective (the outer problem) or when its a set of feasibility constraints, \metaopt just ports the follower's constraints into the outer problem (see~\S\ref{ss:sso}). 

It takes more work to convert the remaining followers whose objectives do not align with the outer problem and are not a set of feasibility constraints. 
We next describe how \metaopt converts these followers (see~\S\ref{ss:convex-follower}) and then describe how we scale the overall solution (see~\S\ref{sec:solverscale} and~\S\ref{ss:cluster}).

\subsection{Rewriting Convex Followers}
\label{ss:convex-follower}
%\srikanth{May be start with this section, as `building blocks' and then present the overall approach? Not sure.}
%\pooria{This section is written based on the linear example I discussed yesterday. We need to update the example or we need to update the text. My handwritten version of the lp is under "figs/Example-linear.jpg"}
%\srikanth{Pooria, can we not use the figure 3 example for primal-dual and primal-dual quantized? If we can, i'd prefer to do that. You could add the primal-dual and primal-dual quantized as separate figures.}
%\pooria{Sure.}

If a follower is not a set of feasibility constraints and its objective does not align with the outer problem then it has to be convex: if not \metaopt cannot convert the two-level optimization into a single-shot problem.

To rewrite a convex follower, we need to convert it into a set of feasibility constraints. In this section, we first describe existing techniques for rewriting and then describe how \metaopt adapts these to scale to larger problem sizes.

\parab{Prior approaches to rewriting.}
The optimization literature has developed two main approaches to rewriting convex optimizations: \textit{Karush–Kuhn–Tucker (KKT)} and \textit{primal-dual}. 

\parae{KKT rewrite.} 
Based on the $KKT$ theorem~\cite{boyd_co}, this rewrite can convert any convex optimization with at least one strictly feasible point, into a set of feasibility constraints. \figref{f:eg_conversion} illustrates this rewrite. In this example, the original optimization finds the rectangle with the longest diameter ($w^2 + l^2$) where the perimeter is greater than some positive {\em constant} value $P$. The KKT rewrite produces a set of feasibility constraints (\figref{f:eg_conversion}). When a convex optimization has at least one strictly feasible point (Slater's condition~\cite{boyd_co}), this rewrite is \textit{exact}~---~a feasible solution to the rewrite is an optimal solution to the original problem.

\parae{Primal-dual rewrite.} Every (primal) optimization has a corresponding dual. This rewrite technique relies on a well-known relationship between the two: the strong duality theorem~\cite{boyd_co} which states that any feasible point of a convex problem is optimal if and only if the primal objective at that point is the same as the dual objectives. The primal-dual rewrite converts a convex optimization into a set of feasibility constraints that include: the feasibility constraints of the primal (green background in \figref{f:pd_conversion}), the feasibility constraints of the dual (blue background), and a constraint that encodes the strong duality theorem~---~the primal objective has to match the dual objective (light red background). The primal-dual rewrite is also exact.



\parab{Performance of exact rewrites.} The KKT rewrite of the two-level optimization (\eqnref{eq:metaopt_full}) scales poorly. For example, with the KKT rewrite \metaopt can analyze \dempin with a topology of $N$ nodes. The primal-dual rewrite is better~---~we can analyze \dempin with a topology of $M$ nodes~---but still not good enough.\ramesh{Pooria, please fill in the numbers.}

\metaopt could have significant value if it could help analyze heuristics at practical problem sizes. To enable this we explore \textit{approximate rewrites} which allow \metaopt to scale to topologies with over $L$ nodes (we later show how to go even larger topologies through a clustering solution). With the approximate re-write we can produce high quality solutions but we can no longer guarantee they are optimal.
\behnaz{replace L @Pooria}



Users can use \metaopt in two modes: an \textit{exact} mode in which they find worst-case inputs to heuristics for small problems, and an \textit{approximate} mode, in which they quickly find adversarial inputs for larger problem sizes using approximate rewrites. This latter mode leverages an important property of today's commodity solvers: they can find a near-optimal solution quickly (\secref{ss:other-considerations}).

\parab{Approximate rewrites in \metaopt}. At a high-level, \metaopt uses primal-dual to rewrite convex followers. In two-level optimizations, primal-dual rewrites often contain parameters (like $P$ in our example in~\autoref{f:eg_conversion}) that are
constants in the follower, but variables that the leader controls and optimizes. Writing the dual for the \heur requires multiplying terms that contain $P$ ($\mathcal{I}$ in \eqnref{eq:metaopt_full}) with the dual variable which results in non-linear constraints (red background in \figref{f:pd_conversion}\footnote{We use this example for its simplicity. Observe that the the original optimization objective is quadratic which leads to quadratic terms in the primal-dual equality. However, there is a fundamental non-linearity that is introduced by the primal-dual rewrite through the multiplication of $\lambda$ and $P$. This term is present even when the original problem is linear.}).

%Non-linear constraints slow down the optimization. We quantize the space of inputs to remove this non-linearity: once (and only after) we choose a quantile for an input it becomes a constant in the multiplication which then becomes a linear constraint.

% To remove this non-linearity (which otherwise would slow down the solution) we convert it to a decision process which we can then convert to linear constraints.

Non-linear constraints slow down the optimization.\footnote{This also explains why KKT rewrites do not scale, since they also have non-linear constraints (red background in \figref{f:eg_conversion}).} To remove this non-linearity, \metaopt quantizes the space of inputs and converts the non-linear constraints into a specific type of multiplicative constraint, one that multiplies a binary variable with a linear term. \figref{f:pd_conversion} (red background) quantized primal-dual rewrite in which we quantize $P$ into two levels, $0$ and $l_{1}$. $x_{1}$ is the corresponding binary variable (This generalizes to an arbitrary number of quantization levels). \metaopt then uses the big-$M$ approach from standard optimization theory~\cite{boyd_co}, implemented in commodity solvers (\eg~\cite{gurobi}), to convert this term into a linear form. 

%\behnaz{@Pooria, double check simplex applies in our case.}
%\pooria{Summary of our discussion: Simplex theorem guarantees that the worst-case happens at the extremum points which are finite, and if the quantization levels completely capture these points, this approach does not impact the quality of the solution. However, finding all the extremum points can be both computationally challenging and result in scalability problem for \metaopt (in case there are too many independent levels). Hence, we use the most probable quantization levels; ...}

%The Primal-Dual rewrite of ${\sf Heuristic}()$ might generate a nonlinear optimization (as in \figref{}). The nonlinearity appears in the dual objective function because of the product of outer level variable ($\mathcal{I}$ in \eqnref{eq:metaopt_full}) and inner level dual variables.

%\footnote{Multiplicative terms appear in the KKT encoding as well but we can not use the quantization idea since the quantization levels are unknown for KKT multipliers ($\lambda$ in~\figref{f:eg_conversion}).};
%for a subspace of heuristics, we find the worst gaps happen only at extremum points; thus, constraining or quantizing the space of inputs can speedup the search and enables us to linearize the Priaml-Dual rewrite without sacrificing quality. 

%For example, for \pop, demands in the worst-case traffic matrix are either zero or max, and for \dempin, most of the demands are either zero, threshold or max.

% The leader has to pick the quantile~---~the quantiles are variables of the outer problem and we need to enable the outer problem to choose between them as part of the optimization. 
% To quantize an input $d$ into $k + 1$ different levels ($=\{0, L_{1},\dots,L_{k}\}$), we have to add $k$ auxiliary binary variables~---~$x_j$ such that $\sum_{j=1}^{k}x_j \leq 1$~---~and replace $d$ with $\sum_{j=1}^{k}L_{j}x_{j}$. This changes the non-linear term we had initially in the dual objective into a product of two terms: a continuous variable (\ie, the dual variable) and a binary one (\ie $x_{j}$). We can now use a big-$M$ approach to convert this term into a linear form. 
% The big-$M$ approach linearizes a term such as $p = xy$ where $x$ is binary and $y$ continuous as:

% {\small
% 	\begin{eqnarray}
% 	p \geq y - M (1 - x),\,\, p \leq y + M (1 - x), \nonumber \\
% 	p \geq - Mx_i,\,\, p \leq Mx_i, \nonumber
% 	\end{eqnarray}
% }
% where $M$ is a upper bound on $|y|$ and is constant. The first two constraints ensure $p = y$ when $x =1$ and the last two that $p = 0$ otherwise.
% The Gurobi ${\sf Indicator}$ function performs this conversion automatically~\cite{gurobi}.

% \santi{Maybe we can get rid of the equation above and simply mention the big-M approach and put a reference? Not sure if it adds much here.}

The key challenge now is to pick quantization levels that minimally impact solution quality. Our intuition, inspired by the Simplex theorem~\cite{bertsimasLinOptBook}~---~ that proves a similar property for linear programs (ours is a mixed-integer linear program)~---~ is that adversarial inputs occur at the extrema of the feasible set. In \pop, for example, the demands that cause the worst case gap are either zero or max. In \dempin demands that cause the worst case gap are either zero, the \dempin threshold, or max. We can choose the quantization levels from these extrema.


In practice, the set of extrema can be prohibitively large; to scale, \metaopt must use a smaller set of extrema. Our key insight is to use \metaopt itself, with exact rewrites on a smaller problem instance, to find this smaller set of extrema. For TE heuristics, the procedure works as follows:
\begin{enumerate}[nosep,leftmargin=*]
\item Run \metaopt on a smaller instance of the problem using either a KKT or a primal-dual exact rewrite. Our experiments use KKT.
\item Use the worst-case input we find from \metaopt to select the $k$ most frequent demand values as the quantiles and use them in the approximate rewrite. 
\end{enumerate}
$k$ controls the trade-off between scalability and solution quality. For \pop $k = 2$ (zero or max demand), and for \dempin $k = 3$ (either zero, the threshold, or max).

This approach generalizes to other convex heuristics, but a user may need to supply a function for step 2 (extracting quantiles from the worst-case input).

\srikanth{The part above needs a major rewrite for clarity and perhaps correctness.}

\subsection{Scaling through the solver}
\label{sec:solverscale}

To further improve {\metaopt}'s ability to scale we exploit the inner workings of today's commodity solvers: (1) most solvers find a near-optimal (but not optimal) solution quickly; (2) branch-and-bound techniques spend a long time trying to improve this initial solution or to otherwise prove it is optimal; (3) most solvers periodically report their progress towards finding an optimal point or proving optimality. We track this progress over fixed stretches of time. When the incremental progress in a stretch is less than $0.5\%$~---~ Gurobi reports this progress through the primal-dual gap~\cite{boyd_co}~---~we stop the solver and use the solution it has at that point.

Some solvers, \eg Z3~\cite{Z3}, do not report incremental progress.
%~---~SMT solvers such as Z3 are much slower than Gurobi and while we can use them in \metaopt we do not recommend them. \ryan{this comment seems unnecessary. I'm sure there are benchmarks where SMT solvers outperform Gurobi or other solvers, and we don't need to take such a strong position - just show how we can handle both.} 
For these solvers we submit periodic queries and progressively ask for inputs which produce higher gaps (we can use this to do a binary search).  

% We can pick the quantization levels to avoid impact on solution quality. The Simplex theorem~\cite{bertsimasLinOptBook} ensures the inputs that cause the worst case gap happen at the extremum points of the feasibile set (the set of inputs that satisfy all of the constraints in the optimization form a convex set which we call the feasibility set). In \pop, for example, the demands that cause the worst case gap are either zero or max. In \dempin we find the demands that cause the worst case gap are either zero, the \dempin threshold, or max. If we set our quantization levels to be this set of extremum points (which we can use the optimization's constraints to compute) we can use the Simplex theorem to ensure our re-write remains optimum. 

% \santi{The simplex is valid for LP. You can apply it to MILP using branch and bound and relaxations of the MILP. Here, we are trying to put a discussion in general, so I would stay clear of this argument if we cannot make it perfectly formal. The intuition that these extreme adversarial examples would contain extreme demand values make sense. These extremes will in general be related to the constraints defining the heuristic (at that level, that is true in general). And as a generic practical methodology to uncover these important quantization levels we propose the KKT. I think that flow can work. }

% In practice the set of extrema can be prohibitively large and we instead use a subset. We find empirically that if we choose the right subset~---~the ones that are more likely to be optimal~---~we can avoid any impact on solution quality.


% \parab{KKT encoding.} Based on the $KKT$ theorem \textcolor{red}{add ref ... Boyd's book, for example}, we can take an optimization and convert it to a set of feasibility constraints: {\em any} $w$ and $\ell$ in our example that satisfy these constraints are optimal (they maximize the objective) in the original optimization. The result is a feasibility problem (the optimization on the right in~\autoref{f:eg_conversion}) where the objective is to find a feasible point that satisfies the constraints. We can use such KKT rewrites on any convex problem which has at least one strictly feasible point (Slater's condition~\cite{boyd_co}). 

% We prefer convex problems: we can solve convex problems in polynomial time. This is not the case when we use KKT encodings: the multiplicative constraint $\lambda (w + \ell - \frac{P}{2}) = 0$ is not convex (in the multiplicative terms in primal-dual we know the inputs are bounded and we know these bounds and so we can use quantization but in KKT this is not the case). Luckily, commodity solvers support this type of non-convexity~---~ we can encode them using special ordered sets in Gurobi~\cite{gurobi} and disjunctions in Z3~\cite{Z3}. But we now have increased the problem size~(in our example, the $1$ constraint and $2$ variables on the top left increased to $5$ and $3$ respectively on the right) which combined with non-convexity slows down the solver. This is why we use the primal-dual method instead to scale and only use the KKT approach on a small example to quickly find the right quantile levels for primal-dual.

% %

% %\ramesh{The first para of Primal-dual is nice, and can be a model for how to write the KKT intuition. And yes, an example would help.}


% The primal-dual method scales better than $KKT$ because it has fewer binary variables. The number of binary variables in KKT depends on the number of followers and the number of inequality constraints they have. For example, the number of constraints in the \dempin and \pop heuristics depend on the number of paths: if we increase the number of path we increase the number of binary variables we need and reduce the solver's ability to scale! In contrast the primal-dual approach requires only a fixed set of binary variables to quantize the input space.  


\cut{
We next provide some background on Primal-Dual and KKT, and how they apply to our framework. 
For the explanation, we use the example in~\autoref{f:eg_conversion}. 
The optimization maximizes the diagonal ($w^2+\ell^2$) of a rectangle but it can only pick $\ell$ and $w$ that satisfy the constraint that the perimeter is at least $P$, using the constraint $2 (w + \ell) \ge P$. Notice the optimization has no control over $P$~---~ as far as the optimization is concerned $P$ is a constant.

\santi{Small comment: you are using primal-dual and Primal-Dual in lower-case and upper-case. Please choose one (probably lower-case makes more sense) and stick to it.}

\parab{Primal-Dual encoding~\cite{chemKKT}.} The primal-dual relationship states: for any maximization, there is a dual minimization where the objective is always greater than or equal to the primal's objective. The strong duality theorem guarantees any feasible point of a convex problem is optimal iff the primal objective is equal to the dual objective at that point. We use this to replace the inner convex optimizations with two sets of constraints: (1) the primal and dual constraints; and (2) strong duality (primal objective = dual objective); to ensure optimality.

But the primal-dual rewrite is tricky in the context of our two-level optimization. This is mainly because of paramters such as $P$ in our example in~\autoref{f:eg_conversion}: while $P$ is a constant in the follower (inner) problem, it is a variable the leader controls and optimizes. When we write the dual for the ${\sf Heuristic}()$ we have to multiply constraints that contain $P$ ($\mathcal{I}$ in \eqnref{eq:metaopt_full}) with the dual variable, resulting in non-linear constraints.

%Non-linear constraints slow down the optimization. We quantize the space of inputs to remove this non-linearity: once (and only after) we choose a quantile for an input it becomes a constant in the multiplication which then becomes a linear constraint.

% To remove this non-linearity (which otherwise would slow down the solution) we convert it to a decision process which we can then convert to linear constraints.

Non-linear constraints slow down the optimization. 
To remove this non-linearity, we quantize the space of inputs, converting the non-linear constraints into a specific type of multiplicative constraint: one that multiplies a binary variable with a linear term~---~we can use standard optimization theory to linearize such constraints~\cite{boyd_co}.

%\behnaz{@Pooria, double check simplex applies in our case.}
%\pooria{Summary of our discussion: Simplex theorem guarantees that the worst-case happens at the extremum points which are finite, and if the quantization levels completely capture these points, this approach does not impact the quality of the solution. However, finding all the extremum points can be both computationally challenging and result in scalability problem for \metaopt (in case there are too many independent levels). Hence, we use the most probable quantization levels; ...}

%The Primal-Dual rewrite of ${\sf Heuristic}()$ might generate a nonlinear optimization (as in \figref{}). The nonlinearity appears in the dual objective function because of the product of outer level variable ($\mathcal{I}$ in \eqnref{eq:metaopt_full}) and inner level dual variables.

%\footnote{Multiplicative terms appear in the KKT encoding as well but we can not use the quantization idea since the quantization levels are unknown for KKT multipliers ($\lambda$ in~\figref{f:eg_conversion}).};
%for a subspace of heuristics, we find the worst gaps happen only at extremum points; thus, constraining or quantizing the space of inputs can speedup the search and enables us to linearize the Priaml-Dual rewrite without sacrificing quality. 

%For example, for \pop, demands in the worst-case traffic matrix are either zero or max, and for \dempin, most of the demands are either zero, threshold or max.

The leader has to pick the quantile~---~the quantiles are variables of the outer problem and we need to enable the outer problem to choose between them as part of the optimization. 
To quantize an input $d$ into $k + 1$ different levels ($=\{0, L_{1},\dots,L_{k}\}$), we have to add $k$ auxiliary binary variables~---~$x_j$ such that $\sum_{j=1}^{k}x_j \leq 1$~---~and replace $d$ with $\sum_{j=1}^{k}L_{j}x_{j}$. This changes the non-linear term we had initially in the dual objective into a product of two terms: a continuous variable (\ie, the dual variable) and a binary one (\ie $x_{j}$). We can now use a big-$M$ approach to convert this term into a linear form. 
The big-$M$ approach linearizes a term such as $p = xy$ where $x$ is binary and $y$ continuous as:

{\small
	\begin{eqnarray}
	p \geq y - M (1 - x),\,\, p \leq y + M (1 - x), \nonumber \\
	p \geq - Mx_i,\,\, p \leq Mx_i, \nonumber
	\end{eqnarray}
}
where $M$ is a upper bound on $|y|$ and is constant. The first two constraints ensure $p = y$ when $x =1$ and the last two that $p = 0$ otherwise.
The Gurobi ${\sf Indicator}$ function performs this conversion automatically~\cite{gurobi}.

\santi{Maybe we can get rid of the equation above and simply mention the big-M approach and put a reference? Not sure if it adds much here.}

We can pick the quantization levels to avoid impact on solution quality. The Simplex theorem~\cite{bertsimasLinOptBook} ensures the inputs that cause the worst case gap happen at the extremum points of the feasibile set (the set of inputs that satisfy all of the constraints in the optimization form a convex set which we call the feasibility set). In \pop, for example, the demands that cause the worst case gap are either zero or max. In \dempin we find the demands that cause the worst case gap are either zero, the \dempin threshold, or max. If we set our quantization levels to be this set of extremum points (which we can use the optimization's constraints to compute) we can use the Simplex theorem to ensure our re-write remains optimum.

\santi{The simplex is valid for LP. You can apply it to MILP using branch and bound and relaxations of the MILP. Here, we are trying to put a discussion in general, so I would stay clear of this argument if we cannot make it perfectly formal. The intuition that these extreme adversarial examples would contain extreme demand values make sense. These extremes will in general be related to the constraints defining the heuristic (at that level, that is true in general). And as a generic practical methodology to uncover these important quantization levels we propose the KKT. I think that flow can work. }

In practice the set of extremums can be prohibitively large and we instead use a subset. We find empirically that if we choose the right subset~---~the ones that are more likely to be optimal~---~we can avoid any impact on solution quality.

But how do we find such quantization levels? We use the KKT encoding~---~which is slower~---~on a small example: we use the solution to pick the quantization levels for primal-dual. We next describe how the KKT approach works.

\parab{KKT encoding.} Based on the $KKT$ theorem \textcolor{red}{add ref ... Boyd's book, for example}, we can take an optimization and convert it to a set of feasibility constraints: {\em any} $w$ and $\ell$ in our example that satisfy these constraints are optimal (they maximize the objective) in the original optimization. The result is a feasibility problem (the optimization on the right in~\autoref{f:eg_conversion}) where the objective is to find a feasible point that satisfies the constraints. We can use such KKT rewrites on any convex problem which has at least one strictly feasible point (Slater's condition~\cite{boyd_co}). 

We prefer convex problems: we can solve convex problems in polynomial time. This is not the case when we use KKT encodings: the multiplicative constraint $\lambda (w + \ell - \frac{P}{2}) = 0$ is not convex (in the multiplicative terms in primal-dual we know the inputs are bounded and we know these bounds and so we can use quantization but in KKT this is not the case). Luckily, commodity solvers support this type of non-convexity~---~ we can encode them using special ordered sets in Gurobi~\cite{gurobi} and disjunctions in Z3~\cite{Z3}. But we now have increased the problem size~(in our example, the $1$ constraint and $2$ variables on the top left increased to $5$ and $3$ respectively on the right) which combined with non-convexity slows down the solver. This is why we use the primal-dual method instead to scale and only use the KKT approach on a small example to quickly find the right quantile levels for primal-dual.

%

%\ramesh{The first para of Primal-dual is nice, and can be a model for how to write the KKT intuition. And yes, an example would help.}


The primal-dual method scales better than $KKT$ because it has fewer binary variables. The number of binary variables in KKT depends on the number of followers and the number of inequality constraints they have. For example, the number of constraints in the \dempin and \pop heuristics depend on the number of paths: if we increase the number of path we increase the number of binary variables we need and reduce the solver's ability to scale! In contrast the primal-dual approach requires only a fixed set of binary variables to quantize the input space.  



\behnaz{@Pooria, you need to describe this in more detail in an algorithm in the appendix and add a forward ref.}

\parab{Summary.} \tabref{tab:metaopt_rewrite_prop}. \pooria{need to complete this.}
}

\begin{table}
	\scriptsize
	\centering
	\begin{tabular}{|l|l|l|} \hline
		\textbf{\textit{Inner}} & \textbf{\textit{Encoding}} & \textbf{\textit{Properties}} \\ \hline \hline
		${\sf OPT}$ & Direct & \\ \hline
		\multirow{4}{*}{${\sf Heuristic}$} & Direct & applies to heuristics in the feasibility format.\\ \cline{2-3}
		& \multirow{2}{*}{KKT} & applies to heuristics in convex optimization. \\
		&& uses one binary variable per inequality constraint. \\ \cline{2-3}
		& \multirow{2}{*}{Primal-Dual} & applies to heuristic in convex optimization. \\ 
		&& uses binary variables to quantize the input space. \\ \hline
	\end{tabular}
	\caption{Summary of single-shot rewrite in \metaopt \pooria{fill the table}}
	\label{tab:metaopt_rewrite_prop}
\end{table}


% ======================== Begin Cut ====================================
\cut{
To our knowledge, no commodity solver directly solves two-stage optimization problems. This may not be a problem for many heuristics: we can write some followers (heuristics and their optimal form) as a set of feasibility constraints~\cite{boyd_co}; in other cases the followers' objective may align with the leader and so we can directly merge the two problems~---~ this is always true for ${\sf OPT}()$ if it is a maximization.

But when the followers don't fall in either of these categories we need to reformulate the problem in~\eqref{eq:metaopt_full} as a single-shot optimization:
% In this section, we explain how \metaopt reformulates them as a single-shot optimization. The key idea is to replace the inner problems with a set of feasibility constraints that guarantee optimality (\eg the right hand side in~\figref{f:eg_conversion}).

\parab{Reformulating ${\sf OPT}()$.} Both ${\sf OPT} ()$ and the leader (outer problem in~\eqref{eqn:adversarial_outer}) want to maximize the ${\sf OPT}()$: the leader so it maximizes the gap between ${}\sf OPT()$ and the heuristic and ${\sf OPT}()$ so it maximizes its objective (if ${\sf OPT}()$ is a minimization we can convert it to an equivalent maximization). This means we can just take the constraints in the ${\sf OPT}()$ and add them to the outer problem (without any modification).

%We can add ${\sf OPT}()$'s constraints directly to the outer problem~\eqref{eqn:adversarial_outer} without any other modification since the objective of the inner problem ${\sf OPT}()$ is aligned with the outer problem; Both are trying to maximize the ${\sf OPT}()$'s solution and therefore, optimality of ${\sf OPT}()$ is guaranteed.


\parab{Reformulating ${\sf HEURISTIC}()$.} To convert the heuristic into a set of constraints we have multiple options: if we can write the heuristic as a feasibility problem, we can directly take the constraints and add them to the outer problem; if not, we can use the KKT theorem~\cite{boyd_co} or the Primal-Dual method~\cite{bilevel_survey} to convert it to a set of constraints~---~ any point that satisfies the new constraints is also optimal in the original formulation as long as the original form is convex~\cite{boyd_co}. 

We next provide some background on Primal-Dual and KKT and how they apply here. To explain our encodings we use the example in~\autoref{f:eg_conversion}. The optimization maximizes $w^2+\ell^2$ but it can only pick $\ell$ and $w$ that satisfy the constraint $2 (w + \ell) \ge P$. Notice the optimization has no control over $P$~---~ as far as the optimization is concerned $P$ is a constant.

%\metaopt currently supports heuristics that are written either in a feasibility format or a convex optimization. For the former, we add the feasibility constraints directly to the outerproblem~\eqref{eqn:adversarial_outer}. For the latter, we reformulate and replace them with sets of feasibility constraints that guarantee the optimality of inner problems~\cite{bilevel_survey}. Leveraging the properties of convex optimizations, we derive two such transformations; KKT encoding and Primal-Dual encoding.




\parae{Primal-Dual encoding~\cite{chemKKT}.} The primal-dual relationship states: for any maximization, there is a dual minimization where the objective is always greater or equal to the primal's objective. The strong duality theorem guarantees any feasible point of a convex problem is optimal iff the primal objective is equal to the dual objective at that point. We use this to replace the inner convex optimizations with two sets of constraints: (1) the primal and dual constraints; and (2) strong duality (primal objective = dual objective); to ensure optimality.

But the primal-dual rewrite is tricky in the context of our two-level optimization. This is mainly because of paramters such as $P$ in our example in~\autoref{f:eg_conversion}: while $P$ is a constant in the follower (inner) problem, it is a variable the leader controls and optimizes~---~when we write the dual for the ${\sf Heuristic}()$ we have to multiply constraints that contain $P$ ($\mathcal{I}$ in \eqnref{eq:metaopt_full}) with the dual variable which turns the problem into one that is no longer linear. 

%Non-linear constraints slow down the optimization. We quantize the space of inputs to remove this non-linearity: once (and only after) we choose a quantile for an input it becomes a constant in the multiplication which then becomes a linear constraint.

% To remove this non-linearity (which otherwise would slow down the solution) we convert it to a decision process which we can then convert to linear constraints.

Non-linear constraints slow down the optimization. To remove this non-linearity, we quantize the space of inputs and through that convert the multiplicative constraint into a different type of multiplicative constraint: one that multiplies a binary variable with a linear term~---~we can use standard optimization theory to linearize such constraints~\cite{boyd_co}.



%\behnaz{@Pooria, double check simplex applies in our case.}
%\pooria{Summary of our discussion: Simplex theorem guarantees that the worst-case happens at the extremum points which are finite, and if the quantization levels completely capture these points, this approach does not impact the quality of the solution. However, finding all the extremum points can be both computationally challenging and result in scalability problem for \metaopt (in case there are too many independent levels). Hence, we use the most probable quantization levels; ...}

%The Primal-Dual rewrite of ${\sf Heuristic}()$ might generate a nonlinear optimization (as in \figref{}). The nonlinearity appears in the dual objective function because of the product of outer level variable ($\mathcal{I}$ in \eqnref{eq:metaopt_full}) and inner level dual variables.

%\footnote{Multiplicative terms appear in the KKT encoding as well but we can not use the quantization idea since the quantization levels are unknown for KKT multipliers ($\lambda$ in~\figref{f:eg_conversion}).};
%for a subspace of heuristics, we find the worst gaps happen only at extremum points; thus, constraining or quantizing the space of inputs can speedup the search and enables us to linearize the Priaml-Dual rewrite without sacrificing quality. 

%For example, for \pop, demands in the worst-case traffic matrix are either zero or max, and for \dempin, most of the demands are either zero, threshold or max.

The leader has to pick the quantile~---~the quantiles are variables of the outer problem and we need to enable the outer problem to choose between them as part of the optimization. 
To quantize an input $d$ into $k + 1$ different levels ($=\{0, L_{1},\dots,L_{k}\}$), we have to add $k$ auxiliary binary variables~---~$x_j$ such that $\sum_{j=1}^{k}x_j \leq 1$~---~and replace $d$ with $\sum_{j=1}^{k}L_{j}x_{j}$. This changes the non-linear term we had initially in the dual objective into a product of two terms: a continues variable (\ie dual variable) and a binary one (\ie $x_{j}$). We can now use a big-$M$ approach to convert this term into a linear form~. The big-$M$ approach linearizes a term such as $p = xy$ where $x$ is binary and $y$ continuous as:

{\small
	\begin{eqnarray}
		p \geq y - M (1 - x),\,\, p \leq y + M (1 - x), \nonumber \\
		p \geq - Mx_i,\,\, p \leq Mx_i, \nonumber
	\end{eqnarray}
}
where $M$ is a upper bound on $|y|$ and is constant. The first two constraints ensure $p = y$ when $x =1$ and the last two that $p = 0$ otherwise.
The Gurobi ${\sf Indicator}$ function performs this conversion automatically~\cite{gurobi}.

We can pick the quantization levels to avoid impact on solution quality. The Simplex theorem~\cite{bertsimasLinOptBook} ensures the inputs that cause the worst case gap happen at the extremum points of the feasibile set (the set of inputs that satisfy all of the constraints in the optimization form a convex set which we call the feasibility set). In \pop, for example, the demands that cause the worst case gap are either zero or max. In \dempin we find the demands that cause the worst case gap are either zero, the \dempin threshold, or max. If we set our quantization levels to be this set of extremum points (which we can use the optimization's constraints to compute) we can use the Simplex theorem to ensure our re-write remains optimum. 

In practice the set of extremums can be prohibitively large and we instead use a subset. We find empirically that if we choose the right subset~---~the ones that are more likely to be optimal~---~we can avoid any impact on solution quality.

But how do we find such quantization levels? We use the KKT encoding~---~which is slower~---~on a small example: we use the solution to pick the quantization levels for primal-dual. We next describe how the KKT approach works.

\parae{KKT encoding.} Based on the $KKT$ theorem, we can take an optimization and convert it to a set of feasibility constraints: {\em any} $w$ and $\ell$ in our example that satisfy these constraints are optimal (they maximize the objective) in the original optimization. The result is an optimization (the optimization on the right in~\autoref{f:eg_conversion}) where the objective is to find a feasible point that satisfies the constraints. We can use such KKT rewrites on any convex problem which has at least one strictly feasible point (Slater's condition~\cite{boyd_co}). 

We prefer convex problems: we can solve convex problems in polynomial time. This is not the case when we use KKT encodings: the multiplicative constraint $\lambda (w + l - \frac{P}{2}) = 0$ is not convex (in the multiplicative terms in primal-dual we know the inputs are bounded and we know these bounds and so we can use quantization but in KKT this is not the case). Luckily, commodity solvers support this type of non-convexity~---~ we can encode them using special ordered sets in Gurobi~\cite{gurobi} and disjunctions in Z3~\cite{Z3}. But we now have increased the problem size~(in our example, the $1$ constraint and $2$ variables on the top left increased to $5$ and $3$ respectively on the right) which combined with non-convexity slows down the solver. This is why we use the primal-dual method instead to scale and only use the KKT approach on a small example to quickly find the right quantile levels for primal-dual.

%

%\ramesh{The first para of Primal-dual is nice, and can be a model for how to write the KKT intuition. And yes, an example would help.}


The primal-dual method scales better than $KKT$ because it has fewer binary variables. The number of binary variables in KKT depends on the number of followers and the number of inequality constraints they have. For example, the number of constraints in the \dempin and \pop heuristics depend on the number of paths: if we increase the number of path we increase the number of binary variables we need and reduce the solver's ability to scale! In contrast the primal-dual approach requires only a fixed set of binary variables to quantize the input space.  



\behnaz{@Pooria, you need to describe this in more detail in an algorithm in the appendix and add a forward ref.}

\parab{Summary.} \tabref{tab:metaopt_rewrite_prop}. \pooria{need to complete this.}


\begin{table}
	\scriptsize
	\centering
	\begin{tabular}{|l|l|l|} \hline
		\textbf{\textit{Inner}} & \textbf{\textit{Encoding}} & \textbf{\textit{Properties}} \\ \hline \hline
		${\sf OPT}$ & Direct & \\ \hline
		\multirow{4}{*}{${\sf Heuristic}$} & Direct & applies to heuristics in the feasibility format.\\ \cline{2-3}
		& \multirow{2}{*}{KKT} & applies to heuristics in convex optimization. \\
		&& uses one binary variable per inequality constraint. \\ \cline{2-3}
		& \multirow{2}{*}{Primal-Dual} & applies to heuristic in convex optimization. \\ 
		&& uses binary variables to quantize the input space. \\ \hline
	\end{tabular}
	\caption{Summary of single-shot rewrite in \metaopt \pooria{fill the table}}
	\label{tab:metaopt_rewrite_prop}
\end{table}
}
% ======================== End Cut ====================================

%We are unaware of any commodity solver directly supporting two-stage optimization~\eqref{eqn:adversarial_outer}. When inner problems are convex, we can reformulate them as a single-shot optimization using KKT and replace them with sets of feasibility constraints. Take the example in~\autoref{f:eg_conversion}. The optimization on the right finds a feasible point satisfying the new constraints -- any such feasible solution is also optimal for the problem on the left. This property holds for any convex problem with at least one strictly feasible point (Slater's condition~\cite{boyd_co}). Variables for the outer problem, which are constants in the inner problems~($P$ in~\autoref{f:eg_conversion} and $\mathcal{I}$ in~\eqref{eqn:adversarial_outer}), play no role in the KKT rewrite. 
%
%An astute reader may observe potential issues with this translation: First, the inequality constraints in the optimization result in non-convex multiplicative constraints. However, we can encode multiplicative constraints using features available in commodity solvers -- special ordered sets in Gurobi~\cite{gurobi} and disjunctions in Z3~\cite{Z3}. Second (see~\autoref{f:eg_conversion}), the KKT conversion increases the problem size~($1$ constraint and $2$ variables on the top left increase to $4$ and $3$ respectively on the right) by a constant factor since the number of new variables and constraints is proportional to the size of the original problem. 
%% since KKT adds one new variable per inequality in the original problem and one per objective; KKT also adds one new constraint per variable in the original problem and one per new variable. 
%We empirically find the number of multiplicative constraints (not the overall size of the problem) determines the latency of the solver.

%While we are aware of prior works that use each of the above techniques~\cite{bilevel_3,bilevel_2,bilevel_1}, we are unaware of any prior work in networking that solves two-stage games, uses KKT rewrites or encodes multiplicative constraints as we do.

%% We show how to reformulate the problem as a single optimization that we can solve using commodity solvers (e.g., Gurobi~\cite{} or Z3~\cite{}) when the users can write the inner optimizations in Eqn.~\ref{eqn:adversarial_outer} as convex programs. \todo{Ryan: I don't understand this sentence. The thing we generate is not convex anyway? We haven't said what this means to the readers as well. Nor why it is important.} Without these changes, the meta-optimization in Eqn.~\ref{eqn:adversarial_outer} is not convex even if the inner optimizations are convex. The variables the outer problem optimizes over are treated as constants in the inner problems. For instance, the demand values are treated as constants in Eqns.~\ref{eq:max_flow}--\ref{eq:pop_max_flow}. The outer problem finds demands such that when we solve the {\sf Heuristic} and the {\sf OPT} problems (to find the flow assignment to each path) given these (constant) demands the gap between the two objectives is maximized.
%
%%
%
%%\subsubsection{Converting the problem}
%%\label{ss:kkt}
%
%% Using KKT conditions, we replace both of the inner problems with a set of constraints. 
%
%An astute reader may observe several potential issues with this translation: First, the inequality constraints in the optimization give rise to multiplicative constraints 
%%(complementary slackness constraints~\cite{boyd_co}) 
%that, in general, are not convex. However, we find we can express multiplicative constraints using features already available in commodity solvers --special ordered sets in Gurobi~\cite{} and disjunctions in SMT~\cite{}. Second, as is evident from~\autoref{f:eg_conversion}, the KKT conversion adds many additional constraints and variables. 
%%
%\todo{Ryan: This sentence is hard to follow and vague. can we say something simpler here? Like the problem size is provably a constant factor larger, and that constant is at most X in practice.}
%%
%We will show however that the problem size is provably no more than a constant factor larger. 
%% the numbers of additional constraints and variables is bounded by the numbers of the constraints and variables in the original problems and so the modified problem is within one order of magnitude in size of the inner problems. 
%In our experiments, we find the numbers of multiplicative constraints (and not the overall size of the outer problem) directly determines the solver latency. %\todo{optimizations}
%
%\todo{Ryan: in hindsight, one thing that may not be coming through clearly is why the original problem of opt - heuristic is hard to solve. Why do we need these fancy tricks. Why can't solvers just directly solve the problem. Are there stackleberg solvers?}

\subsection{Scaling using Clustering}
\label{ss:cluster}

The rewriting approaches we described in \secref{ss:convex-follower} convert the two level optimization~\eqref{eqn:adversarial_outer} into a Mixed Integer Linear Program (MILP). But MILPs do not scale~---~they are not convex. To scale to larger problem sizes for graph-based heuristics (\eg for WAN TE), \metaopt uses graph clustering.

Our approach is similar to NCFLow~\cite{ncflow} and \pop. These approaches partition the topology (each in different ways), solve the problem in parallel on the smaller topologies, and then {\em stitch} the results to produce the overall solution. But since \metaopt solves a two-level optimization the problem is more nuanced and if we do not do it properly we may get adversarial inputs that are far from the optimal (worst-case). This problem mostly arises in the last step where we want to find the inter-cluster inputs.

\metaopt first breaks the optimization into smaller sub-problems (clusters) (\figref{fig:metaopt-cluster-example})~\cite{azadeGap,clustering-1,clustering-2,louvain_method,communities} which it can solve faster and in parallel. 


Next is the more difficult step: we need to combine these intra-cluster inputs and add inter-cluster inputs to produce the overall solution. If we ignore the intra-cluster inputs (like NCFlow~\cite{ncflow}) in this step our solution may be highly sub-optimal. To avoid this we ensure the optimizer observes the adversarial intra-cluster inputs we have found on the individual clusters when it searches for inter-cluster inputs. The solution (1) initializes the input matrix with 0s; (2) computes, in parallel, the intra-cluster inputs ($\mathcal{D}_{ii}$) for each cluster (\figref{fig:metaopt-cluster-demand-matrix}); and (3) computes the inter-cluster inputs ($\mathcal{D}_{ij}$) for each cluster pair. In the last step, it fixes all (the intra-cluster inputs) but a small part of the input matrix (the inter-cluster inputs) and fills each part one at a time (\figref{fig:metaopt-cluster-method}).

We can still use this method to analyze heuristics such as \pop (even though \pop itself is a partitioning solution): within a cluster, \pop would still partition the topology. Clustering also does not interfere with rewriting~---~depending on the scale of the cluster, \metaopt can use approximate or exact rewrites. Like approximate rewriting, clustering also does not guarantee the input it finds produces the worst-case gap. 

%Clustering is also orthogonal to rewriting; depending on the scale of the cluster, \metaopt can use approximate or exact rewrites. Finally, like approximate rewriting, clustering is also not guaranteed to produce the worst-case input.




% \metaopt breaks the optimization into smaller sub-problems and divides the topology into smaller clusters (\figref{fig:metaopt-cluster-example})~\cite{azadeGap,clustering-1,clustering-2,louvain_method,communities}: the sub-problems are smaller (we can solve them faster) and run in parallel. \metaopt finds adversarial (intra-cluster) inputs for each partition separately. Then it combines these intra-cluster inputs and adds inter-cluster inputs to produce the overall solution.

%This last step, which finds adversarial inter-cluster demands, is non-trivial. 


 %For example, if we ignore the intra-cluster demands and decompose the inter-cluster demands on an abstracted topology (similar to the approach in NCFlow~\cite{ncflow}) it can lead to smaller adversarial gaps (sub-optimality). To avoid this, \metaopt ensures the optimizer has visibility into the adversarial intra-cluster demands it has found when it searches for the inter-cluster demands. It (1) initializes the demand matrix with 0s; (2) computes, in parallel, the intra-cluster demand ($\mathcal{D}_{ii}$) for each cluster (\figref{fig:metaopt-cluster-demand-matrix}); and (3) computes the inter-cluster demands ($\mathcal{D}_{ij}$) for each cluster pair. In the last step, it fixes all (the intra-cluster demands) but a small part of the demand matrix (the inter-cluster demands) and fills each part one at a time (\figref{fig:metaopt-cluster-method}).

%Clustering is orthogonal to how heuristics such as \pop operate; within a cluster, \pop would still partition the topology. Clustering is also orthogonal to rewriting; depending on the scale of the cluster, \metaopt can use approximate or exact rewrites. Finally, like approximate rewriting, clustering is also not guaranteed to produce the worst-case input.

The difference between our clustering technique and NCFlow~\cite{ncflow} is that to satisfy as much demand as possible, the latter partitions the topology into smaller clusters, routes (and allocates rates to) the demands within each cluster, and then uses an abstract topology (where each cluster is a meta-node) to find the inter-cluster rate allocations. NCFlow needs to reconcile intra-cluster routes with inter-cluster routes, a step that \metaopt does not need since it seeks to produce adversarial inputs.

%\srikanth{as with 3.1, needs a major rewrite. Consider saying key idea -- partition into sub-problems similar to NcFlow and POP. However, there is nuance because unlike NcFlow and POP which maximize one-level optimizations \metaopt is a two-level optimization. In particular, converse example1 and converse example2. Then, describe the method.  The method itself seems like an *example*; as in, other methods or variants are feasible. So we should say why this method (is it simple, is it perfect? or...?)}


% But the goal and the approach in \metaopt is different. NCFlow needs to find the optimal routes for a given set of demands and has to reconcile the output of different clusters as a result~---~it would congest the intra-cluster links otherwise. This is not an issue in \metaopt which finds inputs (\eg demands) that maximize the gap between the heuristic and the optimal within a cluster~---~we do not need a reconciliation phase to fix the demand we find in \metaopt.

% Notice this clustering approach does not interfere with how heuristics such as \pop operate: \pop still partitions the topology within the cluster. The main change is the scale at which we run \pop in each cluster.

% Our clustering approach is a heuristic and does not find the worst-case gap. But we can use it to analyze heuristics, find lower bounds on what the worse-case gap may be,  find inputs that would cause the heuristic to perform poorly, and compare and improve different heuristics.


  

 
%More specifically, \metaopt first initializes the demand matrix with 0s. Then, it starts by filling each part of demand matrix one at a time (\figref{fig:metaopt-cluster-demand-matrix}) while fixing the rest of the demands. First, it goes through each cluster and computes the adversarial intra-cluster demand (\ie $\mathcal{D}_{ii}$) and then, goes through every pair of clusters and computes the inter-cluster demands (\ie $\mathcal{D}_{ij}$). \metaopt can compute intra-cluster and inter-cluster demands either sequentially or in parallel depending on the time budget and available computational resources.

%\ramesh{I may have missed it, but we haven’t introduced NCFlow, so it is a little hard to understand the comparison. We might add a few sentences about NCFlow and what it does.}
%\ramesh{Also, I would first completely describe what MetaOpt does, and at the end of the section compare with NCFlow. The current discussion interleaves the two which makes it hard to read.}
%\ramesh{Finally, we might briefly point out that this clustering is orthogonal to the partitioning in POP; i.e., POP would still partition within each cluster. Also, should this section go after 3.3, since the latter follows logically after a discussion of Primal-Dual?}
%Optimizations typically do not scale to large systems due to their enormous number of variables and constraints. Recently, NCFlow~\cite{ncflow} and POP~\cite{pop} have explored reducing the search space of optimizations by breaking the problem into smaller sub-problems. 

%As shown by~\cite{ncflow}, WAN topologies are usually constructed from a few well-connected partitions and WAN demands are mostly between nearby nodes. \metaopt uses this intuition to break the problem into smaller subproblems that can be solved separately and in parallel. More specifically, \metaopt divides the topology into different clusters, each containing 

%\begin{figure}
%	\begin{center}
%		\begin{tikzpicture}[->,>=stealth']
%			\node[state,
%			text width=3cm] (A) 
%			{\footnotesize
%				\begin{equation}
%					\mathcal{D} \gets 0_{|V| \times |V|} \nonumber
%				\end{equation}
%			};
%		
%			\node[state,
%			below of=A,
%			yshift=-1.0cm,
%			text width=6.5cm] (B) 
%%			{\begin{equation}
%%%					$\forall clusters:$ \\
%%%					$\,\,\arg\max_{\text{s.t. demand} \mathcal{D} \in ConstrainedSet}$ ${\sf OPT}() - {\sf HUERISTIC}()$\\[.5em]
%%%					$2 \cdot (w + \ell) \geq P$ \\
%%%					$P \geq 0$ \\
%%			\end{equation}};
%			{{\footnotesize
%				\begin{alignat}{4}
%					\mbox{$\displaystyle \label{eq:metaopt_intra_cluster} \forall Cluster\,\,\, i:$}&& \\ 
%					&{\mathcal{D}_{ii} \triangleq \arg\max {\sf OPT}(\mathcal{D}) - {\sf Heuristic}(\mathcal{D})}& \nonumber \\
%					\mbox{s.t.} \quad & {\mathcal{D}_{ii} \in {\sf ConstrainedSet}} & \nonumber\\
%					& {\mbox{FixDemands}(\mathcal{D}\setminus\mathcal{D}_{ii})} \nonumber \\
%					& \mbox{SingleShotRewrite}({\sf OPT}, {\sf Heuristic}) \nonumber
%			\end{alignat}}};
%			
%%			\node[state,
%%			text width=3.2cm,
%%			right of=A,
%%			yshift = -1.1cm,
%%			node distance=4.8cm,
%%			anchor=center] (B)
%%			{%
%%				{\begin{tabular}{l}
%%						\textbf{solve} for $w, \ell, \lambda$\\[.5em]
%%						$2 \cdot (w + \ell) \geq P$ \\
%%						$P \geq 0$ \\
%%						$\lambda \geq 0$ \\
%%						$2w - 2\lambda = 0$ \\
%%						$2\ell - 2\lambda = 0$ \\
%%						%		$\big( \lambda = 0 \big)$ or \\
%%						%		$~~~~\big( w + \ell - \frac{P}{2} = 0 \big)$ \\
%%						$\lambda\big( w + \ell - \frac{P}{2} \big) = 0$\\
%%				\end{tabular}}
%%			};
%			
%			\node[state,
%			below of=B,
%			yshift=-1.9cm,
%			anchor=center,
%			text width=8cm] (C) 
%			{%
%				{\footnotesize
%					\begin{alignat}{4}
%						\mbox{$\displaystyle \label{eq:metaopt_inter_cluster} \forall Clusters\,\,\, i, j, i\neq j:$}&& \\ 
%						&{\mathcal{D}_{ij} \triangleq \arg\max {\sf OPT}(\mathcal{D}) - {\sf Heuristic}(\mathcal{D})}& \nonumber \\
%						\mbox{s.t.} \quad & {\mathcal{D}_{ij} \in {\sf ConstrainedSet}} & \nonumber\\
%						& {\mbox{FixDemands}(\mathcal{D}\setminus\mathcal{D}_{ij})} \nonumber \\
%						& \mbox{SingleShotRewrite}({\sf OPT}, {\sf Heuristic}) \nonumber
%				\end{alignat}}
%			};
%			
%			\path 
%%			(A) 	edge[bend left=20]  node[anchor=south,above]{KKT}
%%			node[anchor=north,below]{encode} (B)
%			(A)     	edge  (B)
%			(B)     	edge  (C);
%%			(B)       	edge[bend left=20]  node[anchor=south,above]{solve}      (C);
%			
%		\end{tikzpicture}
%	\end{center}
%	\caption{{The clustering algorithm in {\metaopt}.\label{fig:metaopt-cluster-formulation}}}
%\end{figure}

%	\begin{algorithm}[t]
%	\caption{MetaOpt-Clustering}\label{alg:metaopt-clustered}
%	\begin{algorithmic}
%		\begin{footnotesize}
%			\Input : $\mathcal{G}$, $\mathcal{N}_c$
%			\EndInput
%			\State $\mathcal{G}_c \gets \mathbf{partition\_topology(\mathcal{G}, \mathcal{N}_c)}$
%			\State $\mathcal{D} \gets 0_{N\times N}$
%			\For{$i \in 1,\dots,\mathcal{N}_c$}
%				\State $D_{ii} \gets \metaopt(G)$
%			\EndFor
%			\State $\mathbf{d} \gets \mathbf{d}_0$, $\,\,\,k \gets 0$ 
%			\While{$k < K$}
%			\State $\mathbf{d}_{\mathrm{aux}} \gets \max(\mathbf{d} + \mathbf{z}, \mathbf{0})\,\,\,\,$ where $\,\,\,\,\mathbf{z} \sim \mathcal{N} (\mathbf{0}, \sigma^2 \mathbf{I})$
%			\IIf{$\mathrm{gap}(\mathbf{d}_{\mathrm{aux}})>\mathrm{gap}(\mathbf{d})$} $\mathbf{d} \gets \mathbf{d}_{\mathrm{aux}}$, $\,\,\,k \gets -1$
%			\EndIIf
%			\State $k \gets k+1$			
%			\EndWhile
%			\Output : $\mathbf{d}$
%			\EndOutput
%		\end{footnotesize}
%	\end{algorithmic}
%	\vspace{-1mm}
%\end{algorithm}

\begin{figure}
	\centering
	\subfigure[Clustered Topology.]{\centering\includegraphics[width=0.45\linewidth]{figs/MetaOpt-clustered-Example-Topo.pdf}\label{fig:metaopt-cluster-example}} \hfill
	\subfigure[Clustered Demand Matrix.]{\centering\includegraphics[width=0.51\linewidth]{figs/MetaOpt-clustered-final.pdf} \label{fig:metaopt-cluster-demand-matrix}} \hfill
	\subfigure[MetaOpt Clustering Method.]{\centering\includegraphics[width=1.0\linewidth]{figs/MetaOpt-Clustering-Method.pdf} \label{fig:metaopt-cluster-method}}
	\caption{\textbf{An example of {\metaopt}'s clustering approach.}}
%	\vspace{-4mm}
\end{figure}

%\cut{ %% Moved to section 4





%}


==> texfiles/usecases.tex <==
\section{Using \metaopt}
\label{ss:convexify}

%In this paper, we use \metaopt to analyze three heuristics: \dempin and \pop for traffic engineering, and \ffd for vector bin packing. 
%These heuristics are of practical importance. 
%For example, Microsoft has deployed the \dempin heuristic~\cite{blastshield} to scale SWAN to larger topologies. 

To use {\metaopt}, it is important to encode different heuristics as either a feasibility problem or a convex optimization. This section explains the process for encoding \dempin, \pop, and \ffd.
These heuristics are of practical importance. 
For example, Microsoft has deployed the \dempin heuristic~\cite{blastshield} to scale SWAN to larger topologies. 
In the end, we provide examples of how {\metaopt} can help analyze heuristics and improve their worst-case performance.

%\metaopt requires we encode these heuristics as either a feasibility problem or a convex optimization. We show how to do this in this section for \dempin, \pop, and \ffd.


%\behnaz{@Pooria you should add the vector bin packing heuristic here too.}
\subsection{Heuristics for Traffic Engineering}
\label{ss:convexify:te}

%\vspace{0.07in}
\parab{Demand Pinning.} \dempin contains an {\em if} clause: if a demand is smaller than the threshold $T_d$, then route it over its default shortest path; otherwise, use the optimal algorithm to route it. 
We leverage the quantized demands in the primal-dual encoding to express this clause in convex form;
%
{\small
	\begin{eqnarray}
		f_k^{\widehat{p}_k} \geq \sum_{j=0}^{Q} \mathbb{1}[L_{j} \leq T_d] L_{j}x^{k}_{j}, \,\,\, \forall k \in \mathcal{D}, \nonumber
	\end{eqnarray}
}
%
%\santi{I am a bit confused by the equation above. First, it seems like we are using $k$ for two things, the number of quantization levels and the indexing of the demand, right? Also, how is this enforcing the conditional? or is this just part of that. In particular, the demand $d_k$ does not appear anywhere in the equation, so something must be missing.}
%\pooria{Thanks for catching this mistake. I updated the formulation so it uses $Q$ as the number of quantization levels. For the second question about demands. We are quantizing demands and hence, we are replacing them with $\sum_{j}L_jx^k_j$. So, $L_j$s and $x^{k}_{j}$ are reflecting the demand value ($d_k$). I updated the text to better show this. please review.}
where  $\{0, L_0, \dots,L_Q\}$ are the quantization levels, $x^k_j$s are the binary variables that decide which quantization level is active for demand $k$ (the term $\mathbb{1}[L_{j} \leq T_d]$ does not contain any variables and only indicates which terms are present in the sum above), and $\widehat{p}_k$ denotes the shortest path for demand $k$. 
When demand $d_k$ is below the threshold $T_d$, one of the quantization levels below $T_d$ is in effect (\ie $x^k_j = 1$). 
To ensure such demands follow their default shortest path $\widehat{p}_k$, we use these constraints to lower bound the related flow variables.
These constraints effectively mimic the big-$M$ model from standard optimization theory~\cite{boyd_co} but result in better solver performance in practice (we show the big-$M$ formulation of {\dempin} in appendix~\S\ref{sec:dempin_bigM}~---~ we use it for our KKT encoding where the demands are not quantized).

\parab{Partitioned Optimization Problems.} {\pop} is convex as it is the union of solutions to multiple disjoint linear optimizations (\eqnref{eq:pop_max_flow}). The challenge in encoding {\pop} lies in its random partitioning, which makes ${\sf POP}(\mathcal{I})$ a random variable in the leader problem. To use {\metaopt}, we need a deterministic representation of these random variables. One way is to look at an specific instance of the random variable but this could result in overfitting to that instance and not reflecting the true behavior of {\pop}. Instead, we rely on the {\em expected value} or a {\em tail percentile} of the worst-case gap. 

For computing the average worst-case gap, we replace \heur in \eqnref{eq:metaopt_full} with its expected value and approximate this expectation through empirical averages over a few randomly generated partitions (see \secref{s:eval:te}). To find the tail worst-case gap, we use a sorting network~\cite{sorting_net_1,pretium} to compute the desired percentile across multiple random partitions. We discuss an advanced version of {\pop} in~\secref{s:appendix:pop} which can divide a large demand between multiple partitions instead of assigning it to a single one.



\subsection{Heuristics for Vector Bin Packing}
\label{ss:convexify:vbp}

To demonstrate the generality of \metaopt, we use it to examine a heuristic for vector bin packing~\cite{protean,tetris,synergy} (\vbp). Resource schedulers use \vbp to help cloud providers assign jobs to available machines~---~they decide how to allocate jobs that need resources along multiple dimensions (\eg memory, CPU, GPU~\cite{drf,borg,pond}). 
\vbp helps reduce resource fragmentation~\cite{jobpacking} and improve efficiency~\cite{tetris} of the clusters.

%Cloud providers use resource schedulers~\cite{protean,borg} to assign available machine to jobs that require resources along multiple dimensions (\eg memory, CPU, GPU)~\cite{protean,pond,borg,jobpacking,drf}. A common approach in these schedulers is to use vector bin packing (\vbp)~\cite{protean,tetris,synergy} as it reduces the resource fragmentation~\cite{jobpacking} and increases the overall efficiency of clusters~\cite{tetris}. 

The objective of \vbp is to fit a set of balls into the minimum number of bins (both with sizes in $\mathbb{R}^n$ where n is the dimension of resources) while respecting the capacity of the bins. 
\vbp is an APX-hard problem~\cite{vbp-nphard}, so resource schedulers often use heuristics to solve \vbp at scale~\cite{VBP-Heuristics}. In this paper, we investigate the worst-case performance of a class of heuristics, first fit decreasing ({\ffd}), which is widely used in practice~\cite{VBP-Heuristics,ffdprod-sandpiper,ffdsum-example,ffddiv-ibm,tetris,protean,synergy}. 

\ffd is a greedy heuristic that iteratively picks the largest unassigned ball and places it in the first bin with enough capacity. It has been shown both empirically and theoretically that \ffd works well in single-dimension (where each job only needs a single resource)~\cite{ffd-1d-tight}.

In multi-dimensional cases, \ffd needs to assign a weight to each ball, which is used to sort them. Researchers have proposed many such weight functions that convert the vector of ball sizes into a scalar:  FFDSum~\cite{ffdsum-example}, FFDDiv~\cite{ffddiv-ibm} and FFDProd~\cite{ffdprod-sandpiper} (more details in Appendix~\S\ref{sec:vbp_details}).
%The multi-dimension \ffd solutions use a weight function to assign merit to each ball~---~they convert the vector of ball sizes into a scalar~---~and use it to sort them. Researchers have proposed many such functions:  FFDSum~\cite{ffdsum-example}, FFDDiv~\cite{ffddiv-ibm} and FFDProd~\cite{ffdprod-sandpiper} (see Appendix~\S\ref{sec:vbp_details} for the details).

Unlike \dempin and \pop, \ffd is {\em not convex} as it has binary decision variables. In addition, \ffd is iterative, so modeling these iterations as part of the optimization is crucial. To use {\metaopt}, we propose a novel re-formulation of \ffd that captures its behavior using a set of feasibility constraints. We explain our solution in detail in Appendix~\S\ref{sec:vbp_details}, but outline the underlying ideas here. 


To ensure the fidelity of our formulation, we must guarantee that in every iteration $i$: (1) it finds the largest unassigned ball, and (2) it places the ball in the first bin with enough capacity. To address the first requirement, we use ${\sf ConstrainedSet()}$ (\eqnref{eq:metaopt_full}) to force the leader to index balls in descending order of their weights. This means that the ball with index $i$ has a higher weight than all the balls with higher indices. To meet the second requirement, we keep track of the remaining capacity of each bin after placing the first $(i-1)$ balls. Then, we use the constraints to identify the bin with the lowest index that can fit ball $i$.

%To ensure the fidelity of our formulation, we must guarantee that in every iteration $i$: (1) it finds the largest unassigned ball, and (2) it places the ball in the first bin that has enough capacity. To address the first requirement, we can assume the balls are already sorted based on their weights without loss of generality (it is simply a re-indexing of the balls). Therefore, we use ${\sf ConstrainedSet()}$ to restrict the leader's search space to inputs where ball $i-1$ has a higher weight than ball $i$. To meet the second requirement, we keep track of the remaining capacity of each bin after placing the first $(i-1)$th balls. Then, we use the constraints to identify the bin with the smallest index that can fit ball $i$.

We also have to track capacity along multiple dimensions and encode the leader's objective. We defer the reader to  Appendix~\secref{sec:vbp_details} for the details on how we model these aspects.

%To enforce that the solution proceeds in the correct order, we use the constraint set ${\sf ConstrainedSet}$ in the outer problem: when the outer problem assigns weights, it has to assign a higher weight to item $i$ compared to item $i + 1$. Notice that this is done without loss of generality: the constraint is only enforcing we index them based on their weights. We can now use these indices to model how \ffd assigns balls one at a time from largest to smallest~---~we formulate the problem such that we assign item $i$, then $i + 1$, and so on.

%What remains is to track capacity and encode the leader's objective. We defer the reader to  Appendix~\S\ref{sec:vbp_details} for the details on how we model these aspects.


%\pooria{papers to cite: \cite{tetris,VBP-Heuristics,protean,synergy,drf,pond,jobpacking,borg,vbp-nphard,ffdprod-sandpiper,ffdsum-example,ffddiv-ibm}}



\subsection{Other uses of {\metaopt}}
\label{ss:extensions}

In \secref{ss:convex-follower}, we have discussed how \metaopt can find worst-case and adversarial inputs. With appropriately designed additional constraints, it can  analyze other properties of heuristics.

% \parab{Find adversarial inputs.} The basic use of \metaopt is to identify the input that leads to the largest gap between the optimal and the heuristic. This allows for a more thorough evaluation of the performance of the heuristics.

%\parab{Evaluate heuristics under realistic conditions.} Sometimes, the examples discovered by {\metaopt} do not represent the typical input behavior (see~\secref{s:eval:te}). This raises concerns that the gap might not reflect the heuristic's performance under ``realistic'' workloads. To overcome this, operators can utilize the ${\sf ConstrainedSet}()$ in {\metaopt} to limit the search space to practical cases. Examples of this include;

\parab{Find inputs with bounded distance from a goalpost.} Users can search for adversarial demands within a certain {\em distance} from a {\em goalpost}. This can help them understand how far inputs can deviate from the norm before the heuristic breaks. Using this, they can determine an appropriate threshold for switching heuristics or applying other remedies. Users specify these goalposts using the ${\sf ConstrainedSet}$ in~\eqnref{eq:metaopt_full}; they do not need to fully specify the goalposts and can leave some demands unconstrained.

\parab{Compare input sets.} \metaopt can analyze the {\em types} of input a heuristic is sensitive to. For example, it can output the adversarial gap when the inputs are sparse or when they exhibit strong locality (\eg distance between the nodes that exchange traffic in TE). To compare input sets, users must specify each set as a ${\sf ConstrainedSet}$ in~\eqnref{eq:metaopt_full}. Each constraint is in terms of $g(\mathcal{I}) \geq f(\mathcal{I})$ or $g(\mathcal{I}) = f(\mathcal{I})$ where $f$ and $g$ are functions of the input $\mathcal{I}$.

\parab{Analyze a combination of heuristics.} Users can potentially reduce the optimality gap of different heuristics that solve the same problem by combining them. This is effective if these heuristics have a non-overlapping set of adversarial inputs, as each can cover weaknesses of the other heuristics. In {\metaopt}, users can analyze the performance of combining heuristics by replacing ${\sf Heuristic}(\mathcal{I})$ in the objective of~\eqnref{eq:metaopt_full} with $\max_{h}({\sf Heuristic}_{h}(\mathcal{I}))$ so that the follower returns the solution of the best heuristic for each input:
%
%Different heuristics that solve the same problem have different adversarial patterns: we can potentially reduce the optimality gap of these heuristics by combining them. Operators can use \metaopt to analyze such combinations and understand the resulting heuristic. We can replace ${\sf Heuristic}(\mathcal{I})$ in the objective of~\eqnref{eq:metaopt_full} with $\max_{h}({\sf Heuristic}_{h}(\mathcal{I}))$ so that the follower returns the solution of the best heuristic for each input:

\vspace*{-2ex}
{\small
	\begin{alignat}{3}
		\label{eq:metaopt_multiple_heuristics} 
		&\mbox{\sf AdversarialInput}() \triangleq \nonumber\\& \arg\max_{\mathcal{I}}\,\,{\sf OPT}(\mathcal{I}) - \max_{h}({\sf Heuristic}_{h}(\mathcal{I}))&
	\end{alignat}
}
%
To transform~\eqnref{eq:metaopt_multiple_heuristics} to a single-level optimization, \metaopt needs to rewrite each of the heuristics using techniques from~\secref{ss:convex-follower}. In \secref{}, we show how combination of \dempin and \pop reduces the worst-case gap by XXX. \pooria{fill this after finishing the evaluation.}

\parab{Improve heuristics through strategic changes.} Users can study the adversarial inputs from \metaopt to understand when and why a heuristic underperforms. Understanding these weaknesses can help them apply fixes to reduce the optimality gap. We show how to do this for \dempin in~\secref{s:eval:te}.
%\pooria{fill this after finishing evaluation.}


\parab{Compare Heuristics.} \metaopt can compare heuristics directly (instead of comparing with \opt): 

\vspace*{-2ex}
{\small
	\begin{equation}
		\mbox{\sf AdversarialInput}() \triangleq \arg\max_{\mathcal{I}}\,\,{\sf Heuristic}_{1}(\mathcal{I}) - {\sf Heuristic}_{2}(\mathcal{I}) \nonumber
\end{equation}}

\parab{Identify Suitable Inputs.} \metaopt can also identify ideal inputs for a given heuristic. Users can achieve this by altering the objective of the leader in~\eqnref{eq:metaopt_full}, so it minimizes the gap between \opt and \heur instead of maximizing it. 

\vspace*{-2ex}
{\small
	\begin{equation}
		\mbox{\sf SuitableInput}() \triangleq \arg\min_{\mathcal{I}}\,\,{\sf OPT}(\mathcal{I}) - {\sf Heuristic}(\mathcal{I}) \nonumber
\end{equation}}
%
Users should restrict inputs using ${\sf ConstrainedSet}()$ to ensure the answers are meaningful and relevant. Without these constraints, the optimization may lead to trivial answers. For example, if there are no demands in the network, any traffic engineering heuristic is optimal.

